Structured Regularization for conditional Gaussian Graphical Models

Conditional Gaussian graphical models (cGGM) are a recent reparametrization of the multivariate linear regression model which explicitly exhibits $i)$ the partial covariances between the predictors and the responses, and $ii)$ the partial covariances between the responses themselves. Such models are particularly suitable for interpretability since partial covariances describe strong relationships between variables. In this framework, we propose a regularization scheme to enhance the learning strategy of the model by driving the selection of the relevant input features by prior structural information. It comes with an efficient alternating optimization procedure which is guaranteed to converge to the global minimum. On top of showing competitive performance on artificial and real datasets, our method demonstrates capabilities for fine interpretation of its parameters, as illustrated on three high-dimensional datasets from spectroscopy, genetics, and genomics.

==> ResMotif-K8.tex <==
\begin{tabular}{l} 
{\tt AGGCACAGCTCATCGCGTTTT} \\ 
\hline 
{\tt ~~~~~~~~~~~ATCGCATT} \\ 
{\tt ~~~~~CACCTCAT} \\ 
\end{tabular} & 
\begin{tabular}{l} 
{\tt GATAGCGC} \\ 
\hline 
{\tt GTTAGAGT} \\ 
{\tt AGAAGCGT} \\ 
\end{tabular} & 
\begin{tabular}{l} 
{\tt CTTACCCCACGG} \\ 
\hline 
{\tt ~~~~CCTCACGA} \\ 
{\tt ~~~ACCTCAAG} \\ 
\end{tabular} & 
\begin{tabular}{l} 
{\tt ATCATGTA} \\ 
\hline 
{\tt CTCAGGTT} \\ 
{\tt AGCGTATT} \\ 
\end{tabular} \\ 
  \\ 
\begin{tabular}{l} 
{\tt AAGGGGCGG} \\ 
\hline 
{\tt TGTGTGGG} \\ 
{\tt ~GGGGGCCA} \\ 
\end{tabular} & 
\begin{tabular}{l} 
{\tt CGGTGTTATA} \\ 
\hline 
{\tt CGATCATA} \\ 
{\tt ~GGACTTAT} \\ 
\end{tabular} & 
\begin{tabular}{l} 
{\tt GTGACTCT} \\ 
\hline 
{\tt GGCACTCC} \\ 
{\tt TTCTCTCT} \\ 
\end{tabular} & 
\begin{tabular}{l} 
{\tt CCAATGAG} \\ 
\hline 
{\tt TCAACTTC} \\ 
{\tt TCAATCGG} \\ 
\end{tabular} \\ 
  \\ 
\begin{tabular}{l} 
{\tt GGGGAGCATGCATCAAGGTGG} \\ 
\hline 
{\tt ~~~~~~~~TGCATCTA} \\ 
{\tt ~~~~~~~~~~CATCTCAG} \\ 
\end{tabular} & 
\begin{tabular}{l} 
{\tt ATTTCGAAAACCCGAGGGAGT} \\ 
\hline 
{\tt ~~~~~~~~~~~~CGATGAAA} \\ 
{\tt ~~~AAGAAAAC} \\ 
\end{tabular} & 
\begin{tabular}{l} 
{\tt ACGTAACGCCACCCTAATCG} \\ 
\hline 
{\tt ~ATAAACGC} \\ 
{\tt ~~~TAACGCCA} \\ 
\end{tabular} & 
\begin{tabular}{l} 
{\tt CACCCCTGA} \\ 
\hline 
{\tt CTCACCTT} \\ 
{\tt CTCACATG} \\ 
{\tt AACCCCTT} \\ 
\end{tabular} \\ 
  \\ 


==> ResMotif-K9.tex <==
\begin{tabular}{l} 
{\tt AAGCCGGAAGCGGGG} \\ 
\hline 
{\tt ~~ACAGGGTGC} \\ 
{\tt ~~~AAGGGAGCA} \\ 
\end{tabular} & 
\begin{tabular}{l} 
{\tt ATTTGCTTACGTAAGCTCGT} \\ 
\hline 
{\tt CTGTACTTA} \\ 
{\tt ~~~~~~~~~~~TAATGTCGT} \\ 
\end{tabular} & 
\begin{tabular}{l} 
{\tt GTTACCCGG} \\ 
\hline 
{\tt GGTCCCCTC} \\ 
{\tt GTGAACCGC} \\ 
\end{tabular} & 
\begin{tabular}{l} 
{\tt ATGCAACCTGTCA} \\ 
\hline 
{\tt ~~~CAAGCTGTG} \\ 
{\tt TGGCAAGCT} \\ 
\end{tabular} \\ 
  \\ 
\begin{tabular}{l} 
{\tt TTTGCACCC} \\ 
\hline 
{\tt GGCGCACCT} \\ 
{\tt GATGCACCC} \\ 
\end{tabular} & 
\begin{tabular}{l} 
{\tt CCTGTATTTAA} \\ 
\hline 
{\tt CCATTATTT} \\ 
{\tt ~~AGTATTTAT} \\ 
\end{tabular} & 
\begin{tabular}{l} 
{\tt ATGACTCAT} \\ 
\hline 
{\tt GGGACTCAC} \\ 
{\tt ATGATTGTC} \\ 
\end{tabular} & 
\begin{tabular}{l} 
{\tt TCTGCGGAAATTAAATACC} \\ 
\hline 
{\tt ~GTGCGGGAT} \\ 
{\tt TGTGCGGGA} \\ 
\end{tabular} \\ 
  \\ 
\begin{tabular}{l} 
{\tt CGTCCTTCGGCCGAAGGGGA} \\ 
\hline 
{\tt ~~~~~~~~~~CCGAGAGGG} \\ 
{\tt ~~AATGTCGGC} \\ 
\end{tabular} & 
\begin{tabular}{l} 
{\tt AAGAAAAATTAGGGGTGGAAT} \\ 
\hline 
{\tt ~~TAGTATTTA} \\ 
{\tt ~~~CAAATTTAG} \\ 
\end{tabular} & 
\begin{tabular}{l} 
{\tt ACTAGTGGATTCACCGA} \\ 
\hline 
{\tt ~ATAGTCAAT} \\ 
{\tt ~~AAGTGGACT} \\ 
{\tt ~~~~~~~ACTTCACTA} \\ 
\end{tabular} & 
\begin{tabular}{l} 
{\tt TTTTTGCTC} \\ 
\hline 
{\tt CTTTTGGTT} \\ 
{\tt GTTTTGCTC} \\ 
{\tt AGTTTGCTC} \\ 
\end{tabular} \\ 
  \\ 
\begin{tabular}{l} 
{\tt CAAATGAGATCTACAAACTG} \\ 
\hline 
{\tt ~~~~~~~~ATCTACTGC} \\ 
{\tt ~~TTGGAGATC} \\ 
{\tt ~~CTTGGGATC} \\ 
\end{tabular} & 
\begin{tabular}{l} 
{\tt CACTCGTGCGGCTGAAGCCGA} \\ 
\hline 
{\tt ~~~~~~~~~~GCTGTGGGA} \\ 
{\tt ~~~~~~~~~~GCTGTTACA} \\ 
{\tt ~~~~~~~~~~~~TGAGAGCTT} \\ 
\end{tabular} & 
\begin{tabular}{l} 
{\tt GGTGGCAAA} \\ 
\hline 
{\tt ATTGGCATA} \\ 
{\tt TGAGCATAA} \\ 
{\tt TGGGCAATA} \\ 
{\tt GGTACCTAT} \\ 
\end{tabular} & 


==> arxiv_version/.svn/text-base/v1/ResMotif-K7.tex <==
\begin{tabular}{@{}l@{}} 
{\tt CTAAGCCAC} \\ 
\hline 
{\tt ~~TAGCCCC} \\ 
{\tt ~~GCGCCCC} \\ 
\end{tabular} & 
\begin{tabular}{@{}l@{}} 
{\tt GCATGTGAA} \\ 
\hline 
{\tt CCATATG} \\ 
{\tt ~~TTGTGAG} \\ 
\end{tabular} & 
\begin{tabular}{@{}l@{}} 
{\tt CATGTAATT} \\ 
\hline 
{\tt ~~TGTAAAT} \\ 
{\tt ~~TGTATAT} \\ 
\end{tabular} & 
\begin{tabular}{@{}l@{}} 
{\tt TGAAACA} \\ 
\hline 
{\tt TTAGACC} \\ 
{\tt TAAAAAG} \\ 
\end{tabular} \\ 
  \\ 
\begin{tabular}{@{}l@{}} 
{\tt TGATCGGCGCCGCACGACGA} \\ 
\hline 
{\tt ~~~~~~~~~~~GTATAAC} \\ 
{\tt ~~~~~~GCGCCGT} \\ 
\end{tabular} & 
\begin{tabular}{@{}l@{}} 
{\tt TGCTGGTT} \\ 
\hline 
{\tt ~GCTGGTT} \\ 
{\tt ~GCTGGTG} \\ 
\end{tabular} & 
\begin{tabular}{@{}l@{}} 
{\tt GATCGTATGATA} \\ 
\hline 
{\tt ~ATCATAT} \\ 
{\tt ~TTGGTAT} \\ 
\end{tabular} & 
\begin{tabular}{@{}l@{}} 
{\tt ACGCGAAAA} \\ 
\hline 
{\tt ~AACGAAA} \\ 
{\tt ~~ACGAAAA} \\ 
\end{tabular} \\ 
  \\ 
\begin{tabular}{@{}l@{}} 
{\tt CCATACATCAC} \\ 
\hline 
{\tt ~CATAGAC} \\ 
{\tt ~~~~ATATCAC} \\ 
\end{tabular} & 
\begin{tabular}{@{}l@{}} 
{\tt ATTGACCTGGTC} \\ 
\hline 
{\tt ~TCGACTT} \\ 
{\tt ~~CGACTTG} \\ 
{\tt ~~~~~CCAGCTT} \\ 
\end{tabular} & 
\begin{tabular}{@{}l@{}} 
{\tt GACTAGATATATATATTCGAT} \\ 
\hline 
{\tt ~~~~~~~~~~ATATATT} \\ 
{\tt ~~~~~~~CATATAT} \\ 
{\tt ~~~~~~~~~~ATATATG} \\ 
{\tt ~~~~~~~~ATATATA} \\ 
\end{tabular} & 


==> arxiv_version/.svn/text-base/v1/application_cookies.tex <==
\subsection{Near-Infrared Spectroscopy of Cookie Dough Pieces}

\paragraph*{Context} In Near-Infrared (NIR)  spectroscopy, one aims to
predict one or several quantitative variables from the NIR spectrum of
a given sample.  Each sampled spectrum  is a curve that represents the
level of reflectance  along the NIR region, that  is, wavelengths from
800 to 2500 nanometers (nm).  The quantitative variables are typically
related to  the chemical  composition of the  sample.  The  problem is
then to  select the most predictive  region of the spectrum,  that is,
some peaks  that show  good capabilities  for predicting  the response
variable(s).   This   is  known   as  a  ``calibration   problem''  in
Statistics.  NIR technique  is used in fields as  diverse as agronomy,
astronomy or pharmacology.  In such  experiments, it is likely to meet
very strong correlations and structure  along the predictors.  In this
perspective, \cite{2011_JASA_hans}  proposes to apply  the Elastic-Net
which  is  known  to  selected  simultaneously  groups  of  correlated
predictors. However  it is  not adapted to  the prediction  of several
responses  simultaneously.  In  \citet{data_cookies2}, an  interesting
wavelets regression  model with Bayesian inference  is introduced that
enters the multivariate regression model, just like our proposal.

\paragraph*{Description  of   the  dataset}  Continuing   the  example
mentioned in the introduction, we  consider the cookie dough data from
\citet{data_cookies1}.   The  data  with the  corresponding  test  and
training sets  are available  in the \textbf{fds}  \texttt{R} package.
After data pretreatments as  in \citet{data_cookies2}, we have $n=39$
dough  pieces in  the training  set: each  sample consists  in an  NIR
spectrum with $p=256$ points measured from  1380 to 2400 nm (spaced by
4  nm),  and   in  four  quantitative  variables   that  describe  the
percentages in fat, sugar flour and water of the dough piece.

\paragraph*{Structure specification} We would  like to account for the
neighborhood structure between the  predictors which is obvious in the
context of  NIR spectroscopy: since spectrum are  continuous curves, a
smooth neighborhood prior will  encourage predictors to be selected by
``wave'', which seems more  satisfactory than isolated peaks. Thus, we
naturally  define  $\bL$ by  means  of  the  first forward  difference
operator \eqref{eq:first_order_diff}.  We also tested higher orders of
the operator  to induce a stronger  smoothing effect, but  they do not
lead to dramatic changes in term of PE and we omit them.  Order $k$ is
simply obtained  by powering the first order  matrix.  Such techniques
have  been  studied  in  a structured  $\ell_1$-penalty  framework  in
\cite{2009_SIAM_Kim,2011_AOS_Tibshirani}  and is known  as \emph{trend
  filtering}.   Our  approach  is   different,  though:  it  enters  a
multivariate framework  and it is  based on a  smooth $\ell_2$-penalty
coupled with the $\ell_1$-penalty for selection.

\paragraph*{Results}  The  predictive  performances  of  a  series  of
regression  techniques   are  compared  in   Table  \ref{Tab:Cookies},
evaluated on the same test set.
\begin{table}[htbp!]
  \centering
  \begin{small}
    \begin{tabular}{l|rrrr}
      \hline
      \textit{\textsf{Method}} & \textit{\textsf{fat}} & \textit{\textsf{sucrose}} & \textit{\textsf{flour}} & \textit{\textsf{water}} \\
      \hline
      {Stepwise MLR} & .044 & 1.188 & .722 & .221 \\
      {Decision theory} & .076 & .566 & .265 & .176 \\
      {PLS} & .151 & .583 & .375 & .105 \\
      {PCR} & .160 & .614 & .388 & .106 \\
      {Wavelet Regression} & .058 & .819 & .457 & .080 \\
      {LASSO} & .044 & .853 & .370 & .088 \\
      {group-LASSO} & .127 & .918 & .467 & .102 \\
      {MRCE} & .151 & .821 & .321 & .081 \\
      {Structured E-net} & .044 & .596 & .363 & .082 \\
      {SPRING} (CV) & .065 & .397 & .237 & .083 \\
      {SPRING} (BIC)& .048 & .389 & .243 & .066 \\
  \end{tabular}
  \end{small}
  \caption{Prediction error for the cookie dough data.}
  \label{Tab:Cookies}
\end{table}
The first four rows (namely stepwise multivariate regression, Bayesian
decision theory approach, Partial Least Square and Principal Component
Regression) correspond to  calibration methods originally presented in
\citet{data_cookies2};  row  five  (Bayesian  Wavelet  Regression)  is
\citeauthor{data_cookies2}'s original  proposal; the remainder  of the
table is due  to our own analysis.  We observe  that, on this example,
SPRING  achieves  extremely  competitive  results.  The  BIC  performs
notably well as a model selection criterion. 
\begin{figure}[htbp!]
  \centering
  \begin{tabular}{@{}c@{}c@{}c@{}c@{}}
    LASSO & group-LASSO &  Structured Elastic-Net & MRCE \\
    \includegraphics[width=.25\textwidth]{figures/cookies_beta_lasso} & 
    \includegraphics[width=.25\textwidth]{figures/cookies_beta_grplasso} &
    \includegraphics[width=.25\textwidth]{figures/cookies_beta_senet} &
    \includegraphics[width=.25\textwidth]{figures/cookies_beta_mrce} \\
    \multicolumn{4}{c}{Wavelength range (nanometer)}
  \end{tabular}
  \caption{Parameters estimated by the penalized regression methods for
    the cookie data}
  \label{Fig:Cookies2}
\end{figure}
% \begin{figure}[htbp!]
%   \centering
%   \begin{tabular}{@{\hspace{1cm}}cc}
%     LASSO & group-LASSO  \\
%     \includegraphics[width=.29\textwidth]{figures/cookies_beta_lasso} & 
%     \includegraphics[width=.29\textwidth]{figures/cookies_beta_grplasso} \\
%     Structured Elastic-Net & MRCE \\
%     \includegraphics[width=.29\textwidth]{figures/cookies_beta_senet} &
%     \includegraphics[width=.29\textwidth]{figures/cookies_beta_mrce} \\
%     \multicolumn{2}{c}{Wavelength range (nanometer)}
%   \end{tabular}
%   \caption{Parameters estimated by the penalized regression methods for
%     the cookie data}
%   \label{Fig:Cookies2}
% \end{figure}
Figure \ref{Fig:Cookies2}  shows the regression  coefficients adjusted
with  the  penalized regression  techniques:  apart  from LASSO  which
selects very isolated  (and unstable) wavelengths, non-zero regression
coefficients  are very spread,  and therefore  hard to  interpret.  As
expected,  the  multitask group-Lasso  activates  the same  predictors
across the  responses, which is  not a good  idea when looking  at the
predictive performance in Table \ref{Tab:Cookies}.  On the other hand,
back to  the beginning of the paper  in Figure~\ref{Fig:Cookies1}, the
direct effects  selected by SPRING with BIC  define predictive regions
specific of  each response which are well  suited for interpretability
purpose.

%%% Local Variables:
%%% TeX-master: "JST_AOAS_main.tex"
%%% End:


==> arxiv_version/.svn/text-base/v1/application_linkage.tex <==
\subsection{Multi-trait Genomic Selection in Brassica napus}

\paragraph{Context} Genomic selection aims at predicting  one or several phenotypes 
based on the information of genetics markers. In plant and animal
genetics,  deriving an  accurate prediction  of complex  traits  is of
major importance for the  early detection and selection of individuals
of  high   genetic  value.  Due   to  the  continued   advancement  of
high-throughput   genotyping  and  sequencing   technologies,  genetic
information is now  available at low cost, whereas acquiring  trait  information  remains expensive. A
typical experiment will only contain a few hundreds
of  phenotyped  individuals genotyped for thousands of markers.
% in the  form of thousands of markers
% On  the  other  hand, acquiring  trait  information  remains
%expensive, and a  typical experiment will only contain  a few hundreds
%of  phenotyped  individuals.
% This  leads to the  classical ``high  dimensional setting''  where the
% number  of features  is much  higher than  the number  of observations
% available for training.  Due to this high dimensional
% setting,
Consequently regularization methods such  as ridge or Lasso regression
or  their Bayesian  counterparts  have been  proposed  since the  very
beginning  of  genomic selection  \citep{LosCampos12}.  Still, in  most
studies only  single trait genomic selection  is performed, neglecting
correlations  between  phenotypes%    and  leading  to  poor  prediction
% performance
.   Moreover,  little attention  has  been  devoted to  the
development   of  regularization   methods  including   prior  genetic
knowledge.

\paragraph*{Description of the dataset} We consider the \emph{Brassica
  napus}     dataset    described    in     \citet{Bnapus_data}    and
\citet{Bnapus_map}.   Data consists  in  $n=103$ double-haploid  lines
derived from 2 parent cultivars,  `Stellar' and `Major', on which $p =
300$ genetic markers and  $q=8$ traits (responses) were recorded. Each
marker is a 0/1 covariate with $x_i^j=0$ if line $i$ has the 'Stellar'
allele  at marker $j$,  and $x_i^j=1$  otherwise. Traits  included are
percent winter survival  for 1992, 1993, 1994, 1997  and 1999 (surv92,
surv93, surv94,  surv97, surv99, respectively), and  days to flowering
after no vernalization (flower0), 4 weeks vernalization (flower4) or 8
weeks vernalization (flower8).

\paragraph{Structure specification} 
In a biparental line population, correlation between 2 markers depends
on their genetic distance defined  in terms of recombination fraction.
As a consequence,  one expects adjacent markers on the  sequence to be
correlated, yielding similar direct  relationships with the phenotypic
traits. Noting $d_{12}$ the genetic distance between markers $M_1$ and
$M_2$, one has $\text{cor}(M_11,M_22)  = \rho^{d_{12}}$, where $\rho =
.98$\footnote{This value  directly arises  from the definition  of the
  genetic  distance itself.}.   The covariance  matrix $\bL^{-1}$  can
hence  be  defined  as  $\bL_{ij}^{-1}  =  \rho^{d_{ij}}$.   Moreover,
assuming recombination events are  independent between $M_1$ and $M_2$
on one hand, and $M_2$ and $M_3$  on the other hand, one has $d_{13} =
d_{12} + d_{23}$ and matrix $\bL^{-1}$ exhibits an inhomogeneous AR(1)
profile.  As a consequence, $\bL$ is tridiagonal with general elements
\begin{eqnarray*}
  w_{i, i} & = & \frac{1 - \rho^{2d_{i-1, i} + 2d_{i, i+1}}}{(1 - \rho^{2d_{i-1, i}})(1 - \rho^{2d_{i, i+1}})}, \\
  w_{i, i+1} & = & \frac{-\rho^{d_{i, i+1}}}{1 - \rho^{2d_{i, i+1}}}
\end{eqnarray*}
and $w_{i,j} =  0$ if $|i-j| > 1$. For the  first (resp. last) marker,
the distance $d_{i-1, i}$ (resp. $d_{i, i+1}$) is infinite.

\paragraph{Results}  We apply SPRING  to study  the influence  of each
marker on the traits and compare its predictive performance with these
of its competitors.   PE is estimated by randomly  splitting the $103$
samples  into training  and test  sets with  sizes 93  and  10. Before
adjusting the models, we first  scale the outcomes on the training and
test sets  to facilitate interpretability.  Five-fold cross-validation
is  used on the  training set  to choose  the tuning  parameters.  Two
hundred random samplings of the  test and training sets were conducted
to estimate the PE given in Table \ref{Tab:BNapus}.
\begin{table*}[htp!]
  \centering
  \begin{small}
    \begin{tabular}{l|rrrrr}
    \hline
    \textit{\textsf{Method}} &
    \textit{\textsf{surv92}}  &
    \textit{\textsf{surv93}}  &
    \textit{\textsf{surv94}}  &
    \textit{\textsf{surv97}}  &
    \textit{\textsf{surv99}} \\
    \hline
    {LASSO} & .730 (.011) & .977 (.009) & .943 (.010) & .947 (.009) & .916
    (.010) \\

    {S. Enet}  & \textbf{.697} (.011) &  .987 (.009) & .941  (.011) & .945
    (.009) & .911 (.010) \\

    {MRCE} & .759 (.010)  & \textbf{.919} (.003) & 917 (.006) & \textbf{.924} (.004) & .926
    (.006) \\

    {SPRING} &  .724 (.010) &  .948 (.008) & \textbf{.848}  (.010) & .940  (.006) &
    \textbf{.907} (.009) \\
  \end{tabular}
  \medskip

  \begin{tabular}{l|rrr}
    \hline
    \textit{\textsf{Method}} &
    \textit{\textsf{flower0}} &
    \textit{\textsf{flower4}} &
    \textit{\textsf{flower8}} \\
    \hline
    {LASSO} & .609 (.011) & .501 (.011) & .744 (.011) \\

    {S. Enet} & .577 (.011) & .478 (.010) & .727 (.012) \\

    {MRCE} & .591 (.011) & .479 (.011) & .736 (.011) \\

    {SPRING} & \textbf{.489} (.010) & \textbf{.419} (.009) & \textbf{.616} (.012) \\
  \end{tabular}

  \end{small}
  \caption{Estimated  prediction error  for the  \emph{Brassica napus}
    data (standard error in parenthesis)}
  \label{Tab:BNapus}
\end{table*}
All  methods  provide similar  results  although  SPRING provides  the
smallest  error   for  half   of  the  traits.    A  picture   of  the
between-response covariance  matrix estimated with SPRING  is given in
Figure \ref{Fig:BNapusCovar}.   In this context,  this matrix reflects
the correlation  between the  traits that are  either explained  by an
unexplored  part  of the  genotype,  by  the  environment or  by  some
interaction  between the two.   The residuals  of the  flowering times
exhibit  strong  correlations,  whereas  the correlation  between  the
survival rates are weak. It also shows that the survival traits have a
larger residual  variability than  the flowering traits,  suggesting a
higher sensitivity to environmental conditions.
\begin{figure}[htpb!]
  \includegraphics[scale=.35]{figures/brassica_cor}
  \caption{Brassica study: residual covariance estimation \label{Fig:BNapusCovar}}
\end{figure}

We  then  turn  to  the  effects  of  each  marker  on  the  different
traits. The left panels of Figure \ref{Fig:BNapusCoefs} gives both the
regression  coefficients (top)  and the  direct effects  (bottom). The
gray zones correspond  to chromosomes 2, 8 and  10, respectively.  The
exact location  of the markers within these  chromosomes are displayed
in the right panels, where the  size of the dots reflects the absolute
value of the  regression coefficients (top) and of  the direct effects
(bottom).
\begin{figure*}[htbp!]
   \centering
   \includegraphics[width=\textwidth]{figures/brassica_fits}
   \caption{Brassica Study: direct and indirect genetic effects of the
     markers on the  traits estimated by SPRING\label{Fig:BNapusCoefs}
     (better seen in color).}
\end{figure*}
The  interest of  considering  direct effects  rather than  regression
coefficients appears  clearly here, looking for  example at chromosome
2.  Three  large overlapping regions  are observed in  the coefficient
plot, for each flowering trait. A straightforward interpretation would
suggest that  the corresponding region controls  the general flowering
process. The  direct effect  plot allows to  go deeper and  shows that
these  three  responses are  actually  controlled  by three  separated
sub-regions within  this chromosome. The confusion  in the coefficient
plot only  results from the  strong correlations observed  between the
three flowering traits.

%%% Local Variables:
%%% TeX-master: "JST_AOAS_main.tex"
%%% End:


==> arxiv_version/.svn/text-base/v1/application_motif.tex <==
\subsection{Selecting regulatory motif from multiple microarrays}

\paragraph{Context} In genomics, the  expression of genes is initiated
by transcription factors that bind to the DNA upstream from the coding
regions, called {\it regulatory  regions}.  This binding occurs when a
given   factor   recognizes   a   certain  (small)   sequence   called
transcription  factor binding  site  or {\it  regulatory motif}.   The
presence of a  regulatory motif in the regulatory region  of a gene is
therefore   required   to   launch  the   transcriptional   machinery.
Conversely, genes  hosting the same  regulatory motif will  be jointly
expressed under certain conditions.  As the binding relies on chemical
affinity, some degeneracy can be tolerated in the motif definition and
motifs similar  up to small  variations may share the  same functional
properties \citep[see, e.g.][]{2012_GB_Lajoie}.

We  are interested  in the  detection of  such regulatory  motifs, the
presence of  which controls genes  expression profile. To this  aim we
try to establish a relation between  the expression level of all genes
across a  series of  conditions with the  content of  their respective
regulatory regions in terms of motifs. In this context, we expect $i)$
the set  of influential motifs to  be small for each  condition, $ii)$
the influent motifs  for a given condition to  be degenerated versions
of each other,  and $iii)$ the expression under  similar conditions to
be controlled by the same motifs.

\paragraph*{Description of the  dataset} In \cite{gasch2000genomic}, a
series  of  microarray  experiments   are  conducted  on  yeast  cells
(\textit{Saccharomyces cerevisae}).   Among these assays,  we consider
12  time-course  experiments profiling  $n=5883$  genes under  various
environmental  changes as  listed in  Table \ref{tab:exp_time_course}.
These expression sets form  12 potential response matrices $\bY$ whose
number of column corresponds to the number of time points.
\begin{table}[htbp!]
  \centering
  \begin{tabular}{lc|c@{\hspace{2.5em}}c@{\hspace{2.5em}}c}
    \textit{Experiment}     &     \textit{\#     time    point}     &
    \multicolumn{3}{c}{\it \# motifs selected by SPRING} \\
    \cline{3-5} 
    & & $k=7$ & $k=8$ & $k=9$ \\
    \hline 
    Heat shock & 8 & 30 & 68 & 43 \\
    Shift from 37\degres to 25 \degres C & 5 & 3 & 11 & 33 \\
    Mild Heat shock & 4 & 24 & 13 & 23 \\
    Response to $\text{H}_2 \text{O}_2$ & 10 & 15 & 10 & 21 \\
    Menadione Exposure & 9 & 16 & 1 & 7 \\
    DDT exposure 1 & 8 & 15 & 10 & 30 \\
    DDT exposure 2 & 7 & 11 & 33 & 21 \\
    Diamide treatment & 8 & 45 & 25 & 35 \\
    Hyper-osmotic shock & 7 & 36 & 24 & 15 \\
    Hypo-osmotic shock & 5 & 20 & 8 & 29 \\
    Amino-acid starvation & 5 & 47 & 30 & 39 \\
    Diauxic Shift & 7 & 16 & 14 & 20 \\
    \hline 
    \multicolumn{2}{l}{\it total number of unique motif inferred} & 87 & 82 & 72 \\
  \end{tabular}
  \caption{Time-course data from \cite{gasch2000genomic} considered for regulatory motif discovery}
  \label{tab:exp_time_course}
\end{table}
Concerning  the predictors,  we consider  the set  of all  motifs with
length  $k$  formed with  the  four  nucleotides,  that is  $\clM_k  =
\set{A,C,G,T}^k$.  There are $p =  |\clM_k| = 4^k$ such motifs. Unless
otherwise stated, the motifs in $\clM$ are lined up in lexicographical
order e.g.,  when $k=2$,  $AA,AC,AG,AT,CA,CC,\dots$ and so  on.  Then,
the $n\times p$ matrix of  predictors $\bX$ is filled such as $X_{ij}$
equals the occurrence  count of motif $j$ in  the regulatory region of
gene $i$.%  This can be  straightforwardly done using the FASTA files of
% the regulatory region of each gene which are publicly available on the
% web.

\paragraph{Structure  specification} As  we expect  influential motifs
for a  given condition  to be degenerated  versions of each  other, we
would  like  to take  this  information  into  account in  the  matrix
$\bL$.  To do  so, we  first measure  the similarity  between  any two
motifs from $\clM_k$ with the Hamming defined as
\begin{equation*}
 \label{eq:hamming_def}
 \forall a,b\in\clM_k, \quad \mathrm{dist}(a,b) = \text{card}\{i:a_i\neq b_i\}.
\end{equation*}
For a distance of interest $0\leq\ell\leq k$, we further define the $m
\times              m$             \emph{symmetric}             matrix
$\bD^{k,\ell}=(d^{k,\ell}_{ab})_{a,b\in\clM_k}$   so  as   each  entry
$d^{k,\ell}_{ab}$ indicates  if the Hamming distance is  less or equal
to $\ell$. We refer to this  distance for fixed value of $\ell$ as the
\textit{$\ell$-distance matrix}:
\begin{equation*}
 \label{eq:distance_matrix}
 \forall a,b\in\clM_k, \quad d^{k,\ell}_{ab} = \left\{
 \begin{array}{ll}
 1 & \text{if $\mathrm{dist}(a,b) \leq \ell$} \\
 0 & \text{otherwise.} \\
 \end{array}\right.
\end{equation*}

For motifs in $\clM_k$ lined up in lexicographical order, manipulation
of $\bD$  greatly simplifies  as motifs  can be mapped  to the  set of
natural integers  $\mathbb{N}$.  The following  proposition shows that
$\bD^{k,\ell}$ can  be computed  recursively for increasing  values of
$k,\ell$ at the cost of a simple Kronecker product.
\begin{proposition} \label{prop:computeDkl}
For $\ell\leq k$, and considering that
\begin{equation*}
 \label{eq:D10_D11}
 \bD^{1,0} =
 \kbordermatrix{
 & A & C & G & T \\
 A & 1 & & & \\
 C & & 1 & & \\
 G & & & 1 & \\
 T & & & & 1 \\
 }, \quad
 \bD^{1,1} =
 \kbordermatrix{
 & A & C & G & T \\
 A & 1 & 1 & 1 & 1 \\
 C & 1 & 1 & 1 & 1 \\
 G & 1 & 1 & 1 & 1 \\
 T & 1 & 1 & 1 & 1 \\
 },
\end{equation*}
then the  $\ell$-distance matrix between  motifs of size $k+1$  can be
expressed as a function of distance between motifs of size $k$ as
 \begin{equation*}
 \label{eq:reck_D}
 \bD^{{k+1},\ell} = \left(\bD^{1,0}\otimes\bD^{k,\ell}\right) \vee
 \left(\bD^{1,1}\otimes\bD^{k,\ell-1}\right),
 \end{equation*}
 where $\vee$ is the OR operator and $\ell\geq 1$. Similarly, for
 values of $\ell:\ell+1\leq k$,
 \begin{equation*}
 \label{eq:recl_D}
 \bD^{k,\ell+1} = \left(\bD^{1,0}\otimes\bD^{k-1,\ell}\right) \vee
 \left(\bD^{1,1}\otimes\bD^{k,\ell}\right).
 \end{equation*}
\end{proposition}

$\bD^{k,\ell}$ can be viewed as the  adjacency matrix of a graph where
the nodes are the motifs and where  an edge is present between 2 nodes
when the 2 motifs  are at a Hamming distance less  or equal to $\ell$.
We finally  use the Laplacian  of this  graph as a  structuring matrix
$\bL^{k,\ell}=(\ell^{k,\ell}_{ab})_{a,b\in\clM_k}$, that is
\begin{equation}
 \label{eq:laplacian}
 \ell^{k,\ell}_{ab} =
 \begin{cases}
 \sum_{c\in\clM_k} d^{k,\ell}_{ac} & \text{if } a = b, \\
 -1 & \text{if } d^{k,\ell}_{ab} = 1, \\
 0 & \text{otherwise}.
 \end{cases}
\end{equation}
{Note that we came across a similar proposal by \cite{li2010learning}
  in the context of sparse, structured PLS. The derivation is
  different though, and the objective of this method is not the
  selection of motifs but of family of motifs via the compression
  performed by the PLS.  }

\paragraph{Results}~  We apply  our methodology  for candidate  motifs
from  $\clM_7,\clM_8$ and  $\clM_9$, which  result in  three lists  of
putative motifs having a direct effect on gene expression.  Due to the
very large  number of potential  predictors that comes with  a sparser
matrix $\bX$  when $k$  increases, we first  perform a  screening step
that keep  the $5,000$ motifs  with the highest  marginal correlations
with  $\bY$.   Second,  SPRING  is   fitted  on  each  of  the  twelve
time-course experiments described  in Table \ref{tab:exp_time_course}.
The selection of $(\lambda_1,\lambda_2)$ is  performed on a grid using
the BIC \eqref{eq:pen_crit} rather than the cross-validation approach,
since we clearly face a variable selection problem.  At the end of the
day,   the  three   lists  corresponding   to  $k=7,8,9$   comprehends
respectively 87, 82 and 72 motifs,  for which at least one coefficient
in the associated  row $\widehat{\bOmega}_{\bx\by}(j,\cdot)$ was found
non-null  for some  of the  twelve experiments,  as detailed  in Table
\ref{tab:exp_time_course}.

To assess the relevance of  the selected motifs, we compared them with
the {\tt MotifDB} patterns available in Bioconductor (\cite{motifdb}),
where known transcription factor binding sites are recorded. There are
453 such reference motifs with size varying from 5 to 23 nucleotides.
% \corSR{To account for degeneracy, a SFBS with length $\ell$ is
% represented  as  position-specific   scoring  matrix  ${\bf  P}  =
% [p_{au}]$  with  dimension  $4   \times  \ell$,  where  $p(a,  u)$
% represents the  probability for the  nucleotide $a \in \{A,  C, G,
% T\}$  to occur  at  position $u  \in  \{1, \dots,  \ell\}$ of  the
% binding site. For each selected  motif ${\bf m}_i$ and each JASPAR
% matrix  ${\bf P}_j$  ($j  = 1,  \dots  , 53$),  we calculated  the
% similarity   score  $T_{ij}   =  \max_{0   \leq  u   \leq  \ell-k}
% \sum_{v=1^k}  \log p_j({\bf  m}_i(v), u+v)$.  A  null distribution
% $\widehat{F}_i$ for this score  was then estimated for each matrix
% ${\bf P}_j$, computing  the same score for all  motifs with length
% $k$  present  in the  set  of  regulatory  regions.  We  furthered
% defined     a     pseudo      $p$-value     $P_{ij}$     as     $1
% -\widehat{F}_i(T_{ij})$. }{}
Consider the case  of $k=7$ for instance: among  the 87 SPRING motifs,
62 match one  \texttt{MotifDB} pattern each and 25  are clustered into
11 \texttt{MotifDB} patterns as depicted in Table \ref{Tab:MotifDB}.
\begin{table}
  \begin{center}
    \begin{tabular}{@{}cccc@{}}
      \input{ResMotif-K7.tex}
    \end{tabular}
    \caption{Comparison    of     SPRING    selected    motifs    with
      \texttt{MotifDB}   patterns.   Each   cell  corresponds   to   a
      \texttt{MotifDB}  pattern (top)  compared  to a  set of  aligned
       SPRING motifs with size 7 (down). \label{Tab:MotifDB}}
  \end{center}
\end{table}
As  seen in  this table,  the clusters  of motifs  selected by  SPRING
correspond  to sets  of variants  of  a same  pattern. These  clusters
consist of motifs  that are close according to  the similarity encoded
in  the structure  matrix $\bL$.   In this  example, the  framework we
propose enabled  us to  orient the regression  problem to  account for
motif degeneracy  and helped us  to select motifs that  are consistent
known  binding sites.   This  example illustrates  the flexibility  of
SPRING,  which  allows  to  use  domain-specific  definitions  of  the
structure between the predictors.

% \begin{table}
%   \begin{center}
%     \begin{tabular}{llll}
%       \input{ResMotif-K8.tex}
%     \end{tabular}
%     \caption{Comparison of SPRING selected motifs with MotifDB patterns. Each cell of the table corresponds to a MotifDB pattern (top) compared to a set of aligned SPRING motifs with length 8 (down). \label{Tab:MotifDB}}
%   \end{center}
% \end{table}

% \begin{table}
%   \begin{center}
%     \begin{tabular}{llll}
%       \input{ResMotif-K9.tex}
%     \end{tabular}
%     \caption{Comparison of SPRING selected motifs with MotifDB patterns. Each cell of the table corresponds to a MotifDB pattern (top) compared to a set of aligned SPRING motifs with length 9 (down). \label{Tab:MotifDB}}
%   \end{center}
% \end{table}

%%% Local Variables:
%%% TeX-master: "JST_AOAS_main.tex"
%%% End:


==> arxiv_version/.svn/text-base/v1/crit_learn.tex <==
\subsection{Structured regularization with underlying sparsity}
\label{Sec:crit_learn}

Our regularization scheme starts  by considering some structural prior
information as for the  relationships between the coefficients. We are
typically thinking of a situation where similar inputs are expected to
have  similar direct relationships  with the  outputs. Right  panel of
Figure  \ref{fig:model_insight}   represents  a  cartoon   of  such  a
situation,  where  there  exists  an  extreme  neighborhood  structure
between the  predictors.  This depicts  a pattern that acts  along the
rows of $\bB$ or  $\bOmega_{\bx\by}$ as substantiated by the following
Bayesian point of view.

\paragraph*{Bayesian interpretation}  Suppose the similarities  can be
encoded  into  a  matrix  $\bL$.   Our  aim is  to  account  for  this
information  when learning the  coefficients.  The  Bayesian framework
provides  a  convenient  setup   to  define  the  way  the  structural
information  should  be accounted  for.   In  the  single output  case
\citep[see, e.g.][]{MaR07},  a conjugate  prior for $\bbeta$  would be
$\mathcal{N}(\bzr, \bL^{-1})$.   Combined with the  covariance between
the outputs, this gives
\begin{equation*}
  \vec(\bB) \sim \mathcal{N}(\bzr,\bR \otimes \mathbf{L}^{-1}), 
\end{equation*}
where $\otimes$ is the Kronecker  product. By properties of the $\vec$
operator, % we have
% \begin{multline*}
%   \var(\vec(\bB))  = \var(\vec(-\bOmega_{\bx\by}\bR)) = \var((\bR\otimes\bI_p)\vec(\bOmega_{\bx\by}))\\
%   =
%   (\bR\otimes\bI_p)\var(\vec(\bOmega_{\bx\by}))(\bR\otimes\bI_p)
%   \\ = 
%   (\bR\otimes\bI_p)(\bR^{-1}\otimes\mathbf{L}^{-1})(\bR\otimes\bI_p) = \bR\otimes\mathbf{L}^{-1}.
% \end{multline*}
% Thus the prior on $B$
this can be stated straightforwardly as
\begin{equation*}
  \vec(\bOmega_{\bx\by}) \sim \mathcal{N}(\bzr,\bR^{-1} \otimes \mathbf{L}^{-1})
\end{equation*}
for the direct links. Choosing such a prior results in
\begin{equation*}
  \label{eq:log_lik_prior}
  \log \prob(\bOmega_{\bx\by}|\mathbf{L},\bR) =  
  \frac{1}{2}\trace\left(\bOmega_{\bx\by}^T             \mathbf{L}
    \bOmega_{\bx\by} \bR \right)
  + \mathrm{cst.}
\end{equation*}

\paragraph*{Criterion} Through  this argument, we  propose a criterion
with two  terms to regularize the  conditional negative log-likelihood
\eqref{eq:log_lik}:  first,  a  smooth   trace  term  relying  on  the
available structural information  $\mathbf{L}$; and second, a $\ell_1$
norm that  encourages sparsity  among the direct  links. We  write the
criterion  as  a  function of  $(\bOmega_{\bx\by},  \bOmega_{\by\by})$
rather than $(\bOmega_{\bx\by}, \bR)$,  although equivalent in term of
estimation,  since the  former  leads to  a  convex formulation.   The
optimization problem turns to the minimization of
\begin{multline}
  \label{eq:objective}
  % (\hat{\bOmega}_{\bx\by},\hat{\bOmega}_{\by\by})
  % = \argmin_{\bOmega_{\bx\by},\bOmega_{\by\by}} J(\bOmega_{\bx\by},\bOmega_{\by\by}),
  % \quad \text{where }
  J(\bOmega_{\bx\by},\bOmega_{\by\by})        = \\      -\frac{1}{n}\log
  L(\bOmega_{\bx\by},\bOmega_{\by\by})      +      \frac{\lambda_2}{2}
  \trace\left(\bOmega_{\by\bx}\mathbf{L}\bOmega_{\bx\by}\bOmega_{\by\by}^{-1}\right)
  + \lambda_1 \|\bOmega_{\bx\by}\|_1.
\end{multline}
Simple  convexity arguments and requirements for positive definiteness of the Hessian of
\eqref{eq:objective} lead to the following proposition, whose proof is
omitted.

\begin{proposition}\label{prop:existence_uniqueness} The objective
  function     \eqref{eq:objective}    is     jointly     convex    in
  $(\bOmega_{\bx\by},\bOmega_{\by\by})$ and admits at least one global
  minimum  which  is  unique  when  $n\geq  q$  and  $(\lambda_2\bL  +
  \bS_{\bx\bx})$ is positive definite.
\end{proposition}

%  \begin{proof}   Thanks  to  the   convexity  of  \eqref{eq:log_lik}
%   \citep[see][]{2012_arxiv_yuan} combined  with the two regularizers
%   which are convex norms,  \eqref{eq:objective} is jointly convex in
%   $(\bOmega_{\bx\by},\bOmega_{\by\by})$ when $(\lambda_1,\lambda_2)$
%   are fixed, which means that a global minimum exists.

%   In fact,  as soon as  $(\lambda_2\bL + \bS_{\bx\bx})$  is positive
%   definite and  $n\geq q$, it is  not difficult to  see, although we
%   omit the details, that the problem is strictly convex and thus the
%   solution to \eqref{eq:objective} is unique.
% \end{proof}

% Introducing   the  notation  $   \hat{\bSigma}_{\bx\bx}^{\lambda_2}  =
% \bS_{\bx\bx}+ \lambda_2\bL$, this writes
% \begin{multline}
%   \label{eq:objective}
%   J(\bOmega_{\bx\by},\bOmega_{\by\by})               =               -
%   \frac{1}{2}\log\left|\bOmega_{\by\by}\right| +
%   \frac{1}{2}\trace\left(\bS_{\by\by} \bOmega_{\by\by} \right) \\
%   +     \trace\left(     \bS_{\bx\by}\bOmega_{\by\bx}    \right)     +
%   \frac{1}{2}\trace\Big(\bOmega_{\by\bx}
%   \hat{\bSigma}_{\bx\bx}^{\lambda_2}                   \bOmega_{\bx\by}
%   \bOmega_{\by\by}^{-1}\Big) + \lambda_1 \|\bOmega_{\bx\by}\|_1,
% \end{multline}
% which gives  additional insights about  the effect of  the structuring
% prior:  it  performs  a   mixture  between  the  empirical  covariance
% $\bS_{\bx\bx}$  and the structure  $\bL$ similar  to this  obtained in
% Bayesian linear  regression.

\subsection{Connection to other sparse regression methods}

To get more insight about our model and to facilitate connections with
existing   approaches,  we   shall   write   the  objective   function
\eqref{eq:objective}  as  a   penalized  \emph{univariate}  regression
problem.       This      amounts      to      ``vectorize''      model
\eqref{eq:cond_model_mat} with respect to $\bOmega_{\bx\by}$, i.e., to
write  the objective  as  a  function of  $(\bomega,\bOmega_{\by\by})$
where  $\bomega=\vec(\bOmega_{\bx\by})$.    This  is  stated   in  the
following  proposition,  which  can be  derived  from  straightforward
matrix algebra,  as proved in Appendix  Section \ref{sec:vec_obj}. The
main interest of this proposition  will become clear when deriving the
optimization  procedure  to   minimize  \eqref{eq:objective},  as  the
optimization  problem  when $\bOmega_{\by\by}$  is  fixed  turns to  a
generalized Elastic-Net  problem.  Remark  that we use  $\bA^{1/2}$ to
denote  the square  root  of  a matrix,  obtained  for  instance by  a
Cholesky  factorization  in  case  of a  symmetric  positive  definite
matrix.
\begin{proposition} \label{prop:vec_obj} \hspace{-2ex} Let $\bomega =
  \vec(\bOmega_{\bx\by})$.    An    equivalent    vector    form    of
  \eqref{eq:objective} is
  \begin{multline*}
    \label{eq:objective_vec}
    J(\bomega,      \bOmega_{\by\by})     =      -\frac{1}{2}     \log
    |\bOmega_{\by\by}|   +    \frac{1}{2   n}   \left\|\tilde{\by}   +
      \tilde{\bX} \bomega
    \right\|_2^2  +  \frac{\lambda_2}{2}  \bomega^T  \left(\bOmega_{\by\by}^{-1}  \otimes  \bL
    \right) \bomega + \lambda_1 \left\| \bomega \right\|_1,
  \end{multline*}
  where the $n\times q$ dimensional vector $\tilde{\by}$ and the $n q
  \times p q$ dimensional matrix $\tilde{\bX}$ depends on
  $\bOmega_{\by\by}$ such that
  \begin{equation*}
    \tilde{\by} = \vec(\bY  \bOmega_{\by\by}^{1/2}), \quad \tilde{\bX} =
    \left(\bOmega_{\by\by}^{-1/2} \otimes \bX\right).
  \end{equation*}
\end{proposition}

When  there  is  only  one  response,  that  is,  when  $q=1$,  direct
connections  can be  made with  various existing  approaches. In  such
cases,   the  variance-covariance   matrix  $\bR$   and  its   inverse
$\bOmega_{\by\by}$ turn to scalars, respectively denoted by $\sigma^2$
and    $\rho^2$,   with    $\sigma=1/\rho$.    Applying    Proposition
\ref{prop:vec_obj}, the objective \eqref{eq:objective} writes
\begin{equation}
  \label{eq:criteria_univariate}
  J(\bomega, \rho) = -\log(\rho) + \frac{1}{2n}\|\rho \by +
  \bX \bomega/(\rho)\|_2^2 + \frac{\lambda_2}{2\rho^2} \bomega^T 
  \bL  \bomega  +  \lambda_1  \|\bomega\|_1.
\end{equation}
Its  counterpart  in term  of  the parametrization  $(\bbeta,\sigma)$,
% where $\bbeta = -\bomega \sigma^2 = -\bomega/(\rho^2)$
is
\begin{equation}
  \label{eq:criteria2_univariate}
  J(\bbeta,\sigma) =             \log(\sigma)             +
  \frac{1}{2n\sigma^2}\left\|\by-\bX\bbeta       \right\|_2^2      +
  \frac{\lambda_2}{2\sigma^2}             \bbeta\bL\bbeta            +
  \frac{\lambda_1}{\sigma^2} \|\bbeta \|_1.
\end{equation}
We recognize in  \eqref{eq:criteria2_univariate} the log-likelihood of
a  ``usual''  linear  model  with  Gaussian  noise,  unknown  variance
$\sigma^2$  and  regression parameters  $\bbeta$,  plus  a mixture  of
$\ell_1$ and $\ell_2$ norm,  a.k.a, an elastic-net penalization.  This
is the univariate analog  of \eqref{eq:reg_model_row}, whose criterion
\eqref{eq:criteria_univariate}   is   the   convex   reparametrizaton.
Criterion  \eqref{eq:criteria2_univariate} entail  many regularization
schemes found in  the literature: assuming that $\sigma$  is known, we
recognize   ridge    regression   when   $\lambda_1=0$,    the   Lasso
\citep{1996_JRSSB_tibshirani} when $\lambda_2=0$, plus the Elastic-Net
\citep{2005_JRSS_Zou}   when  $\bL   =  \bI_p$   and  its   extensions
\citep{2010_AOAS_slawski,2011_EJS_Hebiri}    which    correspond    to
different choices of $\bL$.  Some  natural choices for $\bL$ motivated
by applications  in genetics, genomics and  spectroscopy are discussed
in Sections \ref{Sec:simu} and \ref{Sec:applications}.  If $\sigma$ is
unknown,  letting   $\lambda_2=0$  in  \eqref{eq:criteria2_univariate}
leads to  the $\ell_1$-penalized mixture regression  model proposed by
\citet{2010_Test_Stadler},  where  both  $\bbeta$ and  $\sigma^2$  are
inferred.  In this work,  \citeauthor{2010_Test_Stadler} insist on the
importance of penalizing the vector  of coefficients by an amount that
is  inversely proportional  to  $\sigma$.   Penalizing the  regression
coefficients  and the  small  variances  $\sigma^2$ simultaneously  is
indeed highly desirable, which has  some connections with the Bayesian
Lasso of \citet{2008_JASA_Park}.

To sum-up, our approach can be seen as a generalization of all these
methods  to   the  multiple-responses  case,  not   to  mentioned  the
structured regularization brought by the $\ell_2$-norm.

%%% Local Variables:
%%% TeX-master: "JST_AOAS_main.tex"
%%% End:


==> arxiv_version/.svn/text-base/v1/intro.tex <==
\section{Introduction}

Multivariate regression,  that is,  regression with  multiple response
variables, is increasingly used to model high dimensional problems. By
considering multiple  responses, we wish to  strengthen the estimation
and/or  the  selection  of  the relevant  input  features,  by  taking
advantage  of the  dependency  pattern between  the  outputs. This  is
particularly appealing when the data is scarce, or even in the '$n<p$'
high dimensional setup, in which framework this work enters.  Compared
to  its  univariate counterpart,  the  general  linear model  aims  to
predict several -- say $q$ --  responses from a set of $p$ predictors,
relying on a training data set $\set{(\bx_i,\by_i)}_{i=1,\dots,n}$:
\begin{equation}
  \label{eq:reg_model_row}
  \by_i      =     \bB^T      \bx_i     +      \bvarepsilon_i,     \quad
  \bvarepsilon_i\sim\mathcal{N}(\bzr,\bR), \quad \forall i=1,\dots,n.
\end{equation}
The  $p\times  q$  matrix  of  regression coefficients  $\bB$  and  the
$q\times   q$  covariance   matrix   $\bR$  of   the  Gaussian   noise
$\bvarepsilon_i$ are unknown.
% \old{Note  that we omit  the intercept term    and     center    the    data     for    clarity.}     
Model \eqref{eq:reg_model_row}  has been studied  by \citet{MV_mardia}
in the low dimensional case  where both ordinary and generalized least
squares estimators of $\bB$ coincide and do not depend on $\bR$. These
approaches  boil down  to  perform $q$  independent regressions,  each
column $\bB_j$  describing the weights associating  the $p$ predictors
to the $j$th  response.  In the $n<p$ setup  however, these estimators
are not defined.

The present work proposes  a general multivariate regression framework
suited to  the high dimensional  setup with three purposes  that shall
ease the  learning task: $i)$  We want  to account for  the dependency
structure between the outputs, if it  exists.  That is to say, we want
to integrate the estimation of  $\bR$ in the inference process.  $ii)$
In order to improve interpretability, we  pay a prior attention to the
direct links  between predictors and responses.   Indeed, according to
the Gaussian  graphical models (GGM),  direct effects are  measured by
partial   covariances  between   predictors  and   responses  (denoted
$\bOmega_{\bx\by}$ hereafter), and not  by the regression coefficients
$\bB$.   In   this  regard,   as  few   predictors  are   expected  to
\textit{directly}  influence  each  response,   we  choose  to  induce
sparsity on partial  covariances at once.  $iii)$ We want  to have the
possibility   of  integrating   some  prior   information  about   the
predictors. Indeed, in many applications  such as genomics or spectral
data  analysis,  the  predictors  display  a  structure  (e.g.   their
position along  the genome) and  their influence on the  responses are
likely to display the same structure.

We design  a new estimator  to achieve the three  aforementioned goals
that  we  call  SPRING  (\emph{``Structured  selection  of  Primordial
  Relationships IN  the General  linear model''}).  To  illustrate the
features of  SPRING, we  consider as a  motivating example  the cookie
dough   data from  \cite{data_cookies1}:   in  this   typical  multivariate
regression   problem,  four  continuous   responses  related   to  the
composition of biscuits (percentages of fat, sucrose, flour and water)
may be  linearly explained by predictors  corresponding to reflectance
spectroscopy   measurements.    Parameters   fitted  by   SPRING   are
represented on Figure~\ref{Fig:Cookies1} with, from left to right, the
estimators  of  the  regression  coefficients $\bB$,  of  the  direct
effects $\bOmega_{\bx\by}$ and of the residual covariance $\bR$.
%
\begin{figure*}[tbp!]
  \centering
  \begin{tabular}{@{}c@{}c@{}c@{}c}
    &  $\hat{\bB}$   (indirect  effects)  &  $-\hat{\bOmega}_{\bx\by}$ (direct effects) & $\hat{\bR}$ \\
    \includegraphics[width=.08\textwidth,clip=true,trim=0 -5cm 0 0]{figures/cookies_legend}
    & \includegraphics[width=.3\textwidth]{figures/cookies_beta_spring}
    & \includegraphics[width=.3\textwidth]{figures/cookies_omega_spring}
    & \includegraphics[width=.3\textwidth]{figures/cookies_covariance}\\
    & \multicolumn{2}{c}{wavelength range (nanometer)} & \\
  \end{tabular}
  \caption{Parameters estimated  by SPRING for the  cookies dough data
    (better    seen    in    color).   {Since    $\hat{\bB}$    and
      $\hat{\bOmega}_{\bx\by}$ are  opposite in sign in  our model, we
      represent $-\hat{\bOmega}_{\bx\by}$  to ease the  comparison between
      direct and indirect effects.}}
  \label{Fig:Cookies1}
\end{figure*}
%
The  regression coefficients  show no  sparsity pattern  but  a strong
spatial structure  along the spectrum, characterized  by waves induced
by  a smooth  first order  difference prior.   Concerning  a potential
structure between the outputs, we identify interesting regions where a
strong correlation between  the responses induces correlations between
the regression coefficients.  Consider  for instance positions 1750 to
2000:  the regression  parameters related  to 'dry-flour'  are clearly
anti-correlated  with  those   related  to  'sucrose'.
% \old{,  which  is confirmed  by  the  corresponding  entry  in  $\hat{\bR}$  ($\approx-0.5$)}
Still, we cannot  distinguish {in} $\hat{\bB}$ for a  direct effect of
this  region on  either  the  flour or  sucrose  composition.  Such  a
distinction  is achieved  on  the middle  panel  where direct  effects
$\hat{\bOmega}_{\bx\by}$  selected by SPRING  are plotted:  it defines
sparse predictive regions  specific to each response, where  it is now
obvious  that region 1750  to 2000  is rather  linked to  the sucrose.
This  example   continues  latter,  and  also   illustrates  the  good
predictive performance of SPRING.

The outline of the paper is as follows.  In Section \ref{Sec:model} we
expose  the statistical  model and  the associated  learning strategy:
first,  we  introduce  the   multivariate  regression  model  and  the
parametrization retained.   Second, we propose a  penalized likelihood
criterion   to  regularized   the   model  according   to  the   three
aforementioned  goals.   Then  we develop  an  efficient  optimization
strategy to minimize  this criterion.  A paragraph  also addresses the
model  selection  issue.   Section   \ref{Sec:simu}  is  dedicated  to
illustrative simulation  studies.  In  Section \ref{Sec:applications},
we  develop  further the  cookie  dough  example and  investigate  two
multivariate  problems:  first,   the  relationships  between  genetic
markers and a series of phenotypes of the plant \emph{Brassica napus};
and second, the regulatory motifs  discovery of yeast from time-course
microarray  experiments. In  theses applications,  specific underlying
structuring  priors  arise,  whose  integration within  our  model  is
detailed.

\paragraph*{Links to  related works} Several recent  papers tackle the
multivariate  regression problem  with  penalties-based approaches  by
including  the  dependency pattern  of  the  outputs  in the  learning
process.  When  this pattern  is known \emph{a  priori}, we  enter the
``multitask'' framework  where many authors suggested  variants of the
$\ell_1$-penalty  shaped  accordingly.    A  natural  approach  is  to
encourage a  similar behavior of the regression  parameters across the
outputs -- or  tasks -- using group-norms zeroing a  full row of $\bB$
at    once,    across    the    corresponding    outputs    \citep[see
e.g.][]{2011_SC_Chiquet,2011_AOS_Obozinski}.    Refinements  exist  to
cope  with   complex  dependency  structures,  using   graph  or  tree
structures   \citep{2009_PLOS_kim,2010_ICML_kim},   yet  the   pattern
remains  fixed.   When  it   is  unknown,  the  general  linear  model
\eqref{eq:reg_model_row} is a natural tool to account for dependencies
between        the       responses.         In        this       vein,
\citet{2010_JCGS_rothman,2011_AoAS_yin}   suggest   to  penalize   the
negative  log-likelihood of  \eqref{eq:reg_model_row} by  two $\ell_1$
norms  respectively inducing sparsity  on the  regression coefficients
$\bB$ and  on the  inverse covariance $\bR^{-1}$.   {However their
  criterion is hard to minimize  as it is only bi-convex.  Theoretical
  guarantees are proposed in \citet{,2012_JMA_lee}, accompanied with a
  two-stage  procedure involving a  plug-in estimator of  the inverse
  covariance, which leads to an optimization procedure computationally
  less    demanding.}    In    \citet{2012_JMLR_sohn},    an   elegant
re-parametrization of \eqref{eq:reg_model_row} is depicted, leading to
a formulation  that is jointly convex  and enjoys features  of the GGM
approach.  {\citet{2012_arxiv_yuan}  recently proposed theoretical
  analysis   of   this  model.}    In   this   paper,   we  build   on
\citeauthor{2012_JMLR_sohn}'s   parameterization   yet   we  adopt   a
different  stance regarding  the  regularization, both  on the  output
structure and  on the regression parameters.   SPRING induces sparsity
on  the direct  relationships like  in \citet{2012_JMLR_sohn},  yet no
sparsity  assumption  is  made  for  the  inverse  covariance,  as  we
typically assume a reasonable number of outputs compared to the number
of predictors and sample size.  This leads to a different optimization
strategy,  a   different  estimator  for  the   covariance  $\bR$  and
eventually of  the regression  parameters $\bB$.  On  top of  that, we
include structural  information via an  additional regularization term
using  an application-specific  metric, generalizing  the 'structured'
versions of  the Elastic-net \citep{2010_AOAS_slawski,2011_EJS_Hebiri}
proposed  in  the   univariate-output  case.   Indeed,  an  additional
originality of  our work is  to investigate deeply the  integration of
such structural  information in the various  contexts of spectroscopy,
genomic selection and regulatory  motif discovery, by constructing our
regularization scheme from each application specificity.

%%% Local Variables:
%%% TeX-master: "JST_AOAS_main.tex"
%%% End:


==> arxiv_version/.svn/text-base/v1/optim.tex <==
\subsection{Optimization}
\label{Sec:optim}

To minimize  the objective, we  rely on a simple  strategy alternating
the  optimization on  $\bOmega_{\by\by}$ and  $\bOmega_{\bx\by}$, that
is,
\begin{subequations}
  \begin{equation}
    \label{eq:optim_cov}
    \hat{\bOmega}_{\by\by}^{(k+1)} = \argmin_{\bOmega_{\by\by}\succ 0}
    J_{\lambda_1\lambda_2}(\hat{\bOmega}_{\bx\by}^{(k)}, \bOmega_{\by\by}),
  \end{equation}
  \begin{equation}
    \label{eq:optim_par}
    \hat{\bOmega}_{\bx\by}^{(k+1)}     =    \argmin_{\bOmega_{\bx\by}}
    J_{\lambda_1\lambda_2}(\bOmega_{\bx\by},\hat{\bOmega}_{\by\by}^{(k+1)}).
  \end{equation}
\end{subequations}

Alternate          strategies         were          adopted         by
\citet{2010_JCGS_rothman,2011_AoAS_yin},   yet  in  these   cases  the
objective   is  only  bi-convex   as  they   rely  on   the  classical
parametrization \eqref{eq:reg_model_row} and  their algorithms are not
meant     to     converge    to     the     global    minimum.      In
\citet{2012_JMLR_sohn,2012_arxiv_yuan},   the  criterion   is  jointly
convex yet the regularization is different from ours and requires more
demanding numerical optimization because  of the regularization of the
concentration  matrix  $\bOmega_{\by\by}$.   Besides,  no  convergence
results are given in these works.

Concerning  our   criterion,  the   alternating  scheme   seems  quite
appropriate:   first,  we   may   apply  the   results  developed   in
\cite{2009_MP_tseng,2001_JOTA_tseng}  on  the   convergence  of  block
coordinate  descent  for  the   minimization  of  nonsmooth  separable
function,   since  \eqref{eq:objective}   is   clearly  separable   in
$(\bOmega_{\bx\by}, \bOmega_{\by\by})$ for  the nonsmooth part induced
by  the  $\ell_1$-norm.  Thus,  under  the  assumption of  Proposition
\ref{prop:existence_uniqueness}, the alternating  scheme is guaranteed
to  convergence  to  the  unique global  minimum.   Second,  efficient
procedures   exist    to   solve    the   two    convex   sub-problems
\eqref{eq:optim_cov} and \eqref{eq:optim_par}, as detailed herein.

On  the   first  hand,  \eqref{eq:optim_par}  can  be   recast  as  an
Elastic-Net problem, which  in turn, can be recast  as a LASSO problem
\citep[see,    e.g.][]{2005_JRSS_Zou,2010_AOAS_slawski}.     This   is
straightforward   thanks  to   Proposition   \ref{prop:vec_obj}:  when
$\hat{\bOmega}_{\by\by}$  is fixed,  solution  to \eqref{eq:optim_par}
can be obtained via
\begin{equation}
  \label{eq:enet_recast}
  \hat{\bomega}     \left(=    \vec(\hat{\bOmega}_{\bx\by})    \right)
  =\argmin_{\bomega\in\Rset^{pq}} \frac{1}{2} \|\mathbf{A}\bomega - \mathbf{b}\|_2^2 + \frac{\lambda_2}{2}
  \bomega^T   \tilde{\bL} 
  \bomega + \lambda_1  \|\bomega\|_1 ,
\end{equation}
where $\bA,\mathbf{b}$ and $\tilde{\bL}$ are defined by
\begin{equation*}
\mathbf{A} =
  \left(\hat{\bOmega}_{\by\by}^{-1/2}   \otimes   \bX/\sqrt{n}  \right),
  \mathbf{b} = - \vec\left(\bY\hat{\bOmega}_{\by\by}^{1/2}\right)/ \sqrt{n}
     \text{ and }
  \tilde{\bL} = \hat{\bOmega}_{\by\by}^{-1} \otimes \bL.
\end{equation*}

On  the second  hand, we  can solve  analytically \eqref{eq:optim_cov}
with  simple matrix algebra,  as stated  in the  following Proposition
whose proof is postponed to Appendix Section \ref{sec:cov_solve}.

\begin{proposition}\label{prop:cov_solve} Let $n\geq q$.  If
  $\hat{\bOmega}_{\bx\by}    =   \bzr$,    $\hat{\bOmega}_{\by\by}   =
  \bS_{\by\by}^{-1}$.  Otherwise,  assume  that  the  following  eigen
  decomposition holds
  \begin{equation*}
    \hat{\bOmega}_{\by\bx} (\lambda_2\bL + \bS_{\bx\bx})
    \hat{\bOmega}_{\bx\by} \bS_{\by\by}  = \bU \diag(\boldsymbol\zeta)
    \bU^{-1}
  \end{equation*}
  and denote by $\boldsymbol\eta=(\eta_1,\dots,\eta_q)$ the respective
  unique positive roots  of $\eta_j^2 - \eta_j -  \zeta_j$.  For a fix
  $\hat{\bOmega}_{\bx\by}$,   solution   $\hat{\bOmega}_{\by\by}$   to
  \eqref{eq:optim_cov} and its inverse writes
  \begin{subequations}
    \begin{equation}
      \label{eq:invcov_solve}
      \hat{\bOmega}_{\by\by} = \bU \diag(\boldsymbol\eta/\boldsymbol\zeta) \bU^{-1}
      \hat{\bOmega}_{\by\bx} (\lambda_2\bL + \bS_{\bx\bx}) \hat{\bOmega}_{\bx\by} (=\hat{\bR}^{-1}),
    \end{equation}
    \begin{equation}
      \label{eq:cov_solve}
      \hat{\bOmega}_{\by\by}^{-1}           =          \bS_{\by\by}\bU
      \diag(\boldsymbol\eta^{-1}) \bU^{-1} (=\hat{\bR}).
    \end{equation}
  \end{subequations}
\end{proposition}

Because  our  procedure  relies  on alternating  optimization,  it  is
difficult to give either a global  rate of convergence or a complexity
bound.   Nevertheless, the  complexity of  each iteration  is easy  to
derive,  since  it  amounts  to  two well  known  problems:  the  main
computational  cost in  \eqref{eq:optim_cov} is  due to  the SVD  of a
$q\times  q$  matrix,   which  costs  $\mathcal{O}(q^3)$.   Concerning
\eqref{eq:optim_par}, it  amounts to the resolution  of an Elastic-Net
problem with $p\times  q$ variables and $n \times q$  samples.  If the
final number of nonzero entries  in $\hat{\bOmega}_{\bx\by}$ is $k$, a
good  implementation  with  Cholesky  update/downdate  is  roughly  in
$\mathcal{O}(n p q^2 k)$  \citep[see, e.g.][]{2012_FOT_bach}. Since we
typically  assumed  that  $n\geq  q$,  the global  cost  of  a  single
iteration of the alternating scheme  is thus $\mathcal{O}(n p q^2 k)$,
and  we theoretically  can  treat  problems with  large  $p$ when  $k$
remains moderate.

Finally, we typically want to  compute a series of solutions along the
regularization  path  of Problem  \eqref{eq:objective},  that is,  for
various  values of  $(\lambda_1,\lambda_2)$.  To  this end,  we simply
choose   a   grid  of   penalties   $\Lambda_1   \times  \Lambda_2   =
\set{\lambda_1^{\text{min}},   \dots,  \lambda_1^{\text{max}}}  \times
\set{\lambda_2^{\text{min}},   \dots,  \lambda_2^{\text{max}}}$.   The
process is  easily distributed on different computer  cores, each core
corresponding to a value picked  in $\Lambda_2$.  Then on each core --
i.e.  for a fix $\lambda_2\in\Lambda_2$  -- we cover all the values of
$\lambda_1\in\Lambda_1$ relying on  the warm start strategy frequently
used  to  go through  the  regularization  path of  $\ell_1$-penalized
problems.    A   prototype  implementation   is   distributed  in   an
\texttt{R}/\texttt{C++}-package  available from  the first  author web
site%\footnote{http://stat.genopole.cnrs.fr/$\sim$jchiquet/spring}
.

% Optimality condition are formulated  thanks to subdifferential calculs
% to handled with the differentiation of the $\ell_1$-norm, so as
%   \begin{equation*}
%   \frac{\partial             J(\bOmega_{\bx\by})}{\partial
%     \bOmega_{\bx\by}}          =          0         \Leftrightarrow
%   \bS_{\bx\by}       +      \hat{\bSigma}_{\bx\bx} \bOmega_{\bx\by}\bR + \lambda_1\bs{\Gamma} =
%   0.
% \end{equation*}
% where $\bs{\Gamma}=(\Gamma_{jk})_{j\in\clM,k\in\clC}$  the $m\times c$
% matrix defined by
% \begin{equation*}
%   \Gamma_{jk} = \begin{cases}
%     \sign\left(\bOmega_{\bx\by}\right)_{jk}       &      \text{      if
%       $\left(\bOmega_{\bx\by}\right)_{jk} \neq 0$}\\
%     \theta: |\theta| < 1 & \text{otherwise}.\\
%   \end{cases}
% \end{equation*}


% with optimality conditions
% \begin{equation}
%   \label{eq:KKT_omega}
%   \left\{\begin{array}{lll}
%       \left( \vec(\bS_{\by\bx}) + (\hat{\bSigma}_{\bx\bx}
%         \otimes\bR)\bomega \right)_i& = -\lambda \
%       \sign(\omega_i) & \text{ if } \omega_i \neq 0\\
%       \left| \left(\vec(\bS_{\by\bx}) + (\hat{\bSigma}_{\bx\bx}
%           \otimes\bR)\bomega\right)_i \right| & \leq \lambda & \text{ if } \omega_i = 0\\
%   \end{array}\right.
% \end{equation}
% The corresponding matrix formulation is
% \begin{equation}
%   \label{eq:KKT_Omega}
%   \left\{\begin{array}{lll}
%       \left(\bS_{\by\bx}   +   \bR
%       \bOmega_{\by\bx}\hat{\bSigma}_{\bx\bx}\right)_{kj} & = -\lambda \
%     \sign(\bOmega_{\by\bx})_{kj}& \text{ if }
%     \left(\bOmega_{\by\bx}\right)_{kj} \neq 0\\
%      \left|  \left(\bS_{\by\bx}  +
%         \bR\bOmega_{\by\bx}\hat{\bSigma}_{\bx\bx} \right)_{kj} \right|
%     & \leq \lambda &
%     \text{ if }
%     \left(\bOmega_{\by\bx}\right)_{kj} = 0.\\
%   \end{array}\right.
% \end{equation}

% \paragraph*{Coordinate   update  for   $\bOmega_{\bx\by}$.}   Consider
% optimizing  against a  single entry  $(\bOmega_{\bx\by})_{jk}$  of the
% matrix.   Cumbersome,  yet straightforward  computation  leads to  the
% following update

% \begin{equation}
%   \label{eq:coordinate_update}
%   (\bOmega_{\bx\by}^\lambda)_{jk}                                           =
%   \frac{\mathrm{Soft}\left(a^{(jk)};\lambda_1\right) }{(\hat{\bSigma}_{\bx\bx})_{jj}
%     \bR_{kk}}, \qquad
%   \mathrm{Soft}(x;\lambda) = x\left(1-\frac{\lambda}{|x|}\right)_+
% \end{equation}
% with
% \begin{equation*}
%   \begin{aligned}
%     a^{(jk)} & = - (\bS_{\bx\by})_{jk} - \sum_{\substack{\ell,m : \\(\ell,m) \neq
%       (j,k)}} (\hat{\bSigma}_{\bx\bx})_{j\ell}
%     (\bOmega_{\bx\by})_{\ell m} \bR_{mk} \\
%     &  = -  (\bS_{\bx\by})_{jk}  - (\hat{\bSigma}_{\bx\bx})_{j\bullet}
%     \bOmega_{\bx\by}  \bR_{\bullet k}  + (\hat{\bSigma}_{\bx\bx})_{jj}
%     (\bOmega_{\bx\by})_{jk} \bR_{k k} .
%   \end{aligned}
% \end{equation*}

%%% Local Variables:
%%% TeX-master: "JST_AOAS_main.tex"
%%% End:


==> arxiv_version/.svn/text-base/v1/proofs.tex <==
\section{Proofs}

Most of the  proofs rely on basic algebra and  properties of the trace
and  the   $\vec$  operators  \citep[see   e.g.][]{book_harville},  in
particular
\begin{gather*}
  \trace(\bA^T  \bB  \bC  \bD^T)   =  \vec(\bA)^T  (\bD  \otimes  \bB)
  \vec(\bC),\\
  \vec(\bA\bB\bC) = (\bC^T \otimes \bA) \vec(\bB), \\
  (\bA \otimes\bB) (\bC\otimes\bD) = (\bA\bC) \otimes (\bC\bD).
\end{gather*}

\subsection{Derivation of Proposition \ref{prop:vec_obj}}
\label{sec:vec_obj}

Concerning  the two regularization  terms in  \eqref{eq:objective}, we
have $\|\bOmega_{\bx\by}\|_1 =  \|\bomega\|_1$ since the $\ell_1$-norm
applies element-wise here and
\begin{equation*}
  \trace(\bOmega_{\by\bx} \bL \bOmega_{\bx\by}\bOmega_{\by\by}^{-1}) =
  \bomega^T (\bOmega_{\by\by}^{-1} \otimes \bL) \bomega.
\end{equation*}

As  for the log-likelihood  \eqref{eq:log_lik}, we  work on  the trace
term:
\begin{multline*}
  \trace\left(  \left(\bY +  \bX \bOmega_{\bx\by}\bOmega_{\by\by}^{-1}
    \right)^\intercal \left(\bY          +          \bX
      \bOmega_{\bx\by}\bOmega_{\by\by}^{-1}
    \right)\bOmega_{\by\by}\right) \\ 
  \begin{aligned}
    &         =          &         \vec\left(\bY         +         \bX
      \bOmega_{\bx\by}\bOmega_{\by\by}^{-1}\right)^T
    \left(\bOmega_{\by\by}\otimes\bI_n\right) \vec\left(\bY + \bX
      \bOmega_{\bx\by}\bOmega_{\by\by}^{-1}\right) \\
    &   =   &   \left\|\left(\bOmega_{\by\by}\otimes\bI_n\right)^{1/2}
      \left(  \vec(\bY)   +  \left(\bOmega_{\by\by}^{-1}  \otimes  \bX
        \right)
        \vec(\bOmega_{\bx\by}) \right)\right\|_2^2    \\
      &     =    &    \left\|     \vec(\bY\bOmega_{\by\by}^{1/2})    +
        \left(\bOmega_{\by\by}^{-1/2}\otimes   \bX   \right)   \bomega
      \right\|_2^2.
  \end{aligned}
\end{multline*}
The rest of the proof is straightforward.

\subsection{Derivation of Proposition \ref{prop:cov_solve}}
\label{sec:cov_solve}

By   differentiation  of   the  objective   \eqref{eq:objective}  over
$\bOmega_{\by\by}^{-1}$ we obtain the quadratic form
\begin{equation*}
  \bOmega_{\by\by}       \bS_{\by\by}      \bOmega_{\by\by}      -
  \bOmega_{\by\by}                                                =
  \bOmega_{\by\bx}(\lambda_2 \bL + \bS_{\bx\bx})\bOmega_{\bx\by}.
\end{equation*}
After  right  multiplying both  sides  by  $\bS_{\by\by}$, it  becomes
obvious       that      $\bOmega_{\by\by}       \bS_{\by\by}$      and
$\bOmega_{\by\bx}(\lambda_2                    \bL                   +
\bS_{\bx\bx})\bOmega_{\bx\by}\bS_{\by\by}$ commute  and thus share the
same  eigenvectors  $\bU$.    Besides,  it  induces  the  relationship
$\eta_j^2  -\eta_j  = \zeta_j$  between  their respective  eigenvalues
$\eta_j$ and $\zeta_j$,  and we are looking for  the positive solution
of  $\eta_j$.   To  do  so,  first  remark that  we  may  assume  that
$\bOmega_{\by\bx} (\lambda_2 \bL + \bS_{\bx\bx}) \bOmega_{\bx\by}$ and
$\bS_{\by\by}$  are  positive  definite, when  $\bOmega_{\bx\by}  \neq
\bzr$  and $n\geq q$;  and second,  recall that  the eigenvalues  of a
matrix  being  the  product  of  two positive  definite  matrices  are
positive. Hence, $\zeta_j>0$ % (note that this does not imply the symmetry
% of             $\bOmega_{\by\bx}(\lambda_2            \bL            +
% \bS_{\bx\bx})\bOmega_{\bx\by}\bS_{\by\by}$,   though)
and the positive solution of $\eta_j$ is $\eta_j = (1 +
\sqrt{1+4\zeta_j})/2$. We obtain thus
\begin{equation}
  \label{eq:cov_prf}
  \hat{\bOmega}_{\by\by} = \bU \diag(\boldsymbol\eta) \bU^{-1} \bS_{\by\by}^{-1}.
\end{equation}
Direct      inversion     leads      to  \eqref{eq:cov_solve}.     To    get    an   expression    for
$\hat{\bOmega}_{\by\by}$  which  does  not require  additional  matrix
inversion, just remark that
\begin{equation*}
  \bS_{\by\by}^{-1}                                                =
  \left(\bOmega_{\by\bx}\hat{\bSigma}_{\bx\bx}^{\lambda_2}\bOmega_{\bx\by}\bS_{\by\by}\right)^{-1}
  \bOmega_{\by\bx}\hat{\bSigma}_{\bx\bx}^{\lambda_2}\bOmega_{\bx\by}
   = \bU \diag(\boldsymbol\zeta^{-1})\bU^{-1}\bOmega_{\by\bx}\hat{\bSigma}_{\bx\bx}^{\lambda_2}\bOmega_{\bx\by}
\end{equation*}
which,     combined      with     \eqref{eq:cov_prf},     leads     to
\eqref{eq:invcov_solve}.

\subsection{Derivation of Proposition \ref{prop:df_spring}}
\label{sec:df_spring}

To  apply the  results developed  in  \citet{2012_EJS_Tibshirani} that
rely  on  the   well-known  Stein's  Lemma  \citep{1981_AS_Stein},  we
basically need to recast our problem as a classical LASSO applied on a
Gaussian linear regression  model so as the response  vector follows a
normal distribution of  the form $\mathcal{N}(\bmu,\sigma \bI)$.  This
is straightforward by means  of Proposition \ref{prop:vec_obj}: in the
same way as  we derive expression \eqref{eq:enet_recast}, we  can go a
little farther and reach the following LASSO formulation
\begin{equation}
  \label{eq:lasso_recast}
  \argmin_{\bomega\in\Rset^{pq}} \frac{1}{2} \left\|
    \begin{pmatrix}
      \mathbf{A} \\ \sqrt{\lambda_2} \tilde{\bL}^{1/2}
    \end{pmatrix} \bomega - 
    \begin{pmatrix}
      \mathbf{b} \\ \bzr
    \end{pmatrix} \right\|_2^2  + \lambda_1  \|\bomega\|_1,
\end{equation}
with $\bA,\bb$ and $\tilde{\bL}$ defined as in \eqref{eq:enet_recast}.
From model \eqref{eq:cond_model_mat}, it  is not difficult to see that
$\mathbf{b}$ corresponds to an uncorrelated vector form of $\bY$ so as
\begin{equation*}
  \begin{pmatrix}
    \mathbf{b} \\ \bzr
  \end{pmatrix} = 
  \begin{pmatrix}
    -\vec(\bY \bOmega_{\by\by}^{1/2}) \\ \bzr
  \end{pmatrix} \sim \mathcal{N}(\bmu, \bI_{nq}).
\end{equation*}
The  explicit form  of  $\bmu$ has  no  interest here.   The point  is
essentially to  underline that the response vector  is uncorrelated in
\eqref{eq:lasso_recast},  which  allows  us  to  apply  Theorem  2  of
\citeauthor{2012_EJS_Tibshirani} and results  therein, notably for the
Elastic-Net: by these  means, an unbiased estimator of  the degrees of
freedom in \eqref{eq:lasso_recast} can be written as a function of the
active set $\mathcal{A}$ in $\hat{\bomega}^{\lambda_1,\lambda_2}$:
\begin{equation*}
  \hat{\mathrm{df}}_{\lambda_1,\lambda_2} = \trace\left( 
    \mathbf{A}_{\mathcal{A}} \left( (\bA^T\bA + \lambda_2 \tilde{\bL}\ )_{\mathcal{A}\mathcal{A}}\right)^{-1}
    \mathbf{A}_{\mathcal{A}}^T
  \right).
\end{equation*}
Routine    simplifications     lead    to    the     desired    result
\eqref{eq:df_spring}.



% \subsection{Derivation of Proposition \ref{prop:enet_recast}}
% \label{sec:enet_recast}


% %\begin{proof}
%   Minimizing  \eqref{eq:optim_pb} over $\bOmega_{\bx\by}$  only boils
%   down to the minimization of 
%   \begin{equation*}
%     \trace(\bS_{\bx\by}\bOmega_{\by\bx}) + \frac{1}{2}\trace\left(\bOmega_{\by\bx}
%       \hat{\bSigma}_{\bx\bx}^{\lambda_2}\bOmega_{\bx\by} \bOmega_{\by\by}^{-1} \right) + \lambda \|\bOmega_{\bx\by}\|_1.
%   \end{equation*}
%   Looking towards a familiar vector formulation, we introduce $\bomega
%   = \vec(\bOmega_{\by\bx})  = ((\bOmega_{\bx\by})_{1\bullet}^T, \dots,
%   (\bOmega_{\bx\by})_{q\bullet}^T)$  ,  the   $q\times  p$  vector  of
%   parameters, stacking the coefficients  related to the successive $p$
%   predictors across the $q$  outputs. By means of classical properties
%   of the trace and $\vec$ operators, we first notice that
%   \begin{equation*}
%     \trace(\bS_{\bx\by}\bOmega_{\by\bx})                             =
%     \vec(\bOmega_{\by\bx})^T\vec(\bS_{\by\bx}),
%   \end{equation*}
%   and second,
%   \begin{multline*}
%     \trace\left(\bOmega_{\by\bx}
%       \hat{\bSigma}_{\bx\bx}^{\lambda_2}\bOmega_{\bx\by}
%       \bOmega_{\by\by}^{-1}  \right)  = \trace\left(  \bOmega_{\bx\by}
%       \bOmega_{\by\by}^{-1}                            \bOmega_{\by\bx}
%       \hat{\bSigma}_{\bx\bx}^{\lambda_2}\right)          \\          =
%     \vec(\bOmega_{\bx\by}^T)^T          \vec\left(\bOmega_{\by\by}^{-1}
%       \bOmega_{\by\bx} \hat{\bSigma}_{\bx\bx}^{\lambda_2}\right) \\ =
%     \vec(\bOmega_{\by\bx})^T   \left(\hat{\bSigma}_{\bx\bx}^{\lambda_2}
%       \otimes \bOmega_{\by\by}^{-1} \right) \vec(\bOmega_{\by\bx}).
%   \end{multline*}
%   The above minimization problem is thus equivalent to
%   \begin{equation*}
%     \min_{\bomega\in\Rset^{pq}}   \left\{  \frac{1}{2}   \bomega^T  (\hat{\bSigma}_{\bx\bx}^{\lambda_2}
%       \otimes\bOmega_{\by\by}^{-1}) \bomega + \bomega^T \vec(\bS_{\by\bx}) + \lambda
%       \|\bomega\|_1\right\},
%   \end{equation*}
%   providing  that   $\bomega=\vec(\bOmega_{\by\bx})$.   This  $\ell_1$
%   penalized problem can be recast as a structured Elastic-Net problem:
%   by     direct    identification     with    terms     expanded    in
%   \eqref{eq:enet_recast} from  $\|\bA \bomega -  \mathbf{b}\|_2^2$, we
%   just have to solve in $(\bA, \mathbf{b})$
%   \begin{equation*}
%     \left\{\begin{array}{lcr}
%         \bA^T\bA    & = &    \hat{\bSigma}_{\bx\bx}^{\lambda_2}
%         \otimes\bOmega_{\by\by}^{-1}, \\[.5ex]
%         \mathbf{b}^T \bA & = & \vec(\bS_{\by\bx}),
%       \end{array}\right.
%   \end{equation*}
%   which is straightforward.
  
\subsection{Derivation of Proposition \ref{prop:computeDkl}}
\label{sec:computeDkl}

Both results are established by recurrence, the first on
 indices $k$, the second on indices $\ell$. Consider
 \eqref{eq:reck_D} and indices $k$ for instance: this holds true for
 $k=1$ by straightforward matrix calculus. Now, assume that
 $\bD^{k,\ell}$ is known, and you are looking for $\bD^{k+1,\ell}$ by
 increasing the alphabet $\clM_k$ with one letter, so as
 lexicographical order still holds true: this can be done by adding
 successively each letter from $\clM_1=\set{A,C,G,T}$ to the left of
 each word of $\clM_k$ (first $A$ to every work in $\clM_k$, then $C$
 and so on). There are now only two possibilities, which corresponds
 to each term in the right-hand side of \eqref{eq:reck_D}:

 Consider the first term on the one hand: non null elements in
 $\bD^{k,\ell}$ represent the set of motifs with size $k$ being at
 distance $\ell$ to each other. If adding a letter to such motifs, we
 can split the obtained words in four groups, according to the
 currently added letter ($A,C,G$ or $T$). Then, within each of these
 groups (e.g. the group with words starting by $A$), all the words
 shared the very same first letter and thus stay at a distance $\ell$
 from each other: this is just meant by the Kronecker multiplication
 by $\bD^{1,0}$, which builds four blocks corresponding to the four
 aforementioned groups.

 On the other hand, consider the second term: if motifs with size $k$
 are at distance $\ell-1$ from each other, what represents
 $\bD^{k,\ell-1}$, then we can add any kind of letter and stay at a
 distance $\ell$ for motifs with size $k+1$, what is meant by the
 Kronecker product with $\bD^{1,1}$.

  

  
  
  % Thanks  to  the  Cholesky factorization  introduced  in  Proposition
  % \ref{prop:enet_recast}, we have
  % \begin{multline*}
  %   \hat{\bSigma}_{\bx\bx}^{\lambda_2}  \otimes\bOmega_{\by\by}^{-1} =
  %   \left(\frac{1}{n}  \bX^T \bX  +  \lambda_2 \bL\right)  \otimes
  %   \bC^T\bC \\ =
  %   \begin{bmatrix}
  %     \begin{pmatrix}
  %       \bX /\sqrt{n} \\
  %       \sqrt{\lambda_2} \bD
  %     \end{pmatrix}
  %     \otimes \bC
  %   \end{bmatrix}^T
  %   \begin{bmatrix}
  %     \begin{pmatrix}
  %       \bX /\sqrt{n} \\
  %       \sqrt{\lambda_2} \bD
  %     \end{pmatrix}
  %     \otimes \bC
  %   \end{bmatrix},
  %   \end{multline*}
  % from which  we get $\bA$.  The vector $\mathbf{b}$ follows  with the
  % same kind of algebra.
%\end{proof}


% \subsection{Derivation of Proposition \ref{prop:prop_loglik_reg}}
% \label{sec:prop_loglik_reg}

% Considering    model   \eqref{eq:reg_model_row},    then    for   each
% $i=1,\dots,n$,                         we                         have
% $\tilde{\by}_i\sim\mathcal{N}(\bB^\intercal\tilde{\bx}_i,\bR),$ and by
% successively  using $|\bA  \otimes  \bB| =  |\bA|^{\mathrm{rank}(\bB)}
% |\bB|^{\mathrm{rank}(\bA)}$, $\trace(\bA^\intercal\bB\bC\bD^\intercal)
% =       \vec(\bA)^\intercal       (\bD\otimes\bB)\vec(\bC)$,       and
% $(\bA\otimes\bB)^{-1}=(\bA^{-1}\otimes\bB^{-1})$, we get
% \begin{multline*}
%   \log    L_{\bX,\bY}   \varpropto    -\log|\bR_q\otimes   \bLambda_n|
%   -\frac{1}{2} \vec(\bY-\bX\bB)^\intercal
%   (\bR_q\otimes\bLambda_n)^{-1}\vec(\bY-\bX\bB)\\
%   =                  -n\log|\bR_q|-q\log|                  \bLambda_n|
%   -\frac{1}{2}\trace\left((\bY-\bX\bB)^\intercal\bLambda_n^{-1}
%     (\bY-\bX\bB-\bU)\bR_q^{-1} \right).
% \end{multline*}

% The result follows since $\trace(\bA^\intercal\bA) = \|\bA\|_F^2$.

% \subsection{Derivation of Proposition 1}
% \label{sec:prop_intercept}
% First, we need  a convenient row wise rescaling of  the data $\bY$ and
% $\bX$,  as   in  generalized  least-square.   This  can  be   done  by
% left-multiplying    \eqref{eq:reg_model_vec}   by    $(\bI_q   \otimes
% \bLambda_n^{-\frac{1}{2}})$,  and by  the property  $\vec(\bA\bB\bC) =
% (\bC^\intercal \otimes \bA) \vec(\bB)$ of the $\vec$ operator, we have
% \begin{equation}
%   \label{eq:proof_intercept_1}
%   \vec(\bLambda_n^{-\frac{1}{2}}\bY)                                =
%   \vec(\bLambda_n^{-\frac{1}{2}}\bX\bB)                             +
%   \vec(\bLambda_n^{-\frac{1}{2}}\bU)     +    \var((\bI_q    \otimes
%   \bLambda_n^{-\frac{1}{2}})\vec(\bepsilon)),
% \end{equation}
% where the variance of the residuals is given by\footnote{Recall that
%   $(\bA  \otimes   \bB)  (\bC   \otimes  \bD)  =   (\bA\bC)  \otimes
%   (\bB\bD)$.}
% \begin{equation*}
%   \var((\bI_q  \otimes  \bLambda_n^{-\frac{1}{2}})\vec(\bepsilon)) =
%   (\bI_q    \otimes   \bLambda_n^{-\frac{1}{2}})    (\bR_q   \otimes
%   \bLambda_n) (\bI_q  \otimes \bLambda_n^{-\frac{1}{2}})^\intercal =
%   \bR_q \otimes \bI_n.
% \end{equation*}

% Hence,   we   can   treat   each   conditions   separately   as   in
% \eqref{eq:reg_model_row}.  Consider for  instance condition $c$: the
% residuals  sum of squares  in \eqref{eq:proof_intercept_1}  for this
% condition writes
% \begin{equation*}
%   \left\| \bLambda_n^{-1/2} \left(\by_{(c)}- \mu_c \I_n - \bX \bb_{(c)}\right)\right\|_2^2,
% \end{equation*}
% Then, differentiating over $\mu_c$, we get that
% \begin{equation*}
%   \hat{\mu}_c                 =                \frac{\I_n^\intercal
%     \bLambda_n^{-1}}{\I_n^\intercal             \bLambda_n^{-1}\I_n}
%   \left(\by_{(c)} - \bX \bb_{(c)}\right).
% \end{equation*}
% Write this  formulation for  each condition in  $\clC$, and  we meet
% back \eqref{eq:intercept}.

% \subsection{Derivation of Proposition 3}
% \label{sec:prop_loglik_cggm}

% Considering  model \eqref{eq:reg_model_vec}  with  no intercept,  then
% $\vec(\bY)\sim\mathcal{N}(\vec(\bX\bB),\bR_q\otimes\bLambda_n)$,    and
% by successively using  $|\bA \otimes \bB| = |\bA|^{\mathrm{rank}(\bB)}
% |\bB|^{\mathrm{rank}(\bA)}$, $\trace(\bA^\intercal\bB\bC\bD^\intercal)
% =       \vec(\bA)^\intercal       (\bD\otimes\bB)\vec(\bC)$,       and
% $(\bA\otimes\bB)^{-1}=(\bA^{-1}\otimes\bB^{-1})$, we get
% \begin{multline*}
%   \log   L    (\bB,\bLambda_n,\bR_q)   \varpropto   -\log|\bR_q\otimes
%   \bLambda_n| -\frac{1}{2} \vec(\bY-\bX\bB)^\intercal
%   (\bR_q\otimes\bLambda_n)^{-1}\vec(\bY-\bX\bB)\\
%   =                  -n\log|\bR_q|-q\log|                  \bLambda_n|
%   -\frac{1}{2}\trace\left((\bY-\bX\bB)^\intercal\bLambda_n^{-1}
%     (\bY-\bX\bB)\bR_q^{-1} \right).
% \end{multline*}
% and the result follows since $\trace(\bA^\intercal\bA) = \|\bA\|_F^2$.

%%% Local Variables:
%%% TeX-master: "JST_AOAS_main.tex"
%%% End:


==> arxiv_version/.svn/text-base/v1/selection.tex <==
\subsection{Model selection and parameter tuning}
\label{Sec:selection}

Model selection amounts here to choosing a couple of tuning parameters
$(\lambda_1,\lambda_2)$ among the grid $\Lambda_1 \times
\Lambda_2% = \set{\lambda_1^{\text{min}}, \dots,
  % \lambda_1^{\text{max}}}  \times  \set{\lambda_2^{\text{min}}, \dots,
  % \lambda_2^{\text{max}}}
$, where  $\lambda_1$ tunes the  sparsity while $\lambda_2$  tunes the
amount  of structural regularization.   We aim  either at  picking the
model with  minimum prediction error, or  the one closest  to the true
model   assuming  Equation~\eqref{eq:cond_model}  holds.    These  two
perspectives  generally do  not lead  to the  same model  choice: when
looking  for  the  model  minimizing the  prediction  error,  $K$-fold
cross-validation   is  the  recommended   option  \citep{Hesterberg08}
despite  its   additional  computational  cost.    Letting  $\kappa  :
\set{1,\dots,n}\to\set{1,\dots,K}$ the  function indexing the  fold to
which observation $i$ is allocated, the CV-choice is
\begin{equation*}
  \label{eq:cv_pred}
  (\lambda_1^\text{cv},\lambda_2^\text{cv})                                    =
  \argmin_{(\lambda_1,\lambda_2) \in \Lambda_1\times\Lambda_2}
  \frac{1}{n} \sum_{i=1}^n 
  \left\| \bx_{i}^T \hat{\bB}_{-\kappa(i)}^{\lambda_1,\lambda_2}- \by_{i} \right\|_2^2,
\end{equation*}
where   $\hat{\bB}_{-\kappa(i)}^{\lambda_1,\lambda_2}$  minimizes  the
objective  \eqref{eq:objective},   once  data  $\kappa(i)$   has  been
removed. In  place of  the prediction error,  other quantities  can be
cross-validated  in  our  context,  e.g. the  negative  log-likelihood
\eqref{eq:log_lik}. In  the remainder of  the paper, we  only consider
cross-validating the prediction error, though.

As  an alternative  to cross-validation,  analytic criteria  provide a
fast way to  perform model selection and are  sometimes more suited to
the  selection of  the  true underlying  model.   Although relying  on
asymptotic derivations,  they often offer  good practical performances
when the  sample size  $n$ is  not too small  compared to  the problem
dimension.   For  penalized  methods,   a  general  form  for  various
information criteria is expressed as  a function of the likelihood $L$
(defined  by \eqref{eq:log_lik}  here)  and the  effective degrees  of
freedom:
\begin{equation}
  \label{eq:pen_crit}
  (\lambda_1^\text{pen},\lambda_2^\text{pen}) = \argmin_{(\lambda_1,\lambda_2)\in\Lambda_1\times\Lambda_2}
  - 2\log L(\hat{\bOmega}^{\lambda_1,\lambda_2}_{\bx\by},
  \hat{\bOmega}^{\lambda_1,\lambda_2}_{\by\by})   +   \mathrm{pen}
  \cdot \mathrm{df}_{\lambda_1, \lambda_2}.
\end{equation}
Setting $\text{pen}=2$  or $\log(n)$ respectively lead to  AIC or BIC.
For the practical evaluation of \eqref{eq:pen_crit}, we must give some
sense      to      the      effective     degrees      of      freedom
$\text{df}_{\lambda_1,\lambda_2}$  of a  SPRING fit.   We use  the now
classical definition  of \citet{2004_JASA_Efron} and rely  on the work
of  \citet{2012_EJS_Tibshirani} to  derive the  following Proposition,
whose proof is postponed to Appendix Section \ref{sec:df_spring}.

\begin{proposition}\label{prop:df_spring}  An  unbiased  estimator  of
  $\text{df}_{\lambda_1,\lambda_2}$ for a SPRING fit is 
  \begin{equation}
    \label{eq:df_spring}
    \hat{\mathrm{df}}_{\lambda_1,  \lambda_2} = \mathrm{card}(\mathcal{A})
    - \lambda_2          \mathrm{tr}\left(         (\hat{\bR}\otimes
      \bL )_{\mathcal{A}\mathcal{A}} \left((\hat{\bR}\otimes (\bS_{\bx\bx} +
      \lambda_2\bL))_{\mathcal{A}\mathcal{A}}\right)^{-1}\right),
  \end{equation}
  where               $\mathcal{A}              =              \set{j:
    \vec\left(\hat{\bOmega}_{\bx\by}^{\lambda_1,\lambda_2}\right) \neq
    0}$     is      the     set     of      nonzero     entries     in
  $\hat{\bOmega}_{\bx\by}^{\lambda_1,\lambda_2}$.
\end{proposition}

Note  that  we  can  compute  expression  \eqref{eq:df_spring}  at  no
additional  cost,  relying on  computations  already  made during  the
optimization process.

%%% Local Variables:
%%% TeX-master: "JST_AOAS_main.tex"
%%% End:


==> arxiv_version/.svn/text-base/v1/simu_studies.tex <==
\subsection{Influence of covariance between outcomes}  

The  first  simulation  study  aims  to illustrate  the  advantage  of
splitting $\bB$  into $-\bOmega_{\bx\by}\bR$ over  working directly on
$\bB$.  We  set $p=40$ predictors, $q=5$ outcomes  and randomly select
$25$ non  null entries in $\set{-1,1}$ to  fill $\bOmega_{\bx\by}$. We
do not put any structure along the predictors as this study intends to
measure the gain of using the cGGM approach.  The covariance follows a
Toeplitz  scheme \footnote{We set  $\bR$ a  correlation matrix  not to
  excessively penalize the LASSO or the group-LASSO, that use the same
  tuning parameter $\lambda_1$ across  the outcomes (and thus the same
  variance  estimator).}    so  as  $\bR_{ij}   =  \tau^{|i-j|}$,  for
$i,j=1,\dots,q$.    We  consider  three   scenarios  tuned   by  $\tau
\in\set{.1,.5,.9}$ corresponding to  an increasing correlation between
the  outcomes that  eventually  makes the  cGGM  more relevant.   This
settings    have   been    used   to    generate   panel    $(a)$   of
Figure~\ref{fig:model_insight}.  For   each  covariance  scenario,  we
generate a  training set  with size  $n=50$ and a  test set  with size
$n=1000$.   We assess  the performance  of SPRING  by  comparison with
three baselines:  $i)$ the LASSO, $ii)$  the $\ell_1/\ell_2$ multitask
group-LASSO and $iii)$ SPRING  with known covariance matrix $\bR$.  As
it corresponds to the best fit  that we can meet with our proposal, we
call this variant the ``oracle'' mode of SPRING.  The final estimators
are obtained  by 5-fold cross-validation on the  training set.  Figure
\ref{fig:cov_mse}  gives   the  boxplots   of  PE  obtained   for  100
replicates.  As expected, the  advantage of taking the covariance into
account  becomes more  an more  important to  maintain a  low  PE when
$\tau$ increases.   When correlation is  low, the LASSO  dominates the
group-LASSO;  this is  the other  way  round in  the high  correlation
setup, where  the latter takes  full advantage of its  grouping effect
along the  outcomes. Still, our proposal  remains significantly better
as  soon as  $ \tau$  is  substantial enough.  We also  note that  our
iterative algorithm does a good  job since SPRING remains close to its
oracle variant.
\begin{figure}[htbp!]
  \centering
  \includegraphics[trim=0 0 0 15pt,clip=true,width=.65\columnwidth]{figures/cov_simu_err}
  \caption{Illustration  of  the  influence  of  correlations  between
    outcomes.  Scenarios $\set{\text{low},\text{med},\text{high}}$ map
    to  $\tau\in\set{.1,.5,.9}$   in  the  Toeplitz-shaped  covariance
    matrix $\bR$.}
    \label{fig:cov_mse}
    \vspace{-.5cm}
\end{figure}

\subsection{Structure   integration   and   robustness}   The   second
simulation study is  designed to measure the impact  of introducing an
informative prior along the predictors via $\bL$. To remove any effect
induced by the covariance between  the outputs, we fix $q=1$.  In this
case      the     criterion      writes     as      in     Expressions
\eqref{eq:criteria_univariate}   and  \eqref{eq:criteria2_univariate}:
$\bR$  boils down  to a  scalar $\sigma^2$  and $\bB,\bOmega_{\bx\by}$
turn to two  $p$-size vectors sharing the same  sparsity pattern so as
$\bbeta = -\bomega  \sigma^2$.  In this situation, SPRING  is close to
\citeauthor{2010_AOAS_slawski}'s  structured Elastic-Net,  except that
we  hope for a  better estimation  of the  coefficients thanks  to the
estimation of $\sigma$.  For comparison, we thus draw inspiration from
the simulation  settings originally used to  illustrate the structured
Elastic-Net: we set $\bomega  = (\omega_j)_{j=1}^p, $ with $p=100$, so
as we observe a sparse vector  with two smooth bumps, one positive and
the other one negative:
\begin{equation*}
  \omega_j =
  \begin{cases}
    -( (30-j)^2 -100)/200 & j=21,\dots 39,\\
    \ \ \ ( (70-j)^2 -100)/200 & j=61,\dots 80,\\
    0 & \text{otherwise}.
  \end{cases}
\end{equation*}
A natural choice for $\bL$ is  to rely on the first forward difference
operator  as in the  fused-Lasso \citep{2005_JRSSB_tibshirani},  or it
smooth counterpart \citep{2011_EJS_Hebiri}.  We thus set %\footnote{This
  % is      also     the      default     choice      recommended     by
  % \citeauthor{2010_AOAS_slawski}.}
$\bL = \bD^T\bD$ with
\begin{equation}
  \label{eq:first_order_diff}
  \bD_{ij} = \begin{cases}
    1 & \text{if } i = j,\\
    -1 & \text{if } j = i+1 \\
    0 & \text{otherwise}\\
  \end{cases},
  \quad \begin{array}{c}
    i=1,\dots,p-1, \\
    j=1,\dots,p.    
  \end{array}
\end{equation}
Hence, $\bL$ is  the combinatorial Laplacian of a  chain graph between
the successive predictors.  
\begin{figure}[htpb!]
  \centering
  \includegraphics[trim=0 0 0 15pt,clip=true,width=.65\columnwidth]{figures/struct_simu}
  \caption{Illustrating gain  brought by structure  information toward
    predictive performance}
  \label{fig:struct_illustration}
\end{figure}
Figure~\ref{fig:struct_illustration} shows the typical gain brought by
prior structure knowledge.  We generate $120$ samples for the learning
with $\sigma^2=5$ and  represent 100 averaged PE curves  as a function
of  $\lambda_1$ for the  LASSO and  for two  versions of  SPRING, with
($\lambda_2 =  .01$) and without ($\lambda_2 =  0$) informative prior.
Incorporating a  relevant structural  information leads to  a dramatic
improvement.  As  expected, univariate  SPRING with no  prior performs
like the LASSO, in the sense that they share the same minimal PE.

Now, the question is:  what if we introduce a wrong  prior, that is, a
matrix $\bL$  completely disconnected from  the true structure  of the
coefficients?  To  answer this question,  we use the same  settings as
above and  randomly swap the  entries in $\bomega$, using  exactly the
same $\bx_i$  to generate the  $\by_i$\footnote{We also used  the same
  seed and CV-folds for both  scenarios.}.  We then apply SPRING using
respectively  a non  informative prior  equal to  the identity  matrix
(thus mimicking the Elastic-Net) and  a 'wrong' prior $\bL$ whose rows
and columns remain unswapped.  We  also try the LASSO, the Elastic-Net
and the  structured Elastic-Net.   All methods  are tuned  with 5-fold
cross-validation  on  the  learning  set.   Table~\ref{tab:struct_res}
presents the results averaged over 100  runs both in term of PE (using
a size-1000 test set) and MSE.
\begin{table}[htbp!]
  \centering
  \begin{small}
    \begin{tabular}{lrrr}
    \hline
    \textit{\textsf{Method}} & \textit{\textsf{Scenario}} & \textit{\textsf{MSE}} & \textit{\textsf{PE}} \\
    \hline
    LASSO
    & -- & .336 (.096) & 58.6 (10.2) \\
%    & swapped & .336 (.096) & 58.6 (10.2) \\
    \cline{1-4}
%     E-Net
%     & unswapped& .340 (.095) & 59 (10.3) \\
%     ($\bL=\bI$)
%     & swapped & .340 (.095) & 59 (10.3) \\
    E-Net    ($\bL=\bI$)
    & -- & .340 (.095) & 59 (10.3) \\
    \cline{1-4}
%     SPRING
%     & unswapped& .358 (.094) & 60.7 (10) \\
%     ($\bL=\bI$)
%     & swapped & .358 (.094) & 60.7 (10) \\
    SPRING    ($\bL=\bI$)
    & -- & .358 (.094) & 60.7 (10) \\
    \cline{1-4}
    S. E-net
    & unswapped & .163 (.036) & 41.3 ( 4.08) \\
    ($\bL=\bD^T \bD$)
    & swapped & .352 (.107) & 60.3 (11.42) \\
    \cline{1-4}
    SPRING
    & unswapped & .062 (.022) & 31.4 ( 2.99) \\
    ($\bL=\bD^T \bD$)
    & swapped & .378 (.123) & 62.9 (13.15) \\
    \hline
  \end{tabular}
  \end{small}
  \caption{Structure integration: performance and robustness. Swapped and unswapped results are the same for LASSO, Elastic-Net and SPRING for $\bL = \bI$.}
  \label{tab:struct_res}
\end{table}

As  expected,  the  methods  that  do  not  integrate  any  structural
information  (LASSO, Elastic-Net  and SPRING  with $\bL=\bI$)  are not
affected by the permutation, {and we avoid these redundancies in Table
  \ref{tab:struct_res} to  save space}.   Overall, they  share similar
performance both in  term of PE and MSE.  When  the prior structure is
relevant, SPRING, and  to a lesser extent  the structured Elastic-Net,
clearly  outperform  the  other competitors.   Surprisingly,  this  is
particularly  true in  term of  MSE, where  SPRING also  dominates the
structured Elastic-Net  that disposes  of the same  information.  This
means that the estimation of the variance also helped in the inference
process.  Finally, these results essentially support the robustness of
the structured methods  which are not much altered when  using a wrong
prior
specification.

%%% Local Variables:
%%% TeX-master: "JST_AOAS_main.tex"
%%% End:


==> arxiv_version/.svn/text-base/v1/stat_model.tex <==
\subsection{Convex parametrization of multivariate regression}
\label{Sec:stat_model}

The statistical  framework arises from a  different parametrization of
\eqref{eq:reg_model_row}  which  fills  the gap  between  multivariate
regression  and  GGM.   Such  a  connection was  first  underlined  in
\citet{2012_JMLR_sohn},     generalizing    the    link     made    by
\citet{2009_JRSSB_witten} in the single  output case between the LASSO
and  inverse covariance  estimation. This  amounts to  investigate the
joint  probability distribution  of $(\bx_i,  \by_i)$ in  the Gaussian
case, with the  following block-wise decomposition % \footnote{note that
  % $\bSigma_{\by\bx}=\bSigma_{\bx\by}^T$                             and
  % $\bOmega_{\by\bx}=\bOmega_{\bx\by}^T$ by symmetry}
of the covariance
matrix $\bSigma$ and its inverse $\bOmega=\bSigma^{-1}$:
  \begin{equation}
    \label{eq:joint_model}
    \bSigma = \begin{pmatrix}
      \bSigma_{\bx\bx} & \bSigma_{\bx\by} \\
      \bSigma_{\by\bx} & \bSigma_{\by\by} \\
   \end{pmatrix},\quad
   \bOmega = \begin{pmatrix}
     \bOmega_{\bx\bx} & \bOmega_{\bx\by} \\
     \bOmega_{\by\bx} & \bOmega_{\by\by} \\
   \end{pmatrix}.
 \end{equation}
 Back  to   the  distribution  of  $\by_i$   conditional  on  $\bx_i$,
 multivariate Gaussian  analysis shows that, for  centered $\bx_i$ and
 $\by_i$,
\begin{equation}
  \label{eq:cond_model}
  \by_i | \bx_i \sim
  \mathcal{N}\left(-\bOmega^{-1}_{\by\by}\bOmega_{\by\bx}
    \bx_i, \bOmega_{\by\by}^{-1} \right).
\end{equation}
This      model,      associated      to     the      full      sample
$\{(\bx_i,\by_i)\}_{i=1,\dots,n}$, can be written  in a matrix form by
stacking in  row the observations of  the responses on  the first hand,
and of the  predictors on the second hand, in  two data matrices $\bY$
and $\bX$ with respective sizes $n\times q$ and $n\times p$, so as
\begin{equation}
  \label{eq:cond_model_mat}
  \bY = \bX \bOmega_{\bx\by} \bOmega_{\by\by}^{-1} + \bvarepsilon, \qquad
  \vec(\bvarepsilon) \sim
  \mathcal{N}\left(\bzr_{nq}, \bI_{p} \otimes \bOmega_{\by\by}^{-1} \right),
\end{equation}
where, for a  $n \times p$ matrix ${\bf A}$,  denoting ${\bf A}_j$ its
$j$th  column, the  $\vec$ operator  is  defined as  $\vec({\bf A})  =
(\bA_1^T     \dots     \bA_p^T)^T$.      The     log-likelihood     of
\eqref{eq:cond_model_mat}  --   which  is  a   conditional  likelihood
regarding the joint model \eqref{eq:joint_model} -- writes
\begin{multline}
  \label{eq:log_lik}
  \log L(\bOmega_{\bx\by},\bOmega_{\by\by}) = 
  \frac{n}{2}\log\left|\bOmega_{\by\by}\right| + \\ \frac{n}{2}
  \trace\left(  \left(\bY -  \bX \bOmega_{\bx\by}\bOmega_{\by\by}^{-1}
    \right)          \bOmega_{\by\by}\left(\bY          -          \bX
      \bOmega_{\bx\by}\bOmega_{\by\by}^{-1} \right)^T\right) +
  \mathrm{cst.}
\end{multline}
Introducing  the  empirical  matrices  of covariance  $\bS_{\by\by}  =
n^{-1}\sum_{i=1}^n\by_i        \by_i^T$,        $\bS_{\bx\bx}        =
n^{-1}\sum_{i=1}^n\bx_i     \bx_i^T$,      and     $\bS_{\by\bx}     =
n^{-1}\sum_{i=1}^n\by_i \bx_i^T$, one has
\begin{multline}
  \label{eq:log_lik2}
  - \frac{2}{n}\log L(\bOmega_{\bx\by},\bOmega_{\by\by}) =
  - \log\left|\bOmega_{\by\by}\right| +
  \trace\left(\bS_{\by\by} \bOmega_{\by\by} \right) \\
  +     2\trace\left(    \bS_{\bx\by}\bOmega_{\by\bx}     \right)    +
  \trace(\bOmega_{\by\bx}\bS_{\bx\bx}                  \bOmega_{\bx\by}
  \bOmega_{\by\by}^{-1}) + \mathrm{cst.}
\end{multline}
This has been referred to  as a 'conditional Gaussian Graphical Model'
(cGGM) or 'partial Gaussian  Graphical Model' in the recent literature
\citep{2011_AoAS_yin,2012_JMLR_sohn,2012_JMA_lee,2012_arxiv_yuan}.  We
notice by comparing the cGGM \eqref{eq:cond_model} to the multivariate
regression model  \eqref{eq:reg_model_row} that $\bOmega_{\by\by}^{-1}
=  \bR \text{  and }  \bB =  -\bOmega_{\bx\by} \bOmega_{\by\by}^{-1}$.
Although  equivalent   to  \eqref{eq:reg_model_row},  the  alternative
parametrization \eqref{eq:cond_model}  shows two important differences
with  several implications.   First, in  light of  convex optimization
theory, % \citep{cvx_optim}
the  negative log-likelihood  \eqref{eq:log_lik}  can be  shown to  be
jointly   convex  in   $(\bOmega_{\bx\by},\bOmega_{\by\by})$  \citep[a
formal  proof  can   be  found  in][]{2012_arxiv_yuan}.   Minimization
problems  involving  \eqref{eq:log_lik} will  thus  be  amenable to  a
global solution,  which facilitates both  optimization and theoretical
analysis.    As   such,   the  conditional   negative   log-likelihood
\eqref{eq:log_lik}  will serve as  a building  block for  our learning
criterion.    Second,   it  unveils   new   interpretations  for   the
relationships  between input  and  output variables,  as discussed  in
\citet{2012_JMLR_sohn}: $\bOmega_{\bx\by}$ describes the \emph{direct}
relationships between  predictors and responses, the  support of which
we  are looking  for to  select relevant  interactions.  On  the other
hand,  $\bB$  entails  \emph{both  direct  and  indirect}  influences,
possibly  due  to  some  strong correlations  between  the  responses,
described by the covariance  matrix $\bR$ (or equivalently its inverse
$\bOmega_{\by\by}$).  To  provide additional insights  on cGGM, Figure
\ref{fig:model_insight}   illustrates    the   relationships   between
$\bB,\bOmega_{\bx\by}$ and $\bR$ in  two simple scenarios where $p=40$
and $q=5$.  Scenarios $a)$ and  $b)$ are discriminated by the presence
of a strong structure among the predictors. Still, the important point
to catch at this stage of the paper is how strong correlations between
outcomes can  completely ``mask'' the  direct links in  the regression
coefficients: the  stronger the correlation  in $\bR$, the less  it is
possible  to  distinguish  in   $\bB$  the  non-zero  coefficients  of
$\bOmega_{\bx\by}$.

\begin{figure}[htbp!]
  \centering
  \begin{tabular}{c@{\hspace{1cm}}c}
    \begin{tabular}{cccc}
      & $\bR_{\text{low}}$ & $\bR_{\text{med}}$ & $\bR_{\text{high}}$ \\
      & \includegraphics[scale=.1]{figures/R_low_cov}
      & \includegraphics[scale=.1]{figures/R_med_cov}
      & \includegraphics[scale=.1]{figures/R_high_cov} \\
      $\bOmega_{\bx\by}$ & $\bB_{\text{low}}$ & $\bB_{\text{med}}$ & $\bB_{\text{high}}$ \\
      \includegraphics[scale=.12]{figures/omega_cov}
      & \includegraphics[scale=.12]{figures/beta_low_cov}
      & \includegraphics[scale=.12]{figures/beta_med_cov}
      & \includegraphics[scale=.12]{figures/beta_high_cov}\\
    \end{tabular}
    &
    \begin{tabular}{cccc}
      & $\bR_{\text{low}}$ & $\bR_{\text{med}}$ & $\bR_{\text{high}}$ \\
      & \includegraphics[scale=.1]{figures/R_low_cov}
      & \includegraphics[scale=.1]{figures/R_med_cov}
      & \includegraphics[scale=.1]{figures/R_high_cov} \\
      $\bOmega_{\bx\by}$ & $\bB_{\text{low}}$ & $\bB_{\text{med}}$ & $\bB_{\text{high}}$ \\
      \includegraphics[scale=.12]{figures/omega_str}
      & \includegraphics[scale=.12]{figures/beta_low_str}
      & \includegraphics[scale=.12]{figures/beta_med_str}
      & \includegraphics[scale=.12]{figures/beta_high_str}\\
    \end{tabular} \\
    (a) & (b) \\
  \end{tabular}
  \caption{Toy examples to  illustrate the relationships between $\bB,
    \bOmega_{\bx\by}$ and  $\bR$ in the cGGM (better  seen in colors):
    on panel $a)$, a situation  with no particular structure among the
    predictors; on  panel $b)$, a strong  neighborhood structure.  For
    each panel,  we represent the  effect of stronger  correlations in
    $\bR$ on masking the direct links in $\bB$.}
  \label{fig:model_insight}
\end{figure}



%%% Local Variables:
%%% TeX-master: "JST_AOAS_main.tex"
%%% End:


==> arxiv_version/v1/ResMotif-K7.tex <==
\begin{tabular}{@{}l@{}} 
{\tt CTAAGCCAC} \\ 
\hline 
{\tt ~~TAGCCCC} \\ 
{\tt ~~GCGCCCC} \\ 
\end{tabular} & 
\begin{tabular}{@{}l@{}} 
{\tt GCATGTGAA} \\ 
\hline 
{\tt CCATATG} \\ 
{\tt ~~TTGTGAG} \\ 
\end{tabular} & 
\begin{tabular}{@{}l@{}} 
{\tt CATGTAATT} \\ 
\hline 
{\tt ~~TGTAAAT} \\ 
{\tt ~~TGTATAT} \\ 
\end{tabular} & 
\begin{tabular}{@{}l@{}} 
{\tt TGAAACA} \\ 
\hline 
{\tt TTAGACC} \\ 
{\tt TAAAAAG} \\ 
\end{tabular} \\ 
  \\ 
\begin{tabular}{@{}l@{}} 
{\tt TGATCGGCGCCGCACGACGA} \\ 
\hline 
{\tt ~~~~~~~~~~~GTATAAC} \\ 
{\tt ~~~~~~GCGCCGT} \\ 
\end{tabular} & 
\begin{tabular}{@{}l@{}} 
{\tt TGCTGGTT} \\ 
\hline 
{\tt ~GCTGGTT} \\ 
{\tt ~GCTGGTG} \\ 
\end{tabular} & 
\begin{tabular}{@{}l@{}} 
{\tt GATCGTATGATA} \\ 
\hline 
{\tt ~ATCATAT} \\ 
{\tt ~TTGGTAT} \\ 
\end{tabular} & 
\begin{tabular}{@{}l@{}} 
{\tt ACGCGAAAA} \\ 
\hline 
{\tt ~AACGAAA} \\ 
{\tt ~~ACGAAAA} \\ 
\end{tabular} \\ 
  \\ 
\begin{tabular}{@{}l@{}} 
{\tt CCATACATCAC} \\ 
\hline 
{\tt ~CATAGAC} \\ 
{\tt ~~~~ATATCAC} \\ 
\end{tabular} & 
\begin{tabular}{@{}l@{}} 
{\tt ATTGACCTGGTC} \\ 
\hline 
{\tt ~TCGACTT} \\ 
{\tt ~~CGACTTG} \\ 
{\tt ~~~~~CCAGCTT} \\ 
\end{tabular} & 
\begin{tabular}{@{}l@{}} 
{\tt GACTAGATATATATATTCGAT} \\ 
\hline 
{\tt ~~~~~~~~~~ATATATT} \\ 
{\tt ~~~~~~~CATATAT} \\ 
{\tt ~~~~~~~~~~ATATATG} \\ 
{\tt ~~~~~~~~ATATATA} \\ 
\end{tabular} & 


==> arxiv_version/v1/application_cookies.tex <==
\subsection{Near-Infrared Spectroscopy of Cookie Dough Pieces}

\paragraph*{Context} In Near-Infrared (NIR)  spectroscopy, one aims to
predict one or several quantitative variables from the NIR spectrum of
a given sample.  Each sampled spectrum  is a curve that represents the
level of reflectance  along the NIR region, that  is, wavelengths from
800 to 2500 nanometers (nm).  The quantitative variables are typically
related to  the chemical  composition of the  sample.  The  problem is
then to  select the most predictive  region of the spectrum,  that is,
some peaks  that show  good capabilities  for predicting  the response
variable(s).   This   is  known   as  a  ``calibration   problem''  in
Statistics.  NIR technique  is used in fields as  diverse as agronomy,
astronomy or pharmacology.  In such  experiments, it is likely to meet
very strong correlations and structure  along the predictors.  In this
perspective, \cite{2011_JASA_hans}  proposes to apply  the Elastic-Net
which  is  known  to  selected  simultaneously  groups  of  correlated
predictors. However  it is  not adapted to  the prediction  of several
responses  simultaneously.  In  \citet{data_cookies2}, an  interesting
wavelets regression  model with Bayesian inference  is introduced that
enters the multivariate regression model, just like our proposal.

\paragraph*{Description  of   the  dataset}  Continuing   the  example
mentioned in the introduction, we  consider the cookie dough data from
\citet{data_cookies1}.   The  data  with the  corresponding  test  and
training sets  are available  in the \textbf{fds}  \texttt{R} package.
After data pretreatments as  in \citet{data_cookies2}, we have $n=39$
dough  pieces in  the training  set: each  sample consists  in an  NIR
spectrum with $p=256$ points measured from  1380 to 2400 nm (spaced by
4  nm),  and   in  four  quantitative  variables   that  describe  the
percentages in fat, sugar flour and water of the dough piece.

\paragraph*{Structure specification} We would  like to account for the
neighborhood structure between the  predictors which is obvious in the
context of  NIR spectroscopy: since spectrum are  continuous curves, a
smooth neighborhood prior will  encourage predictors to be selected by
``wave'', which seems more  satisfactory than isolated peaks. Thus, we
naturally  define  $\bL$ by  means  of  the  first forward  difference
operator \eqref{eq:first_order_diff}.  We also tested higher orders of
the operator  to induce a stronger  smoothing effect, but  they do not
lead to dramatic changes in term of PE and we omit them.  Order $k$ is
simply obtained  by powering the first order  matrix.  Such techniques
have  been  studied  in  a structured  $\ell_1$-penalty  framework  in
\cite{2009_SIAM_Kim,2011_AOS_Tibshirani}  and is known  as \emph{trend
  filtering}.   Our  approach  is   different,  though:  it  enters  a
multivariate framework  and it is  based on a  smooth $\ell_2$-penalty
coupled with the $\ell_1$-penalty for selection.

\paragraph*{Results}  The  predictive  performances  of  a  series  of
regression  techniques   are  compared  in   Table  \ref{Tab:Cookies},
evaluated on the same test set.
\begin{table}[htbp!]
  \centering
  \begin{small}
    \begin{tabular}{l|rrrr}
      \hline
      \textit{\textsf{Method}} & \textit{\textsf{fat}} & \textit{\textsf{sucrose}} & \textit{\textsf{flour}} & \textit{\textsf{water}} \\
      \hline
      {Stepwise MLR} & .044 & 1.188 & .722 & .221 \\
      {Decision theory} & .076 & .566 & .265 & .176 \\
      {PLS} & .151 & .583 & .375 & .105 \\
      {PCR} & .160 & .614 & .388 & .106 \\
      {Wavelet Regression} & .058 & .819 & .457 & .080 \\
      {LASSO} & .044 & .853 & .370 & .088 \\
      {group-LASSO} & .127 & .918 & .467 & .102 \\
      {MRCE} & .151 & .821 & .321 & .081 \\
      {Structured E-net} & .044 & .596 & .363 & .082 \\
      {SPRING} (CV) & .065 & .397 & .237 & .083 \\
      {SPRING} (BIC)& .048 & .389 & .243 & .066 \\
  \end{tabular}
  \end{small}
  \caption{Prediction error for the cookie dough data.}
  \label{Tab:Cookies}
\end{table}
The first four rows (namely stepwise multivariate regression, Bayesian
decision theory approach, Partial Least Square and Principal Component
Regression) correspond to  calibration methods originally presented in
\citet{data_cookies2};  row  five  (Bayesian  Wavelet  Regression)  is
\citeauthor{data_cookies2}'s original  proposal; the remainder  of the
table is due  to our own analysis.  We observe  that, on this example,
SPRING  achieves  extremely  competitive  results.  The  BIC  performs
notably well as a model selection criterion. 
\begin{figure}[htbp!]
  \centering
  \begin{tabular}{@{}c@{}c@{}c@{}c@{}}
    LASSO & group-LASSO &  Structured Elastic-Net & MRCE \\
    \includegraphics[width=.25\textwidth]{figures/cookies_beta_lasso} & 
    \includegraphics[width=.25\textwidth]{figures/cookies_beta_grplasso} &
    \includegraphics[width=.25\textwidth]{figures/cookies_beta_senet} &
    \includegraphics[width=.25\textwidth]{figures/cookies_beta_mrce} \\
    \multicolumn{4}{c}{Wavelength range (nanometer)}
  \end{tabular}
  \caption{Parameters estimated by the penalized regression methods for
    the cookie data}
  \label{Fig:Cookies2}
\end{figure}
% \begin{figure}[htbp!]
%   \centering
%   \begin{tabular}{@{\hspace{1cm}}cc}
%     LASSO & group-LASSO  \\
%     \includegraphics[width=.29\textwidth]{figures/cookies_beta_lasso} & 
%     \includegraphics[width=.29\textwidth]{figures/cookies_beta_grplasso} \\
%     Structured Elastic-Net & MRCE \\
%     \includegraphics[width=.29\textwidth]{figures/cookies_beta_senet} &
%     \includegraphics[width=.29\textwidth]{figures/cookies_beta_mrce} \\
%     \multicolumn{2}{c}{Wavelength range (nanometer)}
%   \end{tabular}
%   \caption{Parameters estimated by the penalized regression methods for
%     the cookie data}
%   \label{Fig:Cookies2}
% \end{figure}
Figure \ref{Fig:Cookies2}  shows the regression  coefficients adjusted
with  the  penalized regression  techniques:  apart  from LASSO  which
selects very isolated  (and unstable) wavelengths, non-zero regression
coefficients  are very spread,  and therefore  hard to  interpret.  As
expected,  the  multitask group-Lasso  activates  the same  predictors
across the  responses, which is  not a good  idea when looking  at the
predictive performance in Table \ref{Tab:Cookies}.  On the other hand,
back to  the beginning of the paper  in Figure~\ref{Fig:Cookies1}, the
direct effects  selected by SPRING with BIC  define predictive regions
specific of  each response which are well  suited for interpretability
purpose.

%%% Local Variables:
%%% TeX-master: "JST_AOAS_main.tex"
%%% End:


==> arxiv_version/v1/application_linkage.tex <==
\subsection{Multi-trait Genomic Selection in Brassica napus}

\paragraph{Context} Genomic selection aims at predicting  one or several phenotypes 
based on the information of genetics markers. In plant and animal
genetics,  deriving an  accurate prediction  of complex  traits  is of
major importance for the  early detection and selection of individuals
of  high   genetic  value.  Due   to  the  continued   advancement  of
high-throughput   genotyping  and  sequencing   technologies,  genetic
information is now  available at low cost, whereas acquiring  trait  information  remains expensive. A
typical experiment will only contain a few hundreds
of  phenotyped  individuals genotyped for thousands of markers.
% in the  form of thousands of markers
% On  the  other  hand, acquiring  trait  information  remains
%expensive, and a  typical experiment will only contain  a few hundreds
%of  phenotyped  individuals.
% This  leads to the  classical ``high  dimensional setting''  where the
% number  of features  is much  higher than  the number  of observations
% available for training.  Due to this high dimensional
% setting,
Consequently regularization methods such  as ridge or Lasso regression
or  their Bayesian  counterparts  have been  proposed  since the  very
beginning  of  genomic selection  \citep{LosCampos12}.  Still, in  most
studies only  single trait genomic selection  is performed, neglecting
correlations  between  phenotypes%    and  leading  to  poor  prediction
% performance
.   Moreover,  little attention  has  been  devoted to  the
development   of  regularization   methods  including   prior  genetic
knowledge.

\paragraph*{Description of the dataset} We consider the \emph{Brassica
  napus}     dataset    described    in     \citet{Bnapus_data}    and
\citet{Bnapus_map}.   Data consists  in  $n=103$ double-haploid  lines
derived from 2 parent cultivars,  `Stellar' and `Major', on which $p =
300$ genetic markers and  $q=8$ traits (responses) were recorded. Each
marker is a 0/1 covariate with $x_i^j=0$ if line $i$ has the 'Stellar'
allele  at marker $j$,  and $x_i^j=1$  otherwise. Traits  included are
percent winter survival  for 1992, 1993, 1994, 1997  and 1999 (surv92,
surv93, surv94,  surv97, surv99, respectively), and  days to flowering
after no vernalization (flower0), 4 weeks vernalization (flower4) or 8
weeks vernalization (flower8).

\paragraph{Structure specification} 
In a biparental line population, correlation between 2 markers depends
on their genetic distance defined  in terms of recombination fraction.
As a consequence,  one expects adjacent markers on the  sequence to be
correlated, yielding similar direct  relationships with the phenotypic
traits. Noting $d_{12}$ the genetic distance between markers $M_1$ and
$M_2$, one has $\text{cor}(M_11,M_22)  = \rho^{d_{12}}$, where $\rho =
.98$\footnote{This value  directly arises  from the definition  of the
  genetic  distance itself.}.   The covariance  matrix $\bL^{-1}$  can
hence  be  defined  as  $\bL_{ij}^{-1}  =  \rho^{d_{ij}}$.   Moreover,
assuming recombination events are  independent between $M_1$ and $M_2$
on one hand, and $M_2$ and $M_3$  on the other hand, one has $d_{13} =
d_{12} + d_{23}$ and matrix $\bL^{-1}$ exhibits an inhomogeneous AR(1)
profile.  As a consequence, $\bL$ is tridiagonal with general elements
\begin{eqnarray*}
  w_{i, i} & = & \frac{1 - \rho^{2d_{i-1, i} + 2d_{i, i+1}}}{(1 - \rho^{2d_{i-1, i}})(1 - \rho^{2d_{i, i+1}})}, \\
  w_{i, i+1} & = & \frac{-\rho^{d_{i, i+1}}}{1 - \rho^{2d_{i, i+1}}}
\end{eqnarray*}
and $w_{i,j} =  0$ if $|i-j| > 1$. For the  first (resp. last) marker,
the distance $d_{i-1, i}$ (resp. $d_{i, i+1}$) is infinite.

\paragraph{Results}  We apply SPRING  to study  the influence  of each
marker on the traits and compare its predictive performance with these
of its competitors.   PE is estimated by randomly  splitting the $103$
samples  into training  and test  sets with  sizes 93  and  10. Before
adjusting the models, we first  scale the outcomes on the training and
test sets  to facilitate interpretability.  Five-fold cross-validation
is  used on the  training set  to choose  the tuning  parameters.  Two
hundred random samplings of the  test and training sets were conducted
to estimate the PE given in Table \ref{Tab:BNapus}.
\begin{table*}[htp!]
  \centering
  \begin{small}
    \begin{tabular}{l|rrrrr}
    \hline
    \textit{\textsf{Method}} &
    \textit{\textsf{surv92}}  &
    \textit{\textsf{surv93}}  &
    \textit{\textsf{surv94}}  &
    \textit{\textsf{surv97}}  &
    \textit{\textsf{surv99}} \\
    \hline
    {LASSO} & .730 (.011) & .977 (.009) & .943 (.010) & .947 (.009) & .916
    (.010) \\

    {S. Enet}  & \textbf{.697} (.011) &  .987 (.009) & .941  (.011) & .945
    (.009) & .911 (.010) \\

    {MRCE} & .759 (.010)  & \textbf{.919} (.003) & 917 (.006) & \textbf{.924} (.004) & .926
    (.006) \\

    {SPRING} &  .724 (.010) &  .948 (.008) & \textbf{.848}  (.010) & .940  (.006) &
    \textbf{.907} (.009) \\
  \end{tabular}
  \medskip

  \begin{tabular}{l|rrr}
    \hline
    \textit{\textsf{Method}} &
    \textit{\textsf{flower0}} &
    \textit{\textsf{flower4}} &
    \textit{\textsf{flower8}} \\
    \hline
    {LASSO} & .609 (.011) & .501 (.011) & .744 (.011) \\

    {S. Enet} & .577 (.011) & .478 (.010) & .727 (.012) \\

    {MRCE} & .591 (.011) & .479 (.011) & .736 (.011) \\

    {SPRING} & \textbf{.489} (.010) & \textbf{.419} (.009) & \textbf{.616} (.012) \\
  \end{tabular}

  \end{small}
  \caption{Estimated  prediction error  for the  \emph{Brassica napus}
    data (standard error in parenthesis)}
  \label{Tab:BNapus}
\end{table*}
All  methods  provide similar  results  although  SPRING provides  the
smallest  error   for  half   of  the  traits.    A  picture   of  the
between-response covariance  matrix estimated with SPRING  is given in
Figure \ref{Fig:BNapusCovar}.   In this context,  this matrix reflects
the correlation  between the  traits that are  either explained  by an
unexplored  part  of the  genotype,  by  the  environment or  by  some
interaction  between the two.   The residuals  of the  flowering times
exhibit  strong  correlations,  whereas  the correlation  between  the
survival rates are weak. It also shows that the survival traits have a
larger residual  variability than  the flowering traits,  suggesting a
higher sensitivity to environmental conditions.
\begin{figure}[htpb!]
  \includegraphics[scale=.35]{figures/brassica_cor}
  \caption{Brassica study: residual covariance estimation \label{Fig:BNapusCovar}}
\end{figure}

We  then  turn  to  the  effects  of  each  marker  on  the  different
traits. The left panels of Figure \ref{Fig:BNapusCoefs} gives both the
regression  coefficients (top)  and the  direct effects  (bottom). The
gray zones correspond  to chromosomes 2, 8 and  10, respectively.  The
exact location  of the markers within these  chromosomes are displayed
in the right panels, where the  size of the dots reflects the absolute
value of the  regression coefficients (top) and of  the direct effects
(bottom).
\begin{figure*}[htbp!]
   \centering
   \includegraphics[width=\textwidth]{figures/brassica_fits}
   \caption{Brassica Study: direct and indirect genetic effects of the
     markers on the  traits estimated by SPRING\label{Fig:BNapusCoefs}
     (better seen in color).}
\end{figure*}
The  interest of  considering  direct effects  rather than  regression
coefficients appears  clearly here, looking for  example at chromosome
2.  Three  large overlapping regions  are observed in  the coefficient
plot, for each flowering trait. A straightforward interpretation would
suggest that  the corresponding region controls  the general flowering
process. The  direct effect  plot allows to  go deeper and  shows that
these  three  responses are  actually  controlled  by three  separated
sub-regions within  this chromosome. The confusion  in the coefficient
plot only  results from the  strong correlations observed  between the
three flowering traits.

%%% Local Variables:
%%% TeX-master: "JST_AOAS_main.tex"
%%% End:


==> arxiv_version/v1/application_motif.tex <==
\subsection{Selecting regulatory motif from multiple microarrays}

\paragraph{Context} In genomics, the  expression of genes is initiated
by transcription factors that bind to the DNA upstream from the coding
regions, called {\it regulatory  regions}.  This binding occurs when a
given   factor   recognizes   a   certain  (small)   sequence   called
transcription  factor binding  site  or {\it  regulatory motif}.   The
presence of a  regulatory motif in the regulatory region  of a gene is
therefore   required   to   launch  the   transcriptional   machinery.
Conversely, genes  hosting the same  regulatory motif will  be jointly
expressed under certain conditions.  As the binding relies on chemical
affinity, some degeneracy can be tolerated in the motif definition and
motifs similar  up to small  variations may share the  same functional
properties \citep[see, e.g.][]{2012_GB_Lajoie}.

We  are interested  in the  detection of  such regulatory  motifs, the
presence of  which controls genes  expression profile. To this  aim we
try to establish a relation between  the expression level of all genes
across a  series of  conditions with the  content of  their respective
regulatory regions in terms of motifs. In this context, we expect $i)$
the set  of influential motifs to  be small for each  condition, $ii)$
the influent motifs  for a given condition to  be degenerated versions
of each other,  and $iii)$ the expression under  similar conditions to
be controlled by the same motifs.

\paragraph*{Description of the  dataset} In \cite{gasch2000genomic}, a
series  of  microarray  experiments   are  conducted  on  yeast  cells
(\textit{Saccharomyces cerevisae}).   Among these assays,  we consider
12  time-course  experiments profiling  $n=5883$  genes under  various
environmental  changes as  listed in  Table \ref{tab:exp_time_course}.
These expression sets form  12 potential response matrices $\bY$ whose
number of column corresponds to the number of time points.
\begin{table}[htbp!]
  \centering
  \begin{tabular}{lc|c@{\hspace{2.5em}}c@{\hspace{2.5em}}c}
    \textit{Experiment}     &     \textit{\#     time    point}     &
    \multicolumn{3}{c}{\it \# motifs selected by SPRING} \\
    \cline{3-5} 
    & & $k=7$ & $k=8$ & $k=9$ \\
    \hline 
    Heat shock & 8 & 30 & 68 & 43 \\
    Shift from 37\degres to 25 \degres C & 5 & 3 & 11 & 33 \\
    Mild Heat shock & 4 & 24 & 13 & 23 \\
    Response to $\text{H}_2 \text{O}_2$ & 10 & 15 & 10 & 21 \\
    Menadione Exposure & 9 & 16 & 1 & 7 \\
    DDT exposure 1 & 8 & 15 & 10 & 30 \\
    DDT exposure 2 & 7 & 11 & 33 & 21 \\
    Diamide treatment & 8 & 45 & 25 & 35 \\
    Hyper-osmotic shock & 7 & 36 & 24 & 15 \\
    Hypo-osmotic shock & 5 & 20 & 8 & 29 \\
    Amino-acid starvation & 5 & 47 & 30 & 39 \\
    Diauxic Shift & 7 & 16 & 14 & 20 \\
    \hline 
    \multicolumn{2}{l}{\it total number of unique motif inferred} & 87 & 82 & 72 \\
  \end{tabular}
  \caption{Time-course data from \cite{gasch2000genomic} considered for regulatory motif discovery}
  \label{tab:exp_time_course}
\end{table}
Concerning  the predictors,  we consider  the set  of all  motifs with
length  $k$  formed with  the  four  nucleotides,  that is  $\clM_k  =
\set{A,C,G,T}^k$.  There are $p =  |\clM_k| = 4^k$ such motifs. Unless
otherwise stated, the motifs in $\clM$ are lined up in lexicographical
order e.g.,  when $k=2$,  $AA,AC,AG,AT,CA,CC,\dots$ and so  on.  Then,
the $n\times p$ matrix of  predictors $\bX$ is filled such as $X_{ij}$
equals the occurrence  count of motif $j$ in  the regulatory region of
gene $i$.%  This can be  straightforwardly done using the FASTA files of
% the regulatory region of each gene which are publicly available on the
% web.

\paragraph{Structure  specification} As  we expect  influential motifs
for a  given condition  to be degenerated  versions of each  other, we
would  like  to take  this  information  into  account in  the  matrix
$\bL$.  To do  so, we  first measure  the similarity  between  any two
motifs from $\clM_k$ with the Hamming defined as
\begin{equation*}
 \label{eq:hamming_def}
 \forall a,b\in\clM_k, \quad \mathrm{dist}(a,b) = \text{card}\{i:a_i\neq b_i\}.
\end{equation*}
For a distance of interest $0\leq\ell\leq k$, we further define the $m
\times              m$             \emph{symmetric}             matrix
$\bD^{k,\ell}=(d^{k,\ell}_{ab})_{a,b\in\clM_k}$   so  as   each  entry
$d^{k,\ell}_{ab}$ indicates  if the Hamming distance is  less or equal
to $\ell$. We refer to this  distance for fixed value of $\ell$ as the
\textit{$\ell$-distance matrix}:
\begin{equation*}
 \label{eq:distance_matrix}
 \forall a,b\in\clM_k, \quad d^{k,\ell}_{ab} = \left\{
 \begin{array}{ll}
 1 & \text{if $\mathrm{dist}(a,b) \leq \ell$} \\
 0 & \text{otherwise.} \\
 \end{array}\right.
\end{equation*}

For motifs in $\clM_k$ lined up in lexicographical order, manipulation
of $\bD$  greatly simplifies  as motifs  can be mapped  to the  set of
natural integers  $\mathbb{N}$.  The following  proposition shows that
$\bD^{k,\ell}$ can  be computed  recursively for increasing  values of
$k,\ell$ at the cost of a simple Kronecker product.
\begin{proposition} \label{prop:computeDkl}
For $\ell\leq k$, and considering that
\begin{equation*}
 \label{eq:D10_D11}
 \bD^{1,0} =
 \kbordermatrix{
 & A & C & G & T \\
 A & 1 & & & \\
 C & & 1 & & \\
 G & & & 1 & \\
 T & & & & 1 \\
 }, \quad
 \bD^{1,1} =
 \kbordermatrix{
 & A & C & G & T \\
 A & 1 & 1 & 1 & 1 \\
 C & 1 & 1 & 1 & 1 \\
 G & 1 & 1 & 1 & 1 \\
 T & 1 & 1 & 1 & 1 \\
 },
\end{equation*}
then the  $\ell$-distance matrix between  motifs of size $k+1$  can be
expressed as a function of distance between motifs of size $k$ as
 \begin{equation*}
 \label{eq:reck_D}
 \bD^{{k+1},\ell} = \left(\bD^{1,0}\otimes\bD^{k,\ell}\right) \vee
 \left(\bD^{1,1}\otimes\bD^{k,\ell-1}\right),
 \end{equation*}
 where $\vee$ is the OR operator and $\ell\geq 1$. Similarly, for
 values of $\ell:\ell+1\leq k$,
 \begin{equation*}
 \label{eq:recl_D}
 \bD^{k,\ell+1} = \left(\bD^{1,0}\otimes\bD^{k-1,\ell}\right) \vee
 \left(\bD^{1,1}\otimes\bD^{k,\ell}\right).
 \end{equation*}
\end{proposition}

$\bD^{k,\ell}$ can be viewed as the  adjacency matrix of a graph where
the nodes are the motifs and where  an edge is present between 2 nodes
when the 2 motifs  are at a Hamming distance less  or equal to $\ell$.
We finally  use the Laplacian  of this  graph as a  structuring matrix
$\bL^{k,\ell}=(\ell^{k,\ell}_{ab})_{a,b\in\clM_k}$, that is
\begin{equation}
 \label{eq:laplacian}
 \ell^{k,\ell}_{ab} =
 \begin{cases}
 \sum_{c\in\clM_k} d^{k,\ell}_{ac} & \text{if } a = b, \\
 -1 & \text{if } d^{k,\ell}_{ab} = 1, \\
 0 & \text{otherwise}.
 \end{cases}
\end{equation}
{Note that we came across a similar proposal by \cite{li2010learning}
  in the context of sparse, structured PLS. The derivation is
  different though, and the objective of this method is not the
  selection of motifs but of family of motifs via the compression
  performed by the PLS.  }

\paragraph{Results}~  We apply  our methodology  for candidate  motifs
from  $\clM_7,\clM_8$ and  $\clM_9$, which  result in  three lists  of
putative motifs having a direct effect on gene expression.  Due to the
very large  number of potential  predictors that comes with  a sparser
matrix $\bX$  when $k$  increases, we first  perform a  screening step
that keep  the $5,000$ motifs  with the highest  marginal correlations
with  $\bY$.   Second,  SPRING  is   fitted  on  each  of  the  twelve
time-course experiments described  in Table \ref{tab:exp_time_course}.
The selection of $(\lambda_1,\lambda_2)$ is  performed on a grid using
the BIC \eqref{eq:pen_crit} rather than the cross-validation approach,
since we clearly face a variable selection problem.  At the end of the
day,   the  three   lists  corresponding   to  $k=7,8,9$   comprehends
respectively 87, 82 and 72 motifs,  for which at least one coefficient
in the associated  row $\widehat{\bOmega}_{\bx\by}(j,\cdot)$ was found
non-null  for some  of the  twelve experiments,  as detailed  in Table
\ref{tab:exp_time_course}.

To assess the relevance of  the selected motifs, we compared them with
the {\tt MotifDB} patterns available in Bioconductor (\cite{motifdb}),
where known transcription factor binding sites are recorded. There are
453 such reference motifs with size varying from 5 to 23 nucleotides.
% \corSR{To account for degeneracy, a SFBS with length $\ell$ is
% represented  as  position-specific   scoring  matrix  ${\bf  P}  =
% [p_{au}]$  with  dimension  $4   \times  \ell$,  where  $p(a,  u)$
% represents the  probability for the  nucleotide $a \in \{A,  C, G,
% T\}$  to occur  at  position $u  \in  \{1, \dots,  \ell\}$ of  the
% binding site. For each selected  motif ${\bf m}_i$ and each JASPAR
% matrix  ${\bf P}_j$  ($j  = 1,  \dots  , 53$),  we calculated  the
% similarity   score  $T_{ij}   =  \max_{0   \leq  u   \leq  \ell-k}
% \sum_{v=1^k}  \log p_j({\bf  m}_i(v), u+v)$.  A  null distribution
% $\widehat{F}_i$ for this score  was then estimated for each matrix
% ${\bf P}_j$, computing  the same score for all  motifs with length
% $k$  present  in the  set  of  regulatory  regions.  We  furthered
% defined     a     pseudo      $p$-value     $P_{ij}$     as     $1
% -\widehat{F}_i(T_{ij})$. }{}
Consider the case  of $k=7$ for instance: among  the 87 SPRING motifs,
62 match one  \texttt{MotifDB} pattern each and 25  are clustered into
11 \texttt{MotifDB} patterns as depicted in Table \ref{Tab:MotifDB}.
\begin{table}
  \begin{center}
    \begin{tabular}{@{}cccc@{}}
      \input{ResMotif-K7.tex}
    \end{tabular}
    \caption{Comparison    of     SPRING    selected    motifs    with
      \texttt{MotifDB}   patterns.   Each   cell  corresponds   to   a
      \texttt{MotifDB}  pattern (top)  compared  to a  set of  aligned
       SPRING motifs with size 7 (down). \label{Tab:MotifDB}}
  \end{center}
\end{table}
As  seen in  this table,  the clusters  of motifs  selected by  SPRING
correspond  to sets  of variants  of  a same  pattern. These  clusters
consist of motifs  that are close according to  the similarity encoded
in  the structure  matrix $\bL$.   In this  example, the  framework we
propose enabled  us to  orient the regression  problem to  account for
motif degeneracy  and helped us  to select motifs that  are consistent
known  binding sites.   This  example illustrates  the flexibility  of
SPRING,  which  allows  to  use  domain-specific  definitions  of  the
structure between the predictors.

% \begin{table}
%   \begin{center}
%     \begin{tabular}{llll}
%       \input{ResMotif-K8.tex}
%     \end{tabular}
%     \caption{Comparison of SPRING selected motifs with MotifDB patterns. Each cell of the table corresponds to a MotifDB pattern (top) compared to a set of aligned SPRING motifs with length 8 (down). \label{Tab:MotifDB}}
%   \end{center}
% \end{table}

% \begin{table}
%   \begin{center}
%     \begin{tabular}{llll}
%       \input{ResMotif-K9.tex}
%     \end{tabular}
%     \caption{Comparison of SPRING selected motifs with MotifDB patterns. Each cell of the table corresponds to a MotifDB pattern (top) compared to a set of aligned SPRING motifs with length 9 (down). \label{Tab:MotifDB}}
%   \end{center}
% \end{table}

%%% Local Variables:
%%% TeX-master: "JST_AOAS_main.tex"
%%% End:


==> arxiv_version/v1/crit_learn.tex <==
\subsection{Structured regularization with underlying sparsity}
\label{Sec:crit_learn}

Our regularization scheme starts  by considering some structural prior
information as for the  relationships between the coefficients. We are
typically thinking of a situation where similar inputs are expected to
have  similar direct relationships  with the  outputs. Right  panel of
Figure  \ref{fig:model_insight}   represents  a  cartoon   of  such  a
situation,  where  there  exists  an  extreme  neighborhood  structure
between the  predictors.  This depicts  a pattern that acts  along the
rows of $\bB$ or  $\bOmega_{\bx\by}$ as substantiated by the following
Bayesian point of view.

\paragraph*{Bayesian interpretation}  Suppose the similarities  can be
encoded  into  a  matrix  $\bL$.   Our  aim is  to  account  for  this
information  when learning the  coefficients.  The  Bayesian framework
provides  a  convenient  setup   to  define  the  way  the  structural
information  should  be accounted  for.   In  the  single output  case
\citep[see, e.g.][]{MaR07},  a conjugate  prior for $\bbeta$  would be
$\mathcal{N}(\bzr, \bL^{-1})$.   Combined with the  covariance between
the outputs, this gives
\begin{equation*}
  \vec(\bB) \sim \mathcal{N}(\bzr,\bR \otimes \mathbf{L}^{-1}), 
\end{equation*}
where $\otimes$ is the Kronecker  product. By properties of the $\vec$
operator, % we have
% \begin{multline*}
%   \var(\vec(\bB))  = \var(\vec(-\bOmega_{\bx\by}\bR)) = \var((\bR\otimes\bI_p)\vec(\bOmega_{\bx\by}))\\
%   =
%   (\bR\otimes\bI_p)\var(\vec(\bOmega_{\bx\by}))(\bR\otimes\bI_p)
%   \\ = 
%   (\bR\otimes\bI_p)(\bR^{-1}\otimes\mathbf{L}^{-1})(\bR\otimes\bI_p) = \bR\otimes\mathbf{L}^{-1}.
% \end{multline*}
% Thus the prior on $B$
this can be stated straightforwardly as
\begin{equation*}
  \vec(\bOmega_{\bx\by}) \sim \mathcal{N}(\bzr,\bR^{-1} \otimes \mathbf{L}^{-1})
\end{equation*}
for the direct links. Choosing such a prior results in
\begin{equation*}
  \label{eq:log_lik_prior}
  \log \prob(\bOmega_{\bx\by}|\mathbf{L},\bR) =  
  \frac{1}{2}\trace\left(\bOmega_{\bx\by}^T             \mathbf{L}
    \bOmega_{\bx\by} \bR \right)
  + \mathrm{cst.}
\end{equation*}

\paragraph*{Criterion} Through  this argument, we  propose a criterion
with two  terms to regularize the  conditional negative log-likelihood
\eqref{eq:log_lik}:  first,  a  smooth   trace  term  relying  on  the
available structural information  $\mathbf{L}$; and second, a $\ell_1$
norm that  encourages sparsity  among the direct  links. We  write the
criterion  as  a  function of  $(\bOmega_{\bx\by},  \bOmega_{\by\by})$
rather than $(\bOmega_{\bx\by}, \bR)$,  although equivalent in term of
estimation,  since the  former  leads to  a  convex formulation.   The
optimization problem turns to the minimization of
\begin{multline}
  \label{eq:objective}
  % (\hat{\bOmega}_{\bx\by},\hat{\bOmega}_{\by\by})
  % = \argmin_{\bOmega_{\bx\by},\bOmega_{\by\by}} J(\bOmega_{\bx\by},\bOmega_{\by\by}),
  % \quad \text{where }
  J(\bOmega_{\bx\by},\bOmega_{\by\by})        = \\      -\frac{1}{n}\log
  L(\bOmega_{\bx\by},\bOmega_{\by\by})      +      \frac{\lambda_2}{2}
  \trace\left(\bOmega_{\by\bx}\mathbf{L}\bOmega_{\bx\by}\bOmega_{\by\by}^{-1}\right)
  + \lambda_1 \|\bOmega_{\bx\by}\|_1.
\end{multline}
Simple  convexity arguments and requirements for positive definiteness of the Hessian of
\eqref{eq:objective} lead to the following proposition, whose proof is
omitted.

\begin{proposition}\label{prop:existence_uniqueness} The objective
  function     \eqref{eq:objective}    is     jointly     convex    in
  $(\bOmega_{\bx\by},\bOmega_{\by\by})$ and admits at least one global
  minimum  which  is  unique  when  $n\geq  q$  and  $(\lambda_2\bL  +
  \bS_{\bx\bx})$ is positive definite.
\end{proposition}

%  \begin{proof}   Thanks  to  the   convexity  of  \eqref{eq:log_lik}
%   \citep[see][]{2012_arxiv_yuan} combined  with the two regularizers
%   which are convex norms,  \eqref{eq:objective} is jointly convex in
%   $(\bOmega_{\bx\by},\bOmega_{\by\by})$ when $(\lambda_1,\lambda_2)$
%   are fixed, which means that a global minimum exists.

%   In fact,  as soon as  $(\lambda_2\bL + \bS_{\bx\bx})$  is positive
%   definite and  $n\geq q$, it is  not difficult to  see, although we
%   omit the details, that the problem is strictly convex and thus the
%   solution to \eqref{eq:objective} is unique.
% \end{proof}

% Introducing   the  notation  $   \hat{\bSigma}_{\bx\bx}^{\lambda_2}  =
% \bS_{\bx\bx}+ \lambda_2\bL$, this writes
% \begin{multline}
%   \label{eq:objective}
%   J(\bOmega_{\bx\by},\bOmega_{\by\by})               =               -
%   \frac{1}{2}\log\left|\bOmega_{\by\by}\right| +
%   \frac{1}{2}\trace\left(\bS_{\by\by} \bOmega_{\by\by} \right) \\
%   +     \trace\left(     \bS_{\bx\by}\bOmega_{\by\bx}    \right)     +
%   \frac{1}{2}\trace\Big(\bOmega_{\by\bx}
%   \hat{\bSigma}_{\bx\bx}^{\lambda_2}                   \bOmega_{\bx\by}
%   \bOmega_{\by\by}^{-1}\Big) + \lambda_1 \|\bOmega_{\bx\by}\|_1,
% \end{multline}
% which gives  additional insights about  the effect of  the structuring
% prior:  it  performs  a   mixture  between  the  empirical  covariance
% $\bS_{\bx\bx}$  and the structure  $\bL$ similar  to this  obtained in
% Bayesian linear  regression.

\subsection{Connection to other sparse regression methods}

To get more insight about our model and to facilitate connections with
existing   approaches,  we   shall   write   the  objective   function
\eqref{eq:objective}  as  a   penalized  \emph{univariate}  regression
problem.       This      amounts      to      ``vectorize''      model
\eqref{eq:cond_model_mat} with respect to $\bOmega_{\bx\by}$, i.e., to
write  the objective  as  a  function of  $(\bomega,\bOmega_{\by\by})$
where  $\bomega=\vec(\bOmega_{\bx\by})$.    This  is  stated   in  the
following  proposition,  which  can be  derived  from  straightforward
matrix algebra,  as proved in Appendix  Section \ref{sec:vec_obj}. The
main interest of this proposition  will become clear when deriving the
optimization  procedure  to   minimize  \eqref{eq:objective},  as  the
optimization  problem  when $\bOmega_{\by\by}$  is  fixed  turns to  a
generalized Elastic-Net  problem.  Remark  that we use  $\bA^{1/2}$ to
denote  the square  root  of  a matrix,  obtained  for  instance by  a
Cholesky  factorization  in  case  of a  symmetric  positive  definite
matrix.
\begin{proposition} \label{prop:vec_obj} \hspace{-2ex} Let $\bomega =
  \vec(\bOmega_{\bx\by})$.    An    equivalent    vector    form    of
  \eqref{eq:objective} is
  \begin{multline*}
    \label{eq:objective_vec}
    J(\bomega,      \bOmega_{\by\by})     =      -\frac{1}{2}     \log
    |\bOmega_{\by\by}|   +    \frac{1}{2   n}   \left\|\tilde{\by}   +
      \tilde{\bX} \bomega
    \right\|_2^2  +  \frac{\lambda_2}{2}  \bomega^T  \left(\bOmega_{\by\by}^{-1}  \otimes  \bL
    \right) \bomega + \lambda_1 \left\| \bomega \right\|_1,
  \end{multline*}
  where the $n\times q$ dimensional vector $\tilde{\by}$ and the $n q
  \times p q$ dimensional matrix $\tilde{\bX}$ depends on
  $\bOmega_{\by\by}$ such that
  \begin{equation*}
    \tilde{\by} = \vec(\bY  \bOmega_{\by\by}^{1/2}), \quad \tilde{\bX} =
    \left(\bOmega_{\by\by}^{-1/2} \otimes \bX\right).
  \end{equation*}
\end{proposition}

When  there  is  only  one  response,  that  is,  when  $q=1$,  direct
connections  can be  made with  various existing  approaches. In  such
cases,   the  variance-covariance   matrix  $\bR$   and  its   inverse
$\bOmega_{\by\by}$ turn to scalars, respectively denoted by $\sigma^2$
and    $\rho^2$,   with    $\sigma=1/\rho$.    Applying    Proposition
\ref{prop:vec_obj}, the objective \eqref{eq:objective} writes
\begin{equation}
  \label{eq:criteria_univariate}
  J(\bomega, \rho) = -\log(\rho) + \frac{1}{2n}\|\rho \by +
  \bX \bomega/(\rho)\|_2^2 + \frac{\lambda_2}{2\rho^2} \bomega^T 
  \bL  \bomega  +  \lambda_1  \|\bomega\|_1.
\end{equation}
Its  counterpart  in term  of  the parametrization  $(\bbeta,\sigma)$,
% where $\bbeta = -\bomega \sigma^2 = -\bomega/(\rho^2)$
is
\begin{equation}
  \label{eq:criteria2_univariate}
  J(\bbeta,\sigma) =             \log(\sigma)             +
  \frac{1}{2n\sigma^2}\left\|\by-\bX\bbeta       \right\|_2^2      +
  \frac{\lambda_2}{2\sigma^2}             \bbeta\bL\bbeta            +
  \frac{\lambda_1}{\sigma^2} \|\bbeta \|_1.
\end{equation}
We recognize in  \eqref{eq:criteria2_univariate} the log-likelihood of
a  ``usual''  linear  model  with  Gaussian  noise,  unknown  variance
$\sigma^2$  and  regression parameters  $\bbeta$,  plus  a mixture  of
$\ell_1$ and $\ell_2$ norm,  a.k.a, an elastic-net penalization.  This
is the univariate analog  of \eqref{eq:reg_model_row}, whose criterion
\eqref{eq:criteria_univariate}   is   the   convex   reparametrizaton.
Criterion  \eqref{eq:criteria2_univariate} entail  many regularization
schemes found in  the literature: assuming that $\sigma$  is known, we
recognize   ridge    regression   when   $\lambda_1=0$,    the   Lasso
\citep{1996_JRSSB_tibshirani} when $\lambda_2=0$, plus the Elastic-Net
\citep{2005_JRSS_Zou}   when  $\bL   =  \bI_p$   and  its   extensions
\citep{2010_AOAS_slawski,2011_EJS_Hebiri}    which    correspond    to
different choices of $\bL$.  Some  natural choices for $\bL$ motivated
by applications  in genetics, genomics and  spectroscopy are discussed
in Sections \ref{Sec:simu} and \ref{Sec:applications}.  If $\sigma$ is
unknown,  letting   $\lambda_2=0$  in  \eqref{eq:criteria2_univariate}
leads to  the $\ell_1$-penalized mixture regression  model proposed by
\citet{2010_Test_Stadler},  where  both  $\bbeta$ and  $\sigma^2$  are
inferred.  In this work,  \citeauthor{2010_Test_Stadler} insist on the
importance of penalizing the vector  of coefficients by an amount that
is  inversely proportional  to  $\sigma$.   Penalizing the  regression
coefficients  and the  small  variances  $\sigma^2$ simultaneously  is
indeed highly desirable, which has  some connections with the Bayesian
Lasso of \citet{2008_JASA_Park}.

To sum-up, our approach can be seen as a generalization of all these
methods  to   the  multiple-responses  case,  not   to  mentioned  the
structured regularization brought by the $\ell_2$-norm.

%%% Local Variables:
%%% TeX-master: "JST_AOAS_main.tex"
%%% End:


==> arxiv_version/v1/intro.tex <==
\section{Introduction}

Multivariate regression,  that is,  regression with  multiple response
variables, is increasingly used to model high dimensional problems. By
considering multiple  responses, we wish to  strengthen the estimation
and/or  the  selection  of  the relevant  input  features,  by  taking
advantage  of the  dependency  pattern between  the  outputs. This  is
particularly appealing when the data is scarce, or even in the '$n<p$'
high dimensional setup, in which framework this work enters.  Compared
to  its  univariate counterpart,  the  general  linear model  aims  to
predict several -- say $q$ --  responses from a set of $p$ predictors,
relying on a training data set $\set{(\bx_i,\by_i)}_{i=1,\dots,n}$:
\begin{equation}
  \label{eq:reg_model_row}
  \by_i      =     \bB^T      \bx_i     +      \bvarepsilon_i,     \quad
  \bvarepsilon_i\sim\mathcal{N}(\bzr,\bR), \quad \forall i=1,\dots,n.
\end{equation}
The  $p\times  q$  matrix  of  regression coefficients  $\bB$  and  the
$q\times   q$  covariance   matrix   $\bR$  of   the  Gaussian   noise
$\bvarepsilon_i$ are unknown.
% \old{Note  that we omit  the intercept term    and     center    the    data     for    clarity.}     
Model \eqref{eq:reg_model_row}  has been studied  by \citet{MV_mardia}
in the low dimensional case  where both ordinary and generalized least
squares estimators of $\bB$ coincide and do not depend on $\bR$. These
approaches  boil down  to  perform $q$  independent regressions,  each
column $\bB_j$  describing the weights associating  the $p$ predictors
to the $j$th  response.  In the $n<p$ setup  however, these estimators
are not defined.

The present work proposes  a general multivariate regression framework
suited to  the high dimensional  setup with three purposes  that shall
ease the  learning task: $i)$  We want  to account for  the dependency
structure between the outputs, if it  exists.  That is to say, we want
to integrate the estimation of  $\bR$ in the inference process.  $ii)$
In order to improve interpretability, we  pay a prior attention to the
direct links  between predictors and responses.   Indeed, according to
the Gaussian  graphical models (GGM),  direct effects are  measured by
partial   covariances  between   predictors  and   responses  (denoted
$\bOmega_{\bx\by}$ hereafter), and not  by the regression coefficients
$\bB$.   In   this  regard,   as  few   predictors  are   expected  to
\textit{directly}  influence  each  response,   we  choose  to  induce
sparsity on partial  covariances at once.  $iii)$ We want  to have the
possibility   of  integrating   some  prior   information  about   the
predictors. Indeed, in many applications  such as genomics or spectral
data  analysis,  the  predictors  display  a  structure  (e.g.   their
position along  the genome) and  their influence on the  responses are
likely to display the same structure.

We design  a new estimator  to achieve the three  aforementioned goals
that  we  call  SPRING  (\emph{``Structured  selection  of  Primordial
  Relationships IN  the General  linear model''}).  To  illustrate the
features of  SPRING, we  consider as a  motivating example  the cookie
dough   data from  \cite{data_cookies1}:   in  this   typical  multivariate
regression   problem,  four  continuous   responses  related   to  the
composition of biscuits (percentages of fat, sucrose, flour and water)
may be  linearly explained by predictors  corresponding to reflectance
spectroscopy   measurements.    Parameters   fitted  by   SPRING   are
represented on Figure~\ref{Fig:Cookies1} with, from left to right, the
estimators  of  the  regression  coefficients $\bB$,  of  the  direct
effects $\bOmega_{\bx\by}$ and of the residual covariance $\bR$.
%
\begin{figure*}[tbp!]
  \centering
  \begin{tabular}{@{}c@{}c@{}c@{}c}
    &  $\hat{\bB}$   (indirect  effects)  &  $-\hat{\bOmega}_{\bx\by}$ (direct effects) & $\hat{\bR}$ \\
    \includegraphics[width=.08\textwidth,clip=true,trim=0 -5cm 0 0]{figures/cookies_legend}
    & \includegraphics[width=.3\textwidth]{figures/cookies_beta_spring}
    & \includegraphics[width=.3\textwidth]{figures/cookies_omega_spring}
    & \includegraphics[width=.3\textwidth]{figures/cookies_covariance}\\
    & \multicolumn{2}{c}{wavelength range (nanometer)} & \\
  \end{tabular}
  \caption{Parameters estimated  by SPRING for the  cookies dough data
    (better    seen    in    color).   {Since    $\hat{\bB}$    and
      $\hat{\bOmega}_{\bx\by}$ are  opposite in sign in  our model, we
      represent $-\hat{\bOmega}_{\bx\by}$  to ease the  comparison between
      direct and indirect effects.}}
  \label{Fig:Cookies1}
\end{figure*}
%
The  regression coefficients  show no  sparsity pattern  but  a strong
spatial structure  along the spectrum, characterized  by waves induced
by  a smooth  first order  difference prior.   Concerning  a potential
structure between the outputs, we identify interesting regions where a
strong correlation between  the responses induces correlations between
the regression coefficients.  Consider  for instance positions 1750 to
2000:  the regression  parameters related  to 'dry-flour'  are clearly
anti-correlated  with  those   related  to  'sucrose'.
% \old{,  which  is confirmed  by  the  corresponding  entry  in  $\hat{\bR}$  ($\approx-0.5$)}
Still, we cannot  distinguish {in} $\hat{\bB}$ for a  direct effect of
this  region on  either  the  flour or  sucrose  composition.  Such  a
distinction  is achieved  on  the middle  panel  where direct  effects
$\hat{\bOmega}_{\bx\by}$  selected by SPRING  are plotted:  it defines
sparse predictive regions  specific to each response, where  it is now
obvious  that region 1750  to 2000  is rather  linked to  the sucrose.
This  example   continues  latter,  and  also   illustrates  the  good
predictive performance of SPRING.

The outline of the paper is as follows.  In Section \ref{Sec:model} we
expose  the statistical  model and  the associated  learning strategy:
first,  we  introduce  the   multivariate  regression  model  and  the
parametrization retained.   Second, we propose a  penalized likelihood
criterion   to  regularized   the   model  according   to  the   three
aforementioned  goals.   Then  we develop  an  efficient  optimization
strategy to minimize  this criterion.  A paragraph  also addresses the
model  selection  issue.   Section   \ref{Sec:simu}  is  dedicated  to
illustrative simulation  studies.  In  Section \ref{Sec:applications},
we  develop  further the  cookie  dough  example and  investigate  two
multivariate  problems:  first,   the  relationships  between  genetic
markers and a series of phenotypes of the plant \emph{Brassica napus};
and second, the regulatory motifs  discovery of yeast from time-course
microarray  experiments. In  theses applications,  specific underlying
structuring  priors  arise,  whose  integration within  our  model  is
detailed.

\paragraph*{Links to  related works} Several recent  papers tackle the
multivariate  regression problem  with  penalties-based approaches  by
including  the  dependency pattern  of  the  outputs  in the  learning
process.  When  this pattern  is known \emph{a  priori}, we  enter the
``multitask'' framework  where many authors suggested  variants of the
$\ell_1$-penalty  shaped  accordingly.    A  natural  approach  is  to
encourage a  similar behavior of the regression  parameters across the
outputs -- or  tasks -- using group-norms zeroing a  full row of $\bB$
at    once,    across    the    corresponding    outputs    \citep[see
e.g.][]{2011_SC_Chiquet,2011_AOS_Obozinski}.    Refinements  exist  to
cope  with   complex  dependency  structures,  using   graph  or  tree
structures   \citep{2009_PLOS_kim,2010_ICML_kim},   yet  the   pattern
remains  fixed.   When  it   is  unknown,  the  general  linear  model
\eqref{eq:reg_model_row} is a natural tool to account for dependencies
between        the       responses.         In        this       vein,
\citet{2010_JCGS_rothman,2011_AoAS_yin}   suggest   to  penalize   the
negative  log-likelihood of  \eqref{eq:reg_model_row} by  two $\ell_1$
norms  respectively inducing sparsity  on the  regression coefficients
$\bB$ and  on the  inverse covariance $\bR^{-1}$.   {However their
  criterion is hard to minimize  as it is only bi-convex.  Theoretical
  guarantees are proposed in \citet{,2012_JMA_lee}, accompanied with a
  two-stage  procedure involving a  plug-in estimator of  the inverse
  covariance, which leads to an optimization procedure computationally
  less    demanding.}    In    \citet{2012_JMLR_sohn},    an   elegant
re-parametrization of \eqref{eq:reg_model_row} is depicted, leading to
a formulation  that is jointly convex  and enjoys features  of the GGM
approach.  {\citet{2012_arxiv_yuan}  recently proposed theoretical
  analysis   of   this  model.}    In   this   paper,   we  build   on
\citeauthor{2012_JMLR_sohn}'s   parameterization   yet   we  adopt   a
different  stance regarding  the  regularization, both  on the  output
structure and  on the regression parameters.   SPRING induces sparsity
on  the direct  relationships like  in \citet{2012_JMLR_sohn},  yet no
sparsity  assumption  is  made  for  the  inverse  covariance,  as  we
typically assume a reasonable number of outputs compared to the number
of predictors and sample size.  This leads to a different optimization
strategy,  a   different  estimator  for  the   covariance  $\bR$  and
eventually of  the regression  parameters $\bB$.  On  top of  that, we
include structural  information via an  additional regularization term
using  an application-specific  metric, generalizing  the 'structured'
versions of  the Elastic-net \citep{2010_AOAS_slawski,2011_EJS_Hebiri}
proposed  in  the   univariate-output  case.   Indeed,  an  additional
originality of  our work is  to investigate deeply the  integration of
such structural  information in the various  contexts of spectroscopy,
genomic selection and regulatory  motif discovery, by constructing our
regularization scheme from each application specificity.

%%% Local Variables:
%%% TeX-master: "JST_AOAS_main.tex"
%%% End:


==> arxiv_version/v1/optim.tex <==
\subsection{Optimization}
\label{Sec:optim}

To minimize  the objective, we  rely on a simple  strategy alternating
the  optimization on  $\bOmega_{\by\by}$ and  $\bOmega_{\bx\by}$, that
is,
\begin{subequations}
  \begin{equation}
    \label{eq:optim_cov}
    \hat{\bOmega}_{\by\by}^{(k+1)} = \argmin_{\bOmega_{\by\by}\succ 0}
    J_{\lambda_1\lambda_2}(\hat{\bOmega}_{\bx\by}^{(k)}, \bOmega_{\by\by}),
  \end{equation}
  \begin{equation}
    \label{eq:optim_par}
    \hat{\bOmega}_{\bx\by}^{(k+1)}     =    \argmin_{\bOmega_{\bx\by}}
    J_{\lambda_1\lambda_2}(\bOmega_{\bx\by},\hat{\bOmega}_{\by\by}^{(k+1)}).
  \end{equation}
\end{subequations}

Alternate          strategies         were          adopted         by
\citet{2010_JCGS_rothman,2011_AoAS_yin},   yet  in  these   cases  the
objective   is  only  bi-convex   as  they   rely  on   the  classical
parametrization \eqref{eq:reg_model_row} and  their algorithms are not
meant     to     converge    to     the     global    minimum.      In
\citet{2012_JMLR_sohn,2012_arxiv_yuan},   the  criterion   is  jointly
convex yet the regularization is different from ours and requires more
demanding numerical optimization because  of the regularization of the
concentration  matrix  $\bOmega_{\by\by}$.   Besides,  no  convergence
results are given in these works.

Concerning  our   criterion,  the   alternating  scheme   seems  quite
appropriate:   first,  we   may   apply  the   results  developed   in
\cite{2009_MP_tseng,2001_JOTA_tseng}  on  the   convergence  of  block
coordinate  descent  for  the   minimization  of  nonsmooth  separable
function,   since  \eqref{eq:objective}   is   clearly  separable   in
$(\bOmega_{\bx\by}, \bOmega_{\by\by})$ for  the nonsmooth part induced
by  the  $\ell_1$-norm.  Thus,  under  the  assumption of  Proposition
\ref{prop:existence_uniqueness}, the alternating  scheme is guaranteed
to  convergence  to  the  unique global  minimum.   Second,  efficient
procedures   exist    to   solve    the   two    convex   sub-problems
\eqref{eq:optim_cov} and \eqref{eq:optim_par}, as detailed herein.

On  the   first  hand,  \eqref{eq:optim_par}  can  be   recast  as  an
Elastic-Net problem, which  in turn, can be recast  as a LASSO problem
\citep[see,    e.g.][]{2005_JRSS_Zou,2010_AOAS_slawski}.     This   is
straightforward   thanks  to   Proposition   \ref{prop:vec_obj}:  when
$\hat{\bOmega}_{\by\by}$  is fixed,  solution  to \eqref{eq:optim_par}
can be obtained via
\begin{equation}
  \label{eq:enet_recast}
  \hat{\bomega}     \left(=    \vec(\hat{\bOmega}_{\bx\by})    \right)
  =\argmin_{\bomega\in\Rset^{pq}} \frac{1}{2} \|\mathbf{A}\bomega - \mathbf{b}\|_2^2 + \frac{\lambda_2}{2}
  \bomega^T   \tilde{\bL} 
  \bomega + \lambda_1  \|\bomega\|_1 ,
\end{equation}
where $\bA,\mathbf{b}$ and $\tilde{\bL}$ are defined by
\begin{equation*}
\mathbf{A} =
  \left(\hat{\bOmega}_{\by\by}^{-1/2}   \otimes   \bX/\sqrt{n}  \right),
  \mathbf{b} = - \vec\left(\bY\hat{\bOmega}_{\by\by}^{1/2}\right)/ \sqrt{n}
     \text{ and }
  \tilde{\bL} = \hat{\bOmega}_{\by\by}^{-1} \otimes \bL.
\end{equation*}

On  the second  hand, we  can solve  analytically \eqref{eq:optim_cov}
with  simple matrix algebra,  as stated  in the  following Proposition
whose proof is postponed to Appendix Section \ref{sec:cov_solve}.

\begin{proposition}\label{prop:cov_solve} Let $n\geq q$.  If
  $\hat{\bOmega}_{\bx\by}    =   \bzr$,    $\hat{\bOmega}_{\by\by}   =
  \bS_{\by\by}^{-1}$.  Otherwise,  assume  that  the  following  eigen
  decomposition holds
  \begin{equation*}
    \hat{\bOmega}_{\by\bx} (\lambda_2\bL + \bS_{\bx\bx})
    \hat{\bOmega}_{\bx\by} \bS_{\by\by}  = \bU \diag(\boldsymbol\zeta)
    \bU^{-1}
  \end{equation*}
  and denote by $\boldsymbol\eta=(\eta_1,\dots,\eta_q)$ the respective
  unique positive roots  of $\eta_j^2 - \eta_j -  \zeta_j$.  For a fix
  $\hat{\bOmega}_{\bx\by}$,   solution   $\hat{\bOmega}_{\by\by}$   to
  \eqref{eq:optim_cov} and its inverse writes
  \begin{subequations}
    \begin{equation}
      \label{eq:invcov_solve}
      \hat{\bOmega}_{\by\by} = \bU \diag(\boldsymbol\eta/\boldsymbol\zeta) \bU^{-1}
      \hat{\bOmega}_{\by\bx} (\lambda_2\bL + \bS_{\bx\bx}) \hat{\bOmega}_{\bx\by} (=\hat{\bR}^{-1}),
    \end{equation}
    \begin{equation}
      \label{eq:cov_solve}
      \hat{\bOmega}_{\by\by}^{-1}           =          \bS_{\by\by}\bU
      \diag(\boldsymbol\eta^{-1}) \bU^{-1} (=\hat{\bR}).
    \end{equation}
  \end{subequations}
\end{proposition}

Because  our  procedure  relies  on alternating  optimization,  it  is
difficult to give either a global  rate of convergence or a complexity
bound.   Nevertheless, the  complexity of  each iteration  is easy  to
derive,  since  it  amounts  to  two well  known  problems:  the  main
computational  cost in  \eqref{eq:optim_cov} is  due to  the SVD  of a
$q\times  q$  matrix,   which  costs  $\mathcal{O}(q^3)$.   Concerning
\eqref{eq:optim_par}, it  amounts to the resolution  of an Elastic-Net
problem with $p\times  q$ variables and $n \times q$  samples.  If the
final number of nonzero entries  in $\hat{\bOmega}_{\bx\by}$ is $k$, a
good  implementation  with  Cholesky  update/downdate  is  roughly  in
$\mathcal{O}(n p q^2 k)$  \citep[see, e.g.][]{2012_FOT_bach}. Since we
typically  assumed  that  $n\geq  q$,  the global  cost  of  a  single
iteration of the alternating scheme  is thus $\mathcal{O}(n p q^2 k)$,
and  we theoretically  can  treat  problems with  large  $p$ when  $k$
remains moderate.

Finally, we typically want to  compute a series of solutions along the
regularization  path  of Problem  \eqref{eq:objective},  that is,  for
various  values of  $(\lambda_1,\lambda_2)$.  To  this end,  we simply
choose   a   grid  of   penalties   $\Lambda_1   \times  \Lambda_2   =
\set{\lambda_1^{\text{min}},   \dots,  \lambda_1^{\text{max}}}  \times
\set{\lambda_2^{\text{min}},   \dots,  \lambda_2^{\text{max}}}$.   The
process is  easily distributed on different computer  cores, each core
corresponding to a value picked  in $\Lambda_2$.  Then on each core --
i.e.  for a fix $\lambda_2\in\Lambda_2$  -- we cover all the values of
$\lambda_1\in\Lambda_1$ relying on  the warm start strategy frequently
used  to  go through  the  regularization  path of  $\ell_1$-penalized
problems.    A   prototype  implementation   is   distributed  in   an
\texttt{R}/\texttt{C++}-package  available from  the first  author web
site%\footnote{http://stat.genopole.cnrs.fr/$\sim$jchiquet/spring}
.

% Optimality condition are formulated  thanks to subdifferential calculs
% to handled with the differentiation of the $\ell_1$-norm, so as
%   \begin{equation*}
%   \frac{\partial             J(\bOmega_{\bx\by})}{\partial
%     \bOmega_{\bx\by}}          =          0         \Leftrightarrow
%   \bS_{\bx\by}       +      \hat{\bSigma}_{\bx\bx} \bOmega_{\bx\by}\bR + \lambda_1\bs{\Gamma} =
%   0.
% \end{equation*}
% where $\bs{\Gamma}=(\Gamma_{jk})_{j\in\clM,k\in\clC}$  the $m\times c$
% matrix defined by
% \begin{equation*}
%   \Gamma_{jk} = \begin{cases}
%     \sign\left(\bOmega_{\bx\by}\right)_{jk}       &      \text{      if
%       $\left(\bOmega_{\bx\by}\right)_{jk} \neq 0$}\\
%     \theta: |\theta| < 1 & \text{otherwise}.\\
%   \end{cases}
% \end{equation*}


% with optimality conditions
% \begin{equation}
%   \label{eq:KKT_omega}
%   \left\{\begin{array}{lll}
%       \left( \vec(\bS_{\by\bx}) + (\hat{\bSigma}_{\bx\bx}
%         \otimes\bR)\bomega \right)_i& = -\lambda \
%       \sign(\omega_i) & \text{ if } \omega_i \neq 0\\
%       \left| \left(\vec(\bS_{\by\bx}) + (\hat{\bSigma}_{\bx\bx}
%           \otimes\bR)\bomega\right)_i \right| & \leq \lambda & \text{ if } \omega_i = 0\\
%   \end{array}\right.
% \end{equation}
% The corresponding matrix formulation is
% \begin{equation}
%   \label{eq:KKT_Omega}
%   \left\{\begin{array}{lll}
%       \left(\bS_{\by\bx}   +   \bR
%       \bOmega_{\by\bx}\hat{\bSigma}_{\bx\bx}\right)_{kj} & = -\lambda \
%     \sign(\bOmega_{\by\bx})_{kj}& \text{ if }
%     \left(\bOmega_{\by\bx}\right)_{kj} \neq 0\\
%      \left|  \left(\bS_{\by\bx}  +
%         \bR\bOmega_{\by\bx}\hat{\bSigma}_{\bx\bx} \right)_{kj} \right|
%     & \leq \lambda &
%     \text{ if }
%     \left(\bOmega_{\by\bx}\right)_{kj} = 0.\\
%   \end{array}\right.
% \end{equation}

% \paragraph*{Coordinate   update  for   $\bOmega_{\bx\by}$.}   Consider
% optimizing  against a  single entry  $(\bOmega_{\bx\by})_{jk}$  of the
% matrix.   Cumbersome,  yet straightforward  computation  leads to  the
% following update

% \begin{equation}
%   \label{eq:coordinate_update}
%   (\bOmega_{\bx\by}^\lambda)_{jk}                                           =
%   \frac{\mathrm{Soft}\left(a^{(jk)};\lambda_1\right) }{(\hat{\bSigma}_{\bx\bx})_{jj}
%     \bR_{kk}}, \qquad
%   \mathrm{Soft}(x;\lambda) = x\left(1-\frac{\lambda}{|x|}\right)_+
% \end{equation}
% with
% \begin{equation*}
%   \begin{aligned}
%     a^{(jk)} & = - (\bS_{\bx\by})_{jk} - \sum_{\substack{\ell,m : \\(\ell,m) \neq
%       (j,k)}} (\hat{\bSigma}_{\bx\bx})_{j\ell}
%     (\bOmega_{\bx\by})_{\ell m} \bR_{mk} \\
%     &  = -  (\bS_{\bx\by})_{jk}  - (\hat{\bSigma}_{\bx\bx})_{j\bullet}
%     \bOmega_{\bx\by}  \bR_{\bullet k}  + (\hat{\bSigma}_{\bx\bx})_{jj}
%     (\bOmega_{\bx\by})_{jk} \bR_{k k} .
%   \end{aligned}
% \end{equation*}

%%% Local Variables:
%%% TeX-master: "JST_AOAS_main.tex"
%%% End:


==> arxiv_version/v1/proofs.tex <==
\section{Proofs}

Most of the  proofs rely on basic algebra and  properties of the trace
and  the   $\vec$  operators  \citep[see   e.g.][]{book_harville},  in
particular
\begin{gather*}
  \trace(\bA^T  \bB  \bC  \bD^T)   =  \vec(\bA)^T  (\bD  \otimes  \bB)
  \vec(\bC),\\
  \vec(\bA\bB\bC) = (\bC^T \otimes \bA) \vec(\bB), \\
  (\bA \otimes\bB) (\bC\otimes\bD) = (\bA\bC) \otimes (\bC\bD).
\end{gather*}

\subsection{Derivation of Proposition \ref{prop:vec_obj}}
\label{sec:vec_obj}

Concerning  the two regularization  terms in  \eqref{eq:objective}, we
have $\|\bOmega_{\bx\by}\|_1 =  \|\bomega\|_1$ since the $\ell_1$-norm
applies element-wise here and
\begin{equation*}
  \trace(\bOmega_{\by\bx} \bL \bOmega_{\bx\by}\bOmega_{\by\by}^{-1}) =
  \bomega^T (\bOmega_{\by\by}^{-1} \otimes \bL) \bomega.
\end{equation*}

As  for the log-likelihood  \eqref{eq:log_lik}, we  work on  the trace
term:
\begin{multline*}
  \trace\left(  \left(\bY +  \bX \bOmega_{\bx\by}\bOmega_{\by\by}^{-1}
    \right)^\intercal \left(\bY          +          \bX
      \bOmega_{\bx\by}\bOmega_{\by\by}^{-1}
    \right)\bOmega_{\by\by}\right) \\ 
  \begin{aligned}
    &         =          &         \vec\left(\bY         +         \bX
      \bOmega_{\bx\by}\bOmega_{\by\by}^{-1}\right)^T
    \left(\bOmega_{\by\by}\otimes\bI_n\right) \vec\left(\bY + \bX
      \bOmega_{\bx\by}\bOmega_{\by\by}^{-1}\right) \\
    &   =   &   \left\|\left(\bOmega_{\by\by}\otimes\bI_n\right)^{1/2}
      \left(  \vec(\bY)   +  \left(\bOmega_{\by\by}^{-1}  \otimes  \bX
        \right)
        \vec(\bOmega_{\bx\by}) \right)\right\|_2^2    \\
      &     =    &    \left\|     \vec(\bY\bOmega_{\by\by}^{1/2})    +
        \left(\bOmega_{\by\by}^{-1/2}\otimes   \bX   \right)   \bomega
      \right\|_2^2.
  \end{aligned}
\end{multline*}
The rest of the proof is straightforward.

\subsection{Derivation of Proposition \ref{prop:cov_solve}}
\label{sec:cov_solve}

By   differentiation  of   the  objective   \eqref{eq:objective}  over
$\bOmega_{\by\by}^{-1}$ we obtain the quadratic form
\begin{equation*}
  \bOmega_{\by\by}       \bS_{\by\by}      \bOmega_{\by\by}      -
  \bOmega_{\by\by}                                                =
  \bOmega_{\by\bx}(\lambda_2 \bL + \bS_{\bx\bx})\bOmega_{\bx\by}.
\end{equation*}
After  right  multiplying both  sides  by  $\bS_{\by\by}$, it  becomes
obvious       that      $\bOmega_{\by\by}       \bS_{\by\by}$      and
$\bOmega_{\by\bx}(\lambda_2                    \bL                   +
\bS_{\bx\bx})\bOmega_{\bx\by}\bS_{\by\by}$ commute  and thus share the
same  eigenvectors  $\bU$.    Besides,  it  induces  the  relationship
$\eta_j^2  -\eta_j  = \zeta_j$  between  their respective  eigenvalues
$\eta_j$ and $\zeta_j$,  and we are looking for  the positive solution
of  $\eta_j$.   To  do  so,  first  remark that  we  may  assume  that
$\bOmega_{\by\bx} (\lambda_2 \bL + \bS_{\bx\bx}) \bOmega_{\bx\by}$ and
$\bS_{\by\by}$  are  positive  definite, when  $\bOmega_{\bx\by}  \neq
\bzr$  and $n\geq q$;  and second,  recall that  the eigenvalues  of a
matrix  being  the  product  of  two positive  definite  matrices  are
positive. Hence, $\zeta_j>0$ % (note that this does not imply the symmetry
% of             $\bOmega_{\by\bx}(\lambda_2            \bL            +
% \bS_{\bx\bx})\bOmega_{\bx\by}\bS_{\by\by}$,   though)
and the positive solution of $\eta_j$ is $\eta_j = (1 +
\sqrt{1+4\zeta_j})/2$. We obtain thus
\begin{equation}
  \label{eq:cov_prf}
  \hat{\bOmega}_{\by\by} = \bU \diag(\boldsymbol\eta) \bU^{-1} \bS_{\by\by}^{-1}.
\end{equation}
Direct      inversion     leads      to  \eqref{eq:cov_solve}.     To    get    an   expression    for
$\hat{\bOmega}_{\by\by}$  which  does  not require  additional  matrix
inversion, just remark that
\begin{equation*}
  \bS_{\by\by}^{-1}                                                =
  \left(\bOmega_{\by\bx}\hat{\bSigma}_{\bx\bx}^{\lambda_2}\bOmega_{\bx\by}\bS_{\by\by}\right)^{-1}
  \bOmega_{\by\bx}\hat{\bSigma}_{\bx\bx}^{\lambda_2}\bOmega_{\bx\by}
   = \bU \diag(\boldsymbol\zeta^{-1})\bU^{-1}\bOmega_{\by\bx}\hat{\bSigma}_{\bx\bx}^{\lambda_2}\bOmega_{\bx\by}
\end{equation*}
which,     combined      with     \eqref{eq:cov_prf},     leads     to
\eqref{eq:invcov_solve}.

\subsection{Derivation of Proposition \ref{prop:df_spring}}
\label{sec:df_spring}

To  apply the  results developed  in  \citet{2012_EJS_Tibshirani} that
rely  on  the   well-known  Stein's  Lemma  \citep{1981_AS_Stein},  we
basically need to recast our problem as a classical LASSO applied on a
Gaussian linear regression  model so as the response  vector follows a
normal distribution of  the form $\mathcal{N}(\bmu,\sigma \bI)$.  This
is straightforward by means  of Proposition \ref{prop:vec_obj}: in the
same way as  we derive expression \eqref{eq:enet_recast}, we  can go a
little farther and reach the following LASSO formulation
\begin{equation}
  \label{eq:lasso_recast}
  \argmin_{\bomega\in\Rset^{pq}} \frac{1}{2} \left\|
    \begin{pmatrix}
      \mathbf{A} \\ \sqrt{\lambda_2} \tilde{\bL}^{1/2}
    \end{pmatrix} \bomega - 
    \begin{pmatrix}
      \mathbf{b} \\ \bzr
    \end{pmatrix} \right\|_2^2  + \lambda_1  \|\bomega\|_1,
\end{equation}
with $\bA,\bb$ and $\tilde{\bL}$ defined as in \eqref{eq:enet_recast}.
From model \eqref{eq:cond_model_mat}, it  is not difficult to see that
$\mathbf{b}$ corresponds to an uncorrelated vector form of $\bY$ so as
\begin{equation*}
  \begin{pmatrix}
    \mathbf{b} \\ \bzr
  \end{pmatrix} = 
  \begin{pmatrix}
    -\vec(\bY \bOmega_{\by\by}^{1/2}) \\ \bzr
  \end{pmatrix} \sim \mathcal{N}(\bmu, \bI_{nq}).
\end{equation*}
The  explicit form  of  $\bmu$ has  no  interest here.   The point  is
essentially to  underline that the response vector  is uncorrelated in
\eqref{eq:lasso_recast},  which  allows  us  to  apply  Theorem  2  of
\citeauthor{2012_EJS_Tibshirani} and results  therein, notably for the
Elastic-Net: by these  means, an unbiased estimator of  the degrees of
freedom in \eqref{eq:lasso_recast} can be written as a function of the
active set $\mathcal{A}$ in $\hat{\bomega}^{\lambda_1,\lambda_2}$:
\begin{equation*}
  \hat{\mathrm{df}}_{\lambda_1,\lambda_2} = \trace\left( 
    \mathbf{A}_{\mathcal{A}} \left( (\bA^T\bA + \lambda_2 \tilde{\bL}\ )_{\mathcal{A}\mathcal{A}}\right)^{-1}
    \mathbf{A}_{\mathcal{A}}^T
  \right).
\end{equation*}
Routine    simplifications     lead    to    the     desired    result
\eqref{eq:df_spring}.



% \subsection{Derivation of Proposition \ref{prop:enet_recast}}
% \label{sec:enet_recast}


% %\begin{proof}
%   Minimizing  \eqref{eq:optim_pb} over $\bOmega_{\bx\by}$  only boils
%   down to the minimization of 
%   \begin{equation*}
%     \trace(\bS_{\bx\by}\bOmega_{\by\bx}) + \frac{1}{2}\trace\left(\bOmega_{\by\bx}
%       \hat{\bSigma}_{\bx\bx}^{\lambda_2}\bOmega_{\bx\by} \bOmega_{\by\by}^{-1} \right) + \lambda \|\bOmega_{\bx\by}\|_1.
%   \end{equation*}
%   Looking towards a familiar vector formulation, we introduce $\bomega
%   = \vec(\bOmega_{\by\bx})  = ((\bOmega_{\bx\by})_{1\bullet}^T, \dots,
%   (\bOmega_{\bx\by})_{q\bullet}^T)$  ,  the   $q\times  p$  vector  of
%   parameters, stacking the coefficients  related to the successive $p$
%   predictors across the $q$  outputs. By means of classical properties
%   of the trace and $\vec$ operators, we first notice that
%   \begin{equation*}
%     \trace(\bS_{\bx\by}\bOmega_{\by\bx})                             =
%     \vec(\bOmega_{\by\bx})^T\vec(\bS_{\by\bx}),
%   \end{equation*}
%   and second,
%   \begin{multline*}
%     \trace\left(\bOmega_{\by\bx}
%       \hat{\bSigma}_{\bx\bx}^{\lambda_2}\bOmega_{\bx\by}
%       \bOmega_{\by\by}^{-1}  \right)  = \trace\left(  \bOmega_{\bx\by}
%       \bOmega_{\by\by}^{-1}                            \bOmega_{\by\bx}
%       \hat{\bSigma}_{\bx\bx}^{\lambda_2}\right)          \\          =
%     \vec(\bOmega_{\bx\by}^T)^T          \vec\left(\bOmega_{\by\by}^{-1}
%       \bOmega_{\by\bx} \hat{\bSigma}_{\bx\bx}^{\lambda_2}\right) \\ =
%     \vec(\bOmega_{\by\bx})^T   \left(\hat{\bSigma}_{\bx\bx}^{\lambda_2}
%       \otimes \bOmega_{\by\by}^{-1} \right) \vec(\bOmega_{\by\bx}).
%   \end{multline*}
%   The above minimization problem is thus equivalent to
%   \begin{equation*}
%     \min_{\bomega\in\Rset^{pq}}   \left\{  \frac{1}{2}   \bomega^T  (\hat{\bSigma}_{\bx\bx}^{\lambda_2}
%       \otimes\bOmega_{\by\by}^{-1}) \bomega + \bomega^T \vec(\bS_{\by\bx}) + \lambda
%       \|\bomega\|_1\right\},
%   \end{equation*}
%   providing  that   $\bomega=\vec(\bOmega_{\by\bx})$.   This  $\ell_1$
%   penalized problem can be recast as a structured Elastic-Net problem:
%   by     direct    identification     with    terms     expanded    in
%   \eqref{eq:enet_recast} from  $\|\bA \bomega -  \mathbf{b}\|_2^2$, we
%   just have to solve in $(\bA, \mathbf{b})$
%   \begin{equation*}
%     \left\{\begin{array}{lcr}
%         \bA^T\bA    & = &    \hat{\bSigma}_{\bx\bx}^{\lambda_2}
%         \otimes\bOmega_{\by\by}^{-1}, \\[.5ex]
%         \mathbf{b}^T \bA & = & \vec(\bS_{\by\bx}),
%       \end{array}\right.
%   \end{equation*}
%   which is straightforward.
  
\subsection{Derivation of Proposition \ref{prop:computeDkl}}
\label{sec:computeDkl}

Both results are established by recurrence, the first on
 indices $k$, the second on indices $\ell$. Consider
 \eqref{eq:reck_D} and indices $k$ for instance: this holds true for
 $k=1$ by straightforward matrix calculus. Now, assume that
 $\bD^{k,\ell}$ is known, and you are looking for $\bD^{k+1,\ell}$ by
 increasing the alphabet $\clM_k$ with one letter, so as
 lexicographical order still holds true: this can be done by adding
 successively each letter from $\clM_1=\set{A,C,G,T}$ to the left of
 each word of $\clM_k$ (first $A$ to every work in $\clM_k$, then $C$
 and so on). There are now only two possibilities, which corresponds
 to each term in the right-hand side of \eqref{eq:reck_D}:

 Consider the first term on the one hand: non null elements in
 $\bD^{k,\ell}$ represent the set of motifs with size $k$ being at
 distance $\ell$ to each other. If adding a letter to such motifs, we
 can split the obtained words in four groups, according to the
 currently added letter ($A,C,G$ or $T$). Then, within each of these
 groups (e.g. the group with words starting by $A$), all the words
 shared the very same first letter and thus stay at a distance $\ell$
 from each other: this is just meant by the Kronecker multiplication
 by $\bD^{1,0}$, which builds four blocks corresponding to the four
 aforementioned groups.

 On the other hand, consider the second term: if motifs with size $k$
 are at distance $\ell-1$ from each other, what represents
 $\bD^{k,\ell-1}$, then we can add any kind of letter and stay at a
 distance $\ell$ for motifs with size $k+1$, what is meant by the
 Kronecker product with $\bD^{1,1}$.

  

  
  
  % Thanks  to  the  Cholesky factorization  introduced  in  Proposition
  % \ref{prop:enet_recast}, we have
  % \begin{multline*}
  %   \hat{\bSigma}_{\bx\bx}^{\lambda_2}  \otimes\bOmega_{\by\by}^{-1} =
  %   \left(\frac{1}{n}  \bX^T \bX  +  \lambda_2 \bL\right)  \otimes
  %   \bC^T\bC \\ =
  %   \begin{bmatrix}
  %     \begin{pmatrix}
  %       \bX /\sqrt{n} \\
  %       \sqrt{\lambda_2} \bD
  %     \end{pmatrix}
  %     \otimes \bC
  %   \end{bmatrix}^T
  %   \begin{bmatrix}
  %     \begin{pmatrix}
  %       \bX /\sqrt{n} \\
  %       \sqrt{\lambda_2} \bD
  %     \end{pmatrix}
  %     \otimes \bC
  %   \end{bmatrix},
  %   \end{multline*}
  % from which  we get $\bA$.  The vector $\mathbf{b}$ follows  with the
  % same kind of algebra.
%\end{proof}


% \subsection{Derivation of Proposition \ref{prop:prop_loglik_reg}}
% \label{sec:prop_loglik_reg}

% Considering    model   \eqref{eq:reg_model_row},    then    for   each
% $i=1,\dots,n$,                         we                         have
% $\tilde{\by}_i\sim\mathcal{N}(\bB^\intercal\tilde{\bx}_i,\bR),$ and by
% successively  using $|\bA  \otimes  \bB| =  |\bA|^{\mathrm{rank}(\bB)}
% |\bB|^{\mathrm{rank}(\bA)}$, $\trace(\bA^\intercal\bB\bC\bD^\intercal)
% =       \vec(\bA)^\intercal       (\bD\otimes\bB)\vec(\bC)$,       and
% $(\bA\otimes\bB)^{-1}=(\bA^{-1}\otimes\bB^{-1})$, we get
% \begin{multline*}
%   \log    L_{\bX,\bY}   \varpropto    -\log|\bR_q\otimes   \bLambda_n|
%   -\frac{1}{2} \vec(\bY-\bX\bB)^\intercal
%   (\bR_q\otimes\bLambda_n)^{-1}\vec(\bY-\bX\bB)\\
%   =                  -n\log|\bR_q|-q\log|                  \bLambda_n|
%   -\frac{1}{2}\trace\left((\bY-\bX\bB)^\intercal\bLambda_n^{-1}
%     (\bY-\bX\bB-\bU)\bR_q^{-1} \right).
% \end{multline*}

% The result follows since $\trace(\bA^\intercal\bA) = \|\bA\|_F^2$.

% \subsection{Derivation of Proposition 1}
% \label{sec:prop_intercept}
% First, we need  a convenient row wise rescaling of  the data $\bY$ and
% $\bX$,  as   in  generalized  least-square.   This  can  be   done  by
% left-multiplying    \eqref{eq:reg_model_vec}   by    $(\bI_q   \otimes
% \bLambda_n^{-\frac{1}{2}})$,  and by  the property  $\vec(\bA\bB\bC) =
% (\bC^\intercal \otimes \bA) \vec(\bB)$ of the $\vec$ operator, we have
% \begin{equation}
%   \label{eq:proof_intercept_1}
%   \vec(\bLambda_n^{-\frac{1}{2}}\bY)                                =
%   \vec(\bLambda_n^{-\frac{1}{2}}\bX\bB)                             +
%   \vec(\bLambda_n^{-\frac{1}{2}}\bU)     +    \var((\bI_q    \otimes
%   \bLambda_n^{-\frac{1}{2}})\vec(\bepsilon)),
% \end{equation}
% where the variance of the residuals is given by\footnote{Recall that
%   $(\bA  \otimes   \bB)  (\bC   \otimes  \bD)  =   (\bA\bC)  \otimes
%   (\bB\bD)$.}
% \begin{equation*}
%   \var((\bI_q  \otimes  \bLambda_n^{-\frac{1}{2}})\vec(\bepsilon)) =
%   (\bI_q    \otimes   \bLambda_n^{-\frac{1}{2}})    (\bR_q   \otimes
%   \bLambda_n) (\bI_q  \otimes \bLambda_n^{-\frac{1}{2}})^\intercal =
%   \bR_q \otimes \bI_n.
% \end{equation*}

% Hence,   we   can   treat   each   conditions   separately   as   in
% \eqref{eq:reg_model_row}.  Consider for  instance condition $c$: the
% residuals  sum of squares  in \eqref{eq:proof_intercept_1}  for this
% condition writes
% \begin{equation*}
%   \left\| \bLambda_n^{-1/2} \left(\by_{(c)}- \mu_c \I_n - \bX \bb_{(c)}\right)\right\|_2^2,
% \end{equation*}
% Then, differentiating over $\mu_c$, we get that
% \begin{equation*}
%   \hat{\mu}_c                 =                \frac{\I_n^\intercal
%     \bLambda_n^{-1}}{\I_n^\intercal             \bLambda_n^{-1}\I_n}
%   \left(\by_{(c)} - \bX \bb_{(c)}\right).
% \end{equation*}
% Write this  formulation for  each condition in  $\clC$, and  we meet
% back \eqref{eq:intercept}.

% \subsection{Derivation of Proposition 3}
% \label{sec:prop_loglik_cggm}

% Considering  model \eqref{eq:reg_model_vec}  with  no intercept,  then
% $\vec(\bY)\sim\mathcal{N}(\vec(\bX\bB),\bR_q\otimes\bLambda_n)$,    and
% by successively using  $|\bA \otimes \bB| = |\bA|^{\mathrm{rank}(\bB)}
% |\bB|^{\mathrm{rank}(\bA)}$, $\trace(\bA^\intercal\bB\bC\bD^\intercal)
% =       \vec(\bA)^\intercal       (\bD\otimes\bB)\vec(\bC)$,       and
% $(\bA\otimes\bB)^{-1}=(\bA^{-1}\otimes\bB^{-1})$, we get
% \begin{multline*}
%   \log   L    (\bB,\bLambda_n,\bR_q)   \varpropto   -\log|\bR_q\otimes
%   \bLambda_n| -\frac{1}{2} \vec(\bY-\bX\bB)^\intercal
%   (\bR_q\otimes\bLambda_n)^{-1}\vec(\bY-\bX\bB)\\
%   =                  -n\log|\bR_q|-q\log|                  \bLambda_n|
%   -\frac{1}{2}\trace\left((\bY-\bX\bB)^\intercal\bLambda_n^{-1}
%     (\bY-\bX\bB)\bR_q^{-1} \right).
% \end{multline*}
% and the result follows since $\trace(\bA^\intercal\bA) = \|\bA\|_F^2$.

%%% Local Variables:
%%% TeX-master: "JST_AOAS_main.tex"
%%% End:


==> arxiv_version/v1/selection.tex <==
\subsection{Model selection and parameter tuning}
\label{Sec:selection}

Model selection amounts here to choosing a couple of tuning parameters
$(\lambda_1,\lambda_2)$ among the grid $\Lambda_1 \times
\Lambda_2% = \set{\lambda_1^{\text{min}}, \dots,
  % \lambda_1^{\text{max}}}  \times  \set{\lambda_2^{\text{min}}, \dots,
  % \lambda_2^{\text{max}}}
$, where  $\lambda_1$ tunes the  sparsity while $\lambda_2$  tunes the
amount  of structural regularization.   We aim  either at  picking the
model with  minimum prediction error, or  the one closest  to the true
model   assuming  Equation~\eqref{eq:cond_model}  holds.    These  two
perspectives  generally do  not lead  to the  same model  choice: when
looking  for  the  model  minimizing the  prediction  error,  $K$-fold
cross-validation   is  the  recommended   option  \citep{Hesterberg08}
despite  its   additional  computational  cost.    Letting  $\kappa  :
\set{1,\dots,n}\to\set{1,\dots,K}$ the  function indexing the  fold to
which observation $i$ is allocated, the CV-choice is
\begin{equation*}
  \label{eq:cv_pred}
  (\lambda_1^\text{cv},\lambda_2^\text{cv})                                    =
  \argmin_{(\lambda_1,\lambda_2) \in \Lambda_1\times\Lambda_2}
  \frac{1}{n} \sum_{i=1}^n 
  \left\| \bx_{i}^T \hat{\bB}_{-\kappa(i)}^{\lambda_1,\lambda_2}- \by_{i} \right\|_2^2,
\end{equation*}
where   $\hat{\bB}_{-\kappa(i)}^{\lambda_1,\lambda_2}$  minimizes  the
objective  \eqref{eq:objective},   once  data  $\kappa(i)$   has  been
removed. In  place of  the prediction error,  other quantities  can be
cross-validated  in  our  context,  e.g. the  negative  log-likelihood
\eqref{eq:log_lik}. In  the remainder of  the paper, we  only consider
cross-validating the prediction error, though.

As  an alternative  to cross-validation,  analytic criteria  provide a
fast way to  perform model selection and are  sometimes more suited to
the  selection of  the  true underlying  model.   Although relying  on
asymptotic derivations,  they often offer  good practical performances
when the  sample size  $n$ is  not too small  compared to  the problem
dimension.   For  penalized  methods,   a  general  form  for  various
information criteria is expressed as  a function of the likelihood $L$
(defined  by \eqref{eq:log_lik}  here)  and the  effective degrees  of
freedom:
\begin{equation}
  \label{eq:pen_crit}
  (\lambda_1^\text{pen},\lambda_2^\text{pen}) = \argmin_{(\lambda_1,\lambda_2)\in\Lambda_1\times\Lambda_2}
  - 2\log L(\hat{\bOmega}^{\lambda_1,\lambda_2}_{\bx\by},
  \hat{\bOmega}^{\lambda_1,\lambda_2}_{\by\by})   +   \mathrm{pen}
  \cdot \mathrm{df}_{\lambda_1, \lambda_2}.
\end{equation}
Setting $\text{pen}=2$  or $\log(n)$ respectively lead to  AIC or BIC.
For the practical evaluation of \eqref{eq:pen_crit}, we must give some
sense      to      the      effective     degrees      of      freedom
$\text{df}_{\lambda_1,\lambda_2}$  of a  SPRING fit.   We use  the now
classical definition  of \citet{2004_JASA_Efron} and rely  on the work
of  \citet{2012_EJS_Tibshirani} to  derive the  following Proposition,
whose proof is postponed to Appendix Section \ref{sec:df_spring}.

\begin{proposition}\label{prop:df_spring}  An  unbiased  estimator  of
  $\text{df}_{\lambda_1,\lambda_2}$ for a SPRING fit is 
  \begin{equation}
    \label{eq:df_spring}
    \hat{\mathrm{df}}_{\lambda_1,  \lambda_2} = \mathrm{card}(\mathcal{A})
    - \lambda_2          \mathrm{tr}\left(         (\hat{\bR}\otimes
      \bL )_{\mathcal{A}\mathcal{A}} \left((\hat{\bR}\otimes (\bS_{\bx\bx} +
      \lambda_2\bL))_{\mathcal{A}\mathcal{A}}\right)^{-1}\right),
  \end{equation}
  where               $\mathcal{A}              =              \set{j:
    \vec\left(\hat{\bOmega}_{\bx\by}^{\lambda_1,\lambda_2}\right) \neq
    0}$     is      the     set     of      nonzero     entries     in
  $\hat{\bOmega}_{\bx\by}^{\lambda_1,\lambda_2}$.
\end{proposition}

Note  that  we  can  compute  expression  \eqref{eq:df_spring}  at  no
additional  cost,  relying on  computations  already  made during  the
optimization process.

%%% Local Variables:
%%% TeX-master: "JST_AOAS_main.tex"
%%% End:


==> arxiv_version/v1/simu_studies.tex <==
\subsection{Influence of covariance between outcomes}  

The  first  simulation  study  aims  to illustrate  the  advantage  of
splitting $\bB$  into $-\bOmega_{\bx\by}\bR$ over  working directly on
$\bB$.  We  set $p=40$ predictors, $q=5$ outcomes  and randomly select
$25$ non  null entries in $\set{-1,1}$ to  fill $\bOmega_{\bx\by}$. We
do not put any structure along the predictors as this study intends to
measure the gain of using the cGGM approach.  The covariance follows a
Toeplitz  scheme \footnote{We set  $\bR$ a  correlation matrix  not to
  excessively penalize the LASSO or the group-LASSO, that use the same
  tuning parameter $\lambda_1$ across  the outcomes (and thus the same
  variance  estimator).}    so  as  $\bR_{ij}   =  \tau^{|i-j|}$,  for
$i,j=1,\dots,q$.    We  consider  three   scenarios  tuned   by  $\tau
\in\set{.1,.5,.9}$ corresponding to  an increasing correlation between
the  outcomes that  eventually  makes the  cGGM  more relevant.   This
settings    have   been    used   to    generate   panel    $(a)$   of
Figure~\ref{fig:model_insight}.  For   each  covariance  scenario,  we
generate a  training set  with size  $n=50$ and a  test set  with size
$n=1000$.   We assess  the performance  of SPRING  by  comparison with
three baselines:  $i)$ the LASSO, $ii)$  the $\ell_1/\ell_2$ multitask
group-LASSO and $iii)$ SPRING  with known covariance matrix $\bR$.  As
it corresponds to the best fit  that we can meet with our proposal, we
call this variant the ``oracle'' mode of SPRING.  The final estimators
are obtained  by 5-fold cross-validation on the  training set.  Figure
\ref{fig:cov_mse}  gives   the  boxplots   of  PE  obtained   for  100
replicates.  As expected, the  advantage of taking the covariance into
account  becomes more  an more  important to  maintain a  low  PE when
$\tau$ increases.   When correlation is  low, the LASSO  dominates the
group-LASSO;  this is  the other  way  round in  the high  correlation
setup, where  the latter takes  full advantage of its  grouping effect
along the  outcomes. Still, our proposal  remains significantly better
as  soon as  $ \tau$  is  substantial enough.  We also  note that  our
iterative algorithm does a good  job since SPRING remains close to its
oracle variant.
\begin{figure}[htbp!]
  \centering
  \includegraphics[trim=0 0 0 15pt,clip=true,width=.65\columnwidth]{figures/cov_simu_err}
  \caption{Illustration  of  the  influence  of  correlations  between
    outcomes.  Scenarios $\set{\text{low},\text{med},\text{high}}$ map
    to  $\tau\in\set{.1,.5,.9}$   in  the  Toeplitz-shaped  covariance
    matrix $\bR$.}
    \label{fig:cov_mse}
    \vspace{-.5cm}
\end{figure}

\subsection{Structure   integration   and   robustness}   The   second
simulation study is  designed to measure the impact  of introducing an
informative prior along the predictors via $\bL$. To remove any effect
induced by the covariance between  the outputs, we fix $q=1$.  In this
case      the     criterion      writes     as      in     Expressions
\eqref{eq:criteria_univariate}   and  \eqref{eq:criteria2_univariate}:
$\bR$  boils down  to a  scalar $\sigma^2$  and $\bB,\bOmega_{\bx\by}$
turn to two  $p$-size vectors sharing the same  sparsity pattern so as
$\bbeta = -\bomega  \sigma^2$.  In this situation, SPRING  is close to
\citeauthor{2010_AOAS_slawski}'s  structured Elastic-Net,  except that
we  hope for a  better estimation  of the  coefficients thanks  to the
estimation of $\sigma$.  For comparison, we thus draw inspiration from
the simulation  settings originally used to  illustrate the structured
Elastic-Net: we set $\bomega  = (\omega_j)_{j=1}^p, $ with $p=100$, so
as we observe a sparse vector  with two smooth bumps, one positive and
the other one negative:
\begin{equation*}
  \omega_j =
  \begin{cases}
    -( (30-j)^2 -100)/200 & j=21,\dots 39,\\
    \ \ \ ( (70-j)^2 -100)/200 & j=61,\dots 80,\\
    0 & \text{otherwise}.
  \end{cases}
\end{equation*}
A natural choice for $\bL$ is  to rely on the first forward difference
operator  as in the  fused-Lasso \citep{2005_JRSSB_tibshirani},  or it
smooth counterpart \citep{2011_EJS_Hebiri}.  We thus set %\footnote{This
  % is      also     the      default     choice      recommended     by
  % \citeauthor{2010_AOAS_slawski}.}
$\bL = \bD^T\bD$ with
\begin{equation}
  \label{eq:first_order_diff}
  \bD_{ij} = \begin{cases}
    1 & \text{if } i = j,\\
    -1 & \text{if } j = i+1 \\
    0 & \text{otherwise}\\
  \end{cases},
  \quad \begin{array}{c}
    i=1,\dots,p-1, \\
    j=1,\dots,p.    
  \end{array}
\end{equation}
Hence, $\bL$ is  the combinatorial Laplacian of a  chain graph between
the successive predictors.  
\begin{figure}[htpb!]
  \centering
  \includegraphics[trim=0 0 0 15pt,clip=true,width=.65\columnwidth]{figures/struct_simu}
  \caption{Illustrating gain  brought by structure  information toward
    predictive performance}
  \label{fig:struct_illustration}
\end{figure}
Figure~\ref{fig:struct_illustration} shows the typical gain brought by
prior structure knowledge.  We generate $120$ samples for the learning
with $\sigma^2=5$ and  represent 100 averaged PE curves  as a function
of  $\lambda_1$ for the  LASSO and  for two  versions of  SPRING, with
($\lambda_2 =  .01$) and without ($\lambda_2 =  0$) informative prior.
Incorporating a  relevant structural  information leads to  a dramatic
improvement.  As  expected, univariate  SPRING with no  prior performs
like the LASSO, in the sense that they share the same minimal PE.

Now, the question is:  what if we introduce a wrong  prior, that is, a
matrix $\bL$  completely disconnected from  the true structure  of the
coefficients?  To  answer this question,  we use the same  settings as
above and  randomly swap the  entries in $\bomega$, using  exactly the
same $\bx_i$  to generate the  $\by_i$\footnote{We also used  the same
  seed and CV-folds for both  scenarios.}.  We then apply SPRING using
respectively  a non  informative prior  equal to  the identity  matrix
(thus mimicking the Elastic-Net) and  a 'wrong' prior $\bL$ whose rows
and columns remain unswapped.  We  also try the LASSO, the Elastic-Net
and the  structured Elastic-Net.   All methods  are tuned  with 5-fold
cross-validation  on  the  learning  set.   Table~\ref{tab:struct_res}
presents the results averaged over 100  runs both in term of PE (using
a size-1000 test set) and MSE.
\begin{table}[htbp!]
  \centering
  \begin{small}
    \begin{tabular}{lrrr}
    \hline
    \textit{\textsf{Method}} & \textit{\textsf{Scenario}} & \textit{\textsf{MSE}} & \textit{\textsf{PE}} \\
    \hline
    LASSO
    & -- & .336 (.096) & 58.6 (10.2) \\
%    & swapped & .336 (.096) & 58.6 (10.2) \\
    \cline{1-4}
%     E-Net
%     & unswapped& .340 (.095) & 59 (10.3) \\
%     ($\bL=\bI$)
%     & swapped & .340 (.095) & 59 (10.3) \\
    E-Net    ($\bL=\bI$)
    & -- & .340 (.095) & 59 (10.3) \\
    \cline{1-4}
%     SPRING
%     & unswapped& .358 (.094) & 60.7 (10) \\
%     ($\bL=\bI$)
%     & swapped & .358 (.094) & 60.7 (10) \\
    SPRING    ($\bL=\bI$)
    & -- & .358 (.094) & 60.7 (10) \\
    \cline{1-4}
    S. E-net
    & unswapped & .163 (.036) & 41.3 ( 4.08) \\
    ($\bL=\bD^T \bD$)
    & swapped & .352 (.107) & 60.3 (11.42) \\
    \cline{1-4}
    SPRING
    & unswapped & .062 (.022) & 31.4 ( 2.99) \\
    ($\bL=\bD^T \bD$)
    & swapped & .378 (.123) & 62.9 (13.15) \\
    \hline
  \end{tabular}
  \end{small}
  \caption{Structure integration: performance and robustness. Swapped and unswapped results are the same for LASSO, Elastic-Net and SPRING for $\bL = \bI$.}
  \label{tab:struct_res}
\end{table}

As  expected,  the  methods  that  do  not  integrate  any  structural
information  (LASSO, Elastic-Net  and SPRING  with $\bL=\bI$)  are not
affected by the permutation, {and we avoid these redundancies in Table
  \ref{tab:struct_res} to  save space}.   Overall, they  share similar
performance both in  term of PE and MSE.  When  the prior structure is
relevant, SPRING, and  to a lesser extent  the structured Elastic-Net,
clearly  outperform  the  other competitors.   Surprisingly,  this  is
particularly  true in  term of  MSE, where  SPRING also  dominates the
structured Elastic-Net  that disposes  of the same  information.  This
means that the estimation of the variance also helped in the inference
process.  Finally, these results essentially support the robustness of
the structured methods  which are not much altered when  using a wrong
prior
specification.

%%% Local Variables:
%%% TeX-master: "JST_AOAS_main.tex"
%%% End:


==> arxiv_version/v1/stat_model.tex <==
\subsection{Convex parametrization of multivariate regression}
\label{Sec:stat_model}

The statistical  framework arises from a  different parametrization of
\eqref{eq:reg_model_row}  which  fills  the gap  between  multivariate
regression  and  GGM.   Such  a  connection was  first  underlined  in
\citet{2012_JMLR_sohn},     generalizing    the    link     made    by
\citet{2009_JRSSB_witten} in the single  output case between the LASSO
and  inverse covariance  estimation. This  amounts to  investigate the
joint  probability distribution  of $(\bx_i,  \by_i)$ in  the Gaussian
case, with the  following block-wise decomposition % \footnote{note that
  % $\bSigma_{\by\bx}=\bSigma_{\bx\by}^T$                             and
  % $\bOmega_{\by\bx}=\bOmega_{\bx\by}^T$ by symmetry}
of the covariance
matrix $\bSigma$ and its inverse $\bOmega=\bSigma^{-1}$:
  \begin{equation}
    \label{eq:joint_model}
    \bSigma = \begin{pmatrix}
      \bSigma_{\bx\bx} & \bSigma_{\bx\by} \\
      \bSigma_{\by\bx} & \bSigma_{\by\by} \\
   \end{pmatrix},\quad
   \bOmega = \begin{pmatrix}
     \bOmega_{\bx\bx} & \bOmega_{\bx\by} \\
     \bOmega_{\by\bx} & \bOmega_{\by\by} \\
   \end{pmatrix}.
 \end{equation}
 Back  to   the  distribution  of  $\by_i$   conditional  on  $\bx_i$,
 multivariate Gaussian  analysis shows that, for  centered $\bx_i$ and
 $\by_i$,
\begin{equation}
  \label{eq:cond_model}
  \by_i | \bx_i \sim
  \mathcal{N}\left(-\bOmega^{-1}_{\by\by}\bOmega_{\by\bx}
    \bx_i, \bOmega_{\by\by}^{-1} \right).
\end{equation}
This      model,      associated      to     the      full      sample
$\{(\bx_i,\by_i)\}_{i=1,\dots,n}$, can be written  in a matrix form by
stacking in  row the observations of  the responses on  the first hand,
and of the  predictors on the second hand, in  two data matrices $\bY$
and $\bX$ with respective sizes $n\times q$ and $n\times p$, so as
\begin{equation}
  \label{eq:cond_model_mat}
  \bY = \bX \bOmega_{\bx\by} \bOmega_{\by\by}^{-1} + \bvarepsilon, \qquad
  \vec(\bvarepsilon) \sim
  \mathcal{N}\left(\bzr_{nq}, \bI_{p} \otimes \bOmega_{\by\by}^{-1} \right),
\end{equation}
where, for a  $n \times p$ matrix ${\bf A}$,  denoting ${\bf A}_j$ its
$j$th  column, the  $\vec$ operator  is  defined as  $\vec({\bf A})  =
(\bA_1^T     \dots     \bA_p^T)^T$.      The     log-likelihood     of
\eqref{eq:cond_model_mat}  --   which  is  a   conditional  likelihood
regarding the joint model \eqref{eq:joint_model} -- writes
\begin{multline}
  \label{eq:log_lik}
  \log L(\bOmega_{\bx\by},\bOmega_{\by\by}) = 
  \frac{n}{2}\log\left|\bOmega_{\by\by}\right| + \\ \frac{n}{2}
  \trace\left(  \left(\bY -  \bX \bOmega_{\bx\by}\bOmega_{\by\by}^{-1}
    \right)          \bOmega_{\by\by}\left(\bY          -          \bX
      \bOmega_{\bx\by}\bOmega_{\by\by}^{-1} \right)^T\right) +
  \mathrm{cst.}
\end{multline}
Introducing  the  empirical  matrices  of covariance  $\bS_{\by\by}  =
n^{-1}\sum_{i=1}^n\by_i        \by_i^T$,        $\bS_{\bx\bx}        =
n^{-1}\sum_{i=1}^n\bx_i     \bx_i^T$,      and     $\bS_{\by\bx}     =
n^{-1}\sum_{i=1}^n\by_i \bx_i^T$, one has
\begin{multline}
  \label{eq:log_lik2}
  - \frac{2}{n}\log L(\bOmega_{\bx\by},\bOmega_{\by\by}) =
  - \log\left|\bOmega_{\by\by}\right| +
  \trace\left(\bS_{\by\by} \bOmega_{\by\by} \right) \\
  +     2\trace\left(    \bS_{\bx\by}\bOmega_{\by\bx}     \right)    +
  \trace(\bOmega_{\by\bx}\bS_{\bx\bx}                  \bOmega_{\bx\by}
  \bOmega_{\by\by}^{-1}) + \mathrm{cst.}
\end{multline}
This has been referred to  as a 'conditional Gaussian Graphical Model'
(cGGM) or 'partial Gaussian  Graphical Model' in the recent literature
\citep{2011_AoAS_yin,2012_JMLR_sohn,2012_JMA_lee,2012_arxiv_yuan}.  We
notice by comparing the cGGM \eqref{eq:cond_model} to the multivariate
regression model  \eqref{eq:reg_model_row} that $\bOmega_{\by\by}^{-1}
=  \bR \text{  and }  \bB =  -\bOmega_{\bx\by} \bOmega_{\by\by}^{-1}$.
Although  equivalent   to  \eqref{eq:reg_model_row},  the  alternative
parametrization \eqref{eq:cond_model}  shows two important differences
with  several implications.   First, in  light of  convex optimization
theory, % \citep{cvx_optim}
the  negative log-likelihood  \eqref{eq:log_lik}  can be  shown to  be
jointly   convex  in   $(\bOmega_{\bx\by},\bOmega_{\by\by})$  \citep[a
formal  proof  can   be  found  in][]{2012_arxiv_yuan}.   Minimization
problems  involving  \eqref{eq:log_lik} will  thus  be  amenable to  a
global solution,  which facilitates both  optimization and theoretical
analysis.    As   such,   the  conditional   negative   log-likelihood
\eqref{eq:log_lik}  will serve as  a building  block for  our learning
criterion.    Second,   it  unveils   new   interpretations  for   the
relationships  between input  and  output variables,  as discussed  in
\citet{2012_JMLR_sohn}: $\bOmega_{\bx\by}$ describes the \emph{direct}
relationships between  predictors and responses, the  support of which
we  are looking  for to  select relevant  interactions.  On  the other
hand,  $\bB$  entails  \emph{both  direct  and  indirect}  influences,
possibly  due  to  some  strong correlations  between  the  responses,
described by the covariance  matrix $\bR$ (or equivalently its inverse
$\bOmega_{\by\by}$).  To  provide additional insights  on cGGM, Figure
\ref{fig:model_insight}   illustrates    the   relationships   between
$\bB,\bOmega_{\bx\by}$ and $\bR$ in  two simple scenarios where $p=40$
and $q=5$.  Scenarios $a)$ and  $b)$ are discriminated by the presence
of a strong structure among the predictors. Still, the important point
to catch at this stage of the paper is how strong correlations between
outcomes can  completely ``mask'' the  direct links in  the regression
coefficients: the  stronger the correlation  in $\bR$, the less  it is
possible  to  distinguish  in   $\bB$  the  non-zero  coefficients  of
$\bOmega_{\bx\by}$.

\begin{figure}[htbp!]
  \centering
  \begin{tabular}{c@{\hspace{1cm}}c}
    \begin{tabular}{cccc}
      & $\bR_{\text{low}}$ & $\bR_{\text{med}}$ & $\bR_{\text{high}}$ \\
      & \includegraphics[scale=.1]{figures/R_low_cov}
      & \includegraphics[scale=.1]{figures/R_med_cov}
      & \includegraphics[scale=.1]{figures/R_high_cov} \\
      $\bOmega_{\bx\by}$ & $\bB_{\text{low}}$ & $\bB_{\text{med}}$ & $\bB_{\text{high}}$ \\
      \includegraphics[scale=.12]{figures/omega_cov}
      & \includegraphics[scale=.12]{figures/beta_low_cov}
      & \includegraphics[scale=.12]{figures/beta_med_cov}
      & \includegraphics[scale=.12]{figures/beta_high_cov}\\
    \end{tabular}
    &
    \begin{tabular}{cccc}
      & $\bR_{\text{low}}$ & $\bR_{\text{med}}$ & $\bR_{\text{high}}$ \\
      & \includegraphics[scale=.1]{figures/R_low_cov}
      & \includegraphics[scale=.1]{figures/R_med_cov}
      & \includegraphics[scale=.1]{figures/R_high_cov} \\
      $\bOmega_{\bx\by}$ & $\bB_{\text{low}}$ & $\bB_{\text{med}}$ & $\bB_{\text{high}}$ \\
      \includegraphics[scale=.12]{figures/omega_str}
      & \includegraphics[scale=.12]{figures/beta_low_str}
      & \includegraphics[scale=.12]{figures/beta_med_str}
      & \includegraphics[scale=.12]{figures/beta_high_str}\\
    \end{tabular} \\
    (a) & (b) \\
  \end{tabular}
  \caption{Toy examples to  illustrate the relationships between $\bB,
    \bOmega_{\bx\by}$ and  $\bR$ in the cGGM (better  seen in colors):
    on panel $a)$, a situation  with no particular structure among the
    predictors; on  panel $b)$, a strong  neighborhood structure.  For
    each panel,  we represent the  effect of stronger  correlations in
    $\bR$ on masking the direct links in $\bB$.}
  \label{fig:model_insight}
\end{figure}



%%% Local Variables:
%%% TeX-master: "JST_AOAS_main.tex"
%%% End:

